VirtualSync+: Timing Optimization with Virtual Synchronization

In digital circuit designs, sequential components such as flip-flops are used to synchronize signal propagations. Logic computations are aligned at and thus isolated by flip-flop stages. Although this fully synchronous style can reduce design efforts significantly, it may affect circuit performance negatively, because sequential components can only introduce delays into signal propagations but never accelerate them. In this paper, we propose a new timing model, VirtualSync+, in which signals, specially those along critical paths, are allowed to propagate through several sequential stages without flip-flops. Timing constraints are still satisfied at the boundary of the optimized circuit to maintain a consistent interface with existing designs. By removing clock-to-q delays and setup time requirements of flip-flops on critical paths, the performance of a circuit can be pushed even beyond the limit of traditional sequential designs. In addition, we further enhance the optimization with VirtualSync+ by fine-tuning with commercial design tools, e.g., Design Compiler from Synopsys, to achieve more accurate result. Experimental results demonstrate that circuit performance can be improved by up to 4% (average 1.5%) compared with that after extreme retiming and sizing, while the increase of area is still negligible. This timing performance is enhanced beyond the limit of traditional sequential designs. It also demonstrates that compared with those after retiming and sizing, the circuits with VirtualSync+ can achieve better timing performance under the same area cost or smaller area cost under the same clock period, respectively.

==> Makefile <==
SUBM_NAME := journal_virtualsyn
AUX_FILES := IEEEtran.cls 
BIO_FILE := biographies.tex
PHOTO_DIR := photos
FIGURE_DIR := Fig

# According to TCAD Guidelines
cameraReady: cameraReady/$(SUBM_NAME).pdf cameraReady/allFigsTables.pdf cameraReady/allCaptions.pdf packfigs packbios


cameraReady/$(SUBM_NAME).pdf: cameraReady/$(SUBM_NAME).tex copyfigs copybios
	cd cameraReady; pdflatex $(SUBM_NAME).tex
	cd cameraReady; pdflatex $(SUBM_NAME).tex
	cd cameraReady; pdflatex $(SUBM_NAME).tex

cameraReady/$(SUBM_NAME).tex: *.tex
	cd cameraReady; for i in $(AUX_FILES); do cp ../$$i .; done
	./flatex.py -s $(SUBM_NAME).tex cameraReady/$(SUBM_NAME).tex
        
copyfigs.sh: cameraReady/$(SUBM_NAME).tex
	sed -nf copyfigs.sed <  cameraReady/$(SUBM_NAME).tex > copyfigs.sh
        
copyfigs: copyfigs.sh
	rm -rf cameraReady/$(FIGURE_DIR); mkdir -p cameraReady/$(FIGURE_DIR); bash copyfigs.sh
        
packfigs: copyfigs
	cd cameraReady; rm figures.zip; zip figures.zip $(FIGURE_DIR)/*
        
cameraReady/figs.tex: cameraReady/$(SUBM_NAME).tex
	sed -nf allFigs.sed < cameraReady/$(SUBM_NAME).tex > cameraReady/figs.tex
        
cameraReady/tables.tex: cameraReady/$(SUBM_NAME).tex
	sed -nf allTables.sed < cameraReady/$(SUBM_NAME).tex > cameraReady/tables.tex

cameraReady/allFigsTables.pdf:cameraReady/$(SUBM_NAME).pdf allFigsTables.tex copyfigs cameraReady/figs.tex cameraReady/tables.tex
	cd cameraReady; pdflatex ../allFigsTables.tex
	cd cameraReady; pdflatex ../allFigsTables.tex
	cd cameraReady; pdflatex ../allFigsTables.tex
        
cameraReady/figCaptions.tex: cameraReady/$(SUBM_NAME).tex
	sed -n '/\\begin{figure\**}/,/\\end{figure\**}/ s/^.*\\caption{\(.*\)}/\\begin{figure}[t]\\caption{\1}\\end{figure}\n\n/p' < cameraReady/$(SUBM_NAME).tex > cameraReady/figCaptions.tex
        
cameraReady/tabCaptions.tex: cameraReady/$(SUBM_NAME).tex
	sed -n '/\\begin{table\**}/,/\\end{table\**}/ s/^.*\\caption{\(.*\)}/\\begin{table}[t]\\caption{\1}\\end{table}\n\n/p' < cameraReady/$(SUBM_NAME).tex > cameraReady/tabCaptions.tex
        
cameraReady/allCaptions.pdf:cameraReady/$(SUBM_NAME).pdf allCaptions.tex cameraReady/tabCaptions.tex cameraReady/figCaptions.tex
	cd cameraReady; pdflatex ../allCaptions.tex
	cd cameraReady; pdflatex ../allCaptions.tex
	cd cameraReady; pdflatex ../allCaptions.tex
        
copybios:
	rm -rf cameraReady/$(PHOTO_DIR); mkdir -p cameraReady/$(PHOTO_DIR); cp $(PHOTO_DIR)/* cameraReady/$(PHOTO_DIR)

packbios: copybios
	cp $(BIO_FILE) cameraReady
	cd cameraReady; rm biographies.zip; zip biographies.zip $(PHOTO_DIR)/* $(BIO_FILE)



==> abstract.tex <==
\begin{abstract}

In digital circuit designs, sequential components such as flip-flops are used
to synchronize signal propagations. Logic
computations are aligned at and thus isolated by flip-flop stages.  
%Consequently,
%EDA tools need to focus only on logic design and timing to guarantee proper
%behavior of a circuit.  
Although this fully synchronous style can reduce
design efforts significantly, it may affect circuit performance negatively,
because sequential components can only introduce delays into signal
propagations but never accelerate them.  In this paper, we propose a new
timing model, VirtualSync+, in which signals, specially those along critical
paths, are allowed to propagate through several sequential stages without
flip-flops.  Timing constraints are still satisfied at the boundary of the
optimized circuit to maintain a consistent interface with existing designs.
By removing clock-to-q delays and setup time requirements of flip-flops on critical
paths, the performance of a circuit can be pushed even beyond the limit of
traditional sequential designs. 
%To , %confirm the performance improvement,
%To 
%make the optimization with 
%integrate 
%\titlenym\ accurate, we 
In addition, we further enhance the optimization with VirtualSync+ by fine-tuning with
commercial design tools, 
e.g., Design Compiler from
Synopsys, to 
achieve more accurate result.
%To achieve this fine-tuning, we first 
%optimize the circuits %with the proposed timing model 
%by reallocating sequential components
%with sequential and combinational components as delay units. 
%Afterwards, 
%the removal locations of flip-flops with respect to the circuits under optimization are extracted and 
%the corresponding wave-pipelining timing constraints compatible with commercial design tools are established. 
%These timing constraints are then incorporated into the optimization flow of commercial tools 
%to generate the optimized circuits.
Experimental results demonstrate that circuit
performance can be improved by up to 4\% (average 1.5\%) compared with that
after extreme retiming and sizing, while the increase of area is
still negligible. This timing performance is enhanced beyond 
the limit of traditional sequential designs. 
%The fine-tuning with commercial tools  
%further confirms the timing performance improvement with \titlenym. % in the cases 
%where the extreme retiming and sizing method is relaxed. 
It also demonstrates that 
compared with those
after retiming and sizing, 
 the circuits with VirtualSync+ can achieve 
better timing performance under the same area cost 
or smaller area cost 
under the same clock period, respectively. 
%where extreme retiming and sizing is relaxed. 
 
%In addition, with integration of Design Compiler, we also demonstrate that 
%the circuits with \titlenym\ can achieve a smaller clock 
%period than those with retiming\&sizing under the same area cost and 
%the circuits with \titlenym\ can achieve a smaller area cost than those with 
%retiming\&sizing under the same clock period.
\end{abstract}




==> biographies.tex <==
\begin{footnotesize}
\vskip -40pt
%\begin{IEEEbiographynophoto}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Grace_Li_Zhang}}] 
{Grace Li Zhang} 
received the Dr.-Ing. degree from the Technical University of Munich (TUM), Munich, Germany, in 2018. She is currently a postdoctoral researcher pursuing Habilitation at the Chair of Electronic Design Automation, TUM, where she leads the research team on heterogeneous computing. Her research interests include neural networks and neuromorphic computing, computer architectures, and machine learning for EDA. She has served/is serving on the technical committee of several conferences including DAC, ICCAD, ASP-DAC, GLSVLSI etc. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -25pt
\begin{IEEEbiography}
%\begin{IEEEbiographynophoto}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Bing_Li}}] 
{Bing Li} received the Dr.-Ing. degree from Technical University of Munich (TUM), Munich, Germany, in 2010 and finished the Habilitation there in 2018. He is currently a researcher with the Chair of Electronic Design Automation, TUM. His current research interests include high-performance and low-power design, AI hardware, and emerging systems. He has served on the Technical Program Committees of several conferences including DAC, ICCAD, DATE, ASP-DAC, etc. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -20pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Xing_Huang}}] 
%\begin{IEEEbiographynophoto}
{Xing Huang} received the Ph.D. degree in electronic science and technology from Fuzhou University, Fuzhou, China, in 2018. 
%He was a joint Ph.D. with the Department of Electrical and Computer Engineering, Duke University, Durham, NC, USA. From 2018 to 2019, he was a Postdoctoral Researcher with the Department of Computer Science, National Tsing Hua University, Hsinchu, Taiwan. 
He is currently a Postdoctoral Research Fellow with the Chair of Electronic Design Automation, Technical University of Munich, Germany, sponsored by the Alexander von Humboldt Foundation.  His current research interests include design automation for microfluidic biochips and integrated circuits.
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -20pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Xunzhao_Yin}}]
%\begin{IEEEbiographynophoto}
{Xunzhao Yin} is an assistant professor of the College of Information Science and Electronic Engineering at Zhejiang University. He received his Ph.D. degree from University of Notre Dame in 2019 and B.S. degree from Tsinghua University in 2013, respectively.
His research focuses on emerging circuit/architecture designs and novel computing paradigms with both CMOS and emerging technologies. 
%He has published top journals and conference papers including Nature Electronics, IEEE TC, IEEE TCAD, IEEE TCAS, IEEE TED, DAC, IEDM, Symposium on VLSI, etc. He has received the best paper award nomination of ICCAD 2020, DATE2022 and VLSI Test Symposium 2021, Zhejiang University 2020 Top 10 academic research advancements nomination, etc. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -20pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Cheng_Zhuo}}]
%\begin{IEEEbiographynophoto}
{Cheng Zhuo} 
(M'12--SM'16)
received the B.S. and M.S. degrees in electronic engineering from Zhejiang University, Hangzhou, China, in 2005 and 2007, respectively. He received the Ph.D. degree in computer science \& engineering from the University of Michigan, Ann Arbor, MI, USA, in 2010. He is currently with Zhejiang University as a Professor in the college of Information Science \& Electronic Engineering. His current research interests include computing in memory, deep learning, and general VLSI EDA areas. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -15pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Masanori_Hashimoto}}]
%\begin{IEEEbiographynophoto}
{Masanori Hashimoto} received the Ph.D. degrees
from Kyoto University in 2001. He is currently a Professor with the Graduate
School of Informatics, Kyoto University. His current research interests include
design for reliability, timing and power integrity analysis, reconfigurable
computing, soft error characterization, and low-power circuit design.
%\end{IEEEbiographynophoto}
\end{IEEEbiography}
\vskip -15pt

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Ulf_Schlichtmann}}] 
%\begin{IEEEbiographynophoto}
{Ulf Schlichtmann} %(S'88--M'90--SM'18) 
 received the Dipl.-Ing. and Dr.-Ing. Degrees in electrical engineering and information technology from Technical University of Munich (TUM), Munich, Germany, in 1990 and 1995, respectively. He was with Siemens AG, Munich, and Infineon Technologies AG, Munich, from 1994 to 2003, where he held various technical and management positions in design automation, design libraries, IP reuse, and product development. Since 2003, he is Professor and the Head of the Chair of Electronic Design Automation at TUM. His current research interests include computer-aided design of electronic circuits and systems, with an emphasis on designing reliable and robust systems. Increasingly, he focuses on emerging technologies such as lab-on-a-chip and photonics.
%end{IEEEbiographynophoto}
%\end{IEEEbiographynophoto}
\end{IEEEbiography}
\end{footnotesize}
\vfill



==> cameraReady/biographies.tex <==
\begin{footnotesize}
\vskip -40pt
%\begin{IEEEbiographynophoto}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Grace_Li_Zhang}}] 
{Grace Li Zhang} 
received the Dr.-Ing. degree from the Technical University of Munich (TUM), Munich, Germany, in 2018. She is currently a postdoctoral researcher pursuing Habilitation at the Chair of Electronic Design Automation, TUM, where she leads the research team on heterogeneous computing. Her research interests include neural networks and neuromorphic computing, computer architectures, and machine learning for EDA. She has served/is serving on the technical committee of several conferences including DAC, ICCAD, ASP-DAC, GLSVLSI etc. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -25pt
\begin{IEEEbiography}
%\begin{IEEEbiographynophoto}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Bing_Li}}] 
{Bing Li} received the Dr.-Ing. degree from Technical University of Munich (TUM), Munich, Germany, in 2010 and finished the Habilitation there in 2018. He is currently a researcher with the Chair of Electronic Design Automation, TUM. His current research interests include high-performance and low-power design, AI hardware, and emerging systems. He has served on the Technical Program Committees of several conferences including DAC, ICCAD, DATE, ASP-DAC, etc. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -20pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Xing_Huang}}] 
%\begin{IEEEbiographynophoto}
{Xing Huang} received the Ph.D. degree in electronic science and technology from Fuzhou University, Fuzhou, China, in 2018. 
%He was a joint Ph.D. with the Department of Electrical and Computer Engineering, Duke University, Durham, NC, USA. From 2018 to 2019, he was a Postdoctoral Researcher with the Department of Computer Science, National Tsing Hua University, Hsinchu, Taiwan. 
He is currently a Postdoctoral Research Fellow with the Chair of Electronic Design Automation, Technical University of Munich, Germany, sponsored by the Alexander von Humboldt Foundation.  His current research interests include design automation for microfluidic biochips and integrated circuits.
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -20pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Xunzhao_Yin}}]
%\begin{IEEEbiographynophoto}
{Xunzhao Yin} is an assistant professor of the College of Information Science and Electronic Engineering at Zhejiang University. He received his Ph.D. degree from University of Notre Dame in 2019 and B.S. degree from Tsinghua University in 2013, respectively.
His research focuses on emerging circuit/architecture designs and novel computing paradigms with both CMOS and emerging technologies. 
%He has published top journals and conference papers including Nature Electronics, IEEE TC, IEEE TCAD, IEEE TCAS, IEEE TED, DAC, IEDM, Symposium on VLSI, etc. He has received the best paper award nomination of ICCAD 2020, DATE2022 and VLSI Test Symposium 2021, Zhejiang University 2020 Top 10 academic research advancements nomination, etc. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -20pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Cheng_Zhuo}}]
%\begin{IEEEbiographynophoto}
{Cheng Zhuo} 
(M'12--SM'16)
received the B.S. and M.S. degrees in electronic engineering from Zhejiang University, Hangzhou, China, in 2005 and 2007, respectively. He received the Ph.D. degree in computer science \& engineering from the University of Michigan, Ann Arbor, MI, USA, in 2010. He is currently with Zhejiang University as a Professor in the college of Information Science \& Electronic Engineering. His current research interests include computing in memory, deep learning, and general VLSI EDA areas. 
%\end{IEEEbiographynophoto}
\end{IEEEbiography}

\vskip -15pt
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Masanori_Hashimoto}}]
%\begin{IEEEbiographynophoto}
{Masanori Hashimoto} received the Ph.D. degrees
from Kyoto University in 2001. He is currently a Professor with the Graduate
School of Informatics, Kyoto University. His current research interests include
design for reliability, timing and power integrity analysis, reconfigurable
computing, soft error characterization, and low-power circuit design.
%\end{IEEEbiographynophoto}
\end{IEEEbiography}
\vskip -15pt

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./photos/Ulf_Schlichtmann}}] 
%\begin{IEEEbiographynophoto}
{Ulf Schlichtmann} %(S'88--M'90--SM'18) 
 received the Dipl.-Ing. and Dr.-Ing. Degrees in electrical engineering and information technology from Technical University of Munich (TUM), Munich, Germany, in 1990 and 1995, respectively. He was with Siemens AG, Munich, and Infineon Technologies AG, Munich, from 1994 to 2003, where he held various technical and management positions in design automation, design libraries, IP reuse, and product development. Since 2003, he is Professor and the Head of the Chair of Electronic Design Automation at TUM. His current research interests include computer-aided design of electronic circuits and systems, with an emphasis on designing reliable and robust systems. Increasingly, he focuses on emerging technologies such as lab-on-a-chip and photonics.
%end{IEEEbiographynophoto}
%\end{IEEEbiographynophoto}
\end{IEEEbiography}
\end{footnotesize}
\vfill



==> cameraReady/figCaptions.tex <==
\begin{figure}[t]\caption{Timing optimization methods. Delays of logic gates are shown on the gates. The clock-to-q delay ($t_{cq}$), setup time ($t_{su}$) and hold time ($t_{h}$) of a flip-flop are 3, 1 and 1, respectively. (a) Original circuit. (b) Sized circuit. (c) Circuit after retiming.  (d) Circuit after optimization using \titlenym.}\end{figure}


\begin{figure}[t]\caption{Properties of delay units, assuming the launching and capturing times of an active clock edge are 0 and $T$, respectively. (a) Linear delaying effect of a combinational delay unit. (b) Constant delaying effect of a flip-flop. (c) Piecewise delaying effect of a latch.}\end{figure}


\begin{figure}[t]\caption{Concept of relative timing references. Clock period T=10. Clock-to-q delay $t_{cq}$=3. Both setup time $t_{su}$ and hold time $t_h$ are equal to 1. F3 is kept in the optimized circuit and F2 is not included.}\end{figure}


\begin{figure}[t]\caption{Delay insertion model in \titlenym.}\end{figure}


\begin{figure}[t]\caption{The proposed timing optimization with relaxed \titlenym\ flow.}\end{figure}


\begin{figure}[t]\caption{The circuit under optimization and the optimized circuit after the adjusted iterative relaxation. (a) The circuit under optimization where $g_i$/ZN represent the output pin of $g_i$ and $g_i$/A, $g_i$/A1 and $g_i$/A2 are the input pins of $g_i$. (b) the optimized circuit where flip-flops are removed. }\end{figure}


\begin{figure}[t]\caption{Wave-pipelining paths with different number of logic waves are entangled with each other. Red dots represent anchor points, also the removal locations of flip-flops. $P1$, $P2$ and $P_3$ are the path set. The paths in $P_1$, as shown in blue, have three logic waves propagating along them and the paths in $P_2$ and $P_3$, as shown in green, have two logic waves propagating along them.}\end{figure}


\begin{figure}[t]\caption{Comparison of sequential delay units after buffer replacement.}\label{fig:se_cmp}\end{figure}


\begin{figure}[t]\caption{Area comparison before and after buffer replacement.}\label{fig:buffer_replace}\end{figure}


\begin{figure}[t]\caption{Area comparisons with extreme R\&S with the same clock period.}\label{fig:samet_area_cmp}\end{figure}


\begin{figure}[t]\caption{Comparison of the clock period reduction before and after fine-tuning with Design Compiler.}\end{figure}


\begin{figure}[t]\caption{Comparison of the area increase before and after fine-tuning with Design Compiler.}\end{figure}


\begin{figure}[t]\caption{The reduction of power and power-delay-area product compared with extreme R\&S.}\end{figure}


\begin{figure}[t]\caption{Area comparison between relaxed retiming and sizing and \titlenym\ when the target clock period is relaxed to 1.05T, 1.10T, 1.15T, 1.20T and 1.25T, where T is the clock period achieved by extreme R\&S.}\end{figure}




==> cameraReady/tabCaptions.tex <==
\begin{table}[t]\caption{Results of \titlenym}\end{table}




==> cameraReady/tables.tex <==
\begin{table*}[p]
\renewcommand{\tabcolsep}{4.15pt}
\centering
{\small
\renewcommand{\arraystretch}{1}
\vskip 10pt
\vskip -2pt
\label{tb_test}
\begin{tabular}{lrrr r rrrr r rr r rrr r rr r r} \hlinewd{0.7pt}
\multicolumn{4}{c}{Circuit} &
\multicolumn{1}{c}{} & 
\multicolumn{4}{c}{Ret.\&Siz.} &
\multicolumn{1}{c}{} &
\multicolumn{2}{c}{Cri. Part} &
\multicolumn{1}{c}{} &
\multicolumn{3}{c}{Opt. Circuit} &
\multicolumn{1}{c}{} &
\multicolumn{2}{c}{Comparison} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{Runtime}  \\
\cline {1-4} \cline{6-9}  \cline{11-12}  \cline{14-16} \cline {18-19} \cline {21-21} 
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$n_s$} &
\multicolumn{1}{c}{$n_c$} &
\multicolumn{1}{c}{$T(ps)$} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$n^\prime_{s}$} &
\multicolumn{1}{c}{$n^\prime_{c}$} &
\multicolumn{1}{c}{$n^\prime_{t}$} &
\multicolumn{1}{c}{$n^\prime_{a}$} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$n_{cs}$} & 
\multicolumn{1}{c}{$n_{cc}$} & 
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$n_{f}$} & 
\multicolumn{1}{c}{$n_{l}$} &
\multicolumn{1}{c}{$n_{b}$} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$n_{t}$} &
\multicolumn{1}{c}{$n_{a}$} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$t(s)$} \\
\hlinewd{0.8pt}
systemcdes &574  &1286 &1132 & &523 &2429 &55.5\% &23.1\% & &195  &2290 &  &65 &66  & 31& &2.5\%  &-5.4\%  & &2619.5 \\
tv80     &1014 &2998 &1025 & &1228 &5818 &40.0\% &50.4\% & &296 &5758 &  &158 &141  & 383 & &2\%  &0.6\% & &3081.5 \\
wb\_dma     &720  &1632 &666 & &716 &1974 &31.5\% &11.4\% & &129  &1375 &  &65 &46  & 240 & &8.5\%    &1.5\%  & &2211.3 \\
systemcaes &1181  &3318 &921 & &1635 &5078 &29.5\% &38.0\% & &363  &4531 &  &258 &150  & 141 & &3\%    &-1.5\%  & &2052.1 \\
mem\_ctrl  &879 &1840 &1105 & &1429 &3318 &51.0\% &68.3\% & &290 &2642 &  &156&93  & 296& &4.5\%  &-1.5\%  & &4510.5 \\
usb\_funct &2699 &4952 &1042 & &3005 &8901 &35.5\% &28.6\% & &333 &6293 &  &253&71  & 252 & &3\%    &0.1\%  & &2166.5 \\
ac97\_ctrl &1145 &1467 &802 & &2021 &2363 &48.5\% &70.9\% & &579 &1978 &  &430 &125 & 163& &1\%    &-2.2\% & &1961.2 \\
pci\_bridge&2301 &4993 &1141 & &6243 &6476 &33.5\% &130.1\% & &264 &4410 &  &156&48  & 140& &1\%    &-0.7\%  & &3563.1 \\
\hlinewd{0.7pt}
\end{tabular}
}
\end{table*}
	\clearpage


==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we have proposed a new timing model, \titlenym, in which 
sequential components and combinational logic gates are considered as delay units.
They provide different delay effects on signal propagations on short and long paths. 
With this new timing model, a timing optimization framework has been proposed
to insert delay units only at necessary locations.
%in the circuits to synchronize signal propagations. 
%We integrated \titlenym with Design Compiler to further demonstrate 
%the improvement of timing performance and area reduction. 
%With this technique, circuit performance can be
%improved by up to 8.5\% with a negligible increase of area overhead.
%allowing signal propagations to pass through several sequential stages with 
%flip-flops.
%Experimental results confirm the improvement of circuit performance in most cases while the increased 
%area overhead is accpetable.
%To improve the optimization accuracy, 
%we fine-tune the optimized circuits with \titlenym\ in Design Compiler. % to further demonstrate 
In addition, we further enhance the optimization with \titlenym\ by fine-tuning with
commercial design tools,
e.g., Design Compiler from
Synopsys, to
achieve more accurate result.
%the improvement of timing performance and area reduction. 
Experimental results show that circuit
performance can be improved by up to 4\% (average 1.5\%) compared with that
after extreme retiming and sizing, while the increase of area is
still negligible. 
%The circuit fine-tuning with \titlenym\ in commercial tools  
%also confirms the performance improvement. 
%In addition, 
%With integration of Design Compiler, we also demonstrate that
%compared with those
%after retiming and sizing, 
% the circuits with \titlenym\ can achieve
%better timing performance under the same area cost 
%and smaller area cost
%under the same clock period, respectively. 
\reviewhl{In the future work, 
we will %incorporate latches and 
enhance the framework to 
integrate \titlenym\ with physical design tools to fully automate virtual synchronization 
into the EDA flow. %We will also contact Synopsys for the access to their 
%Application Programming
%Interfaces (APIs), so that latches can be accommodated into the commercial tool to fully exploit the advantages of \titlenym. Furthermore, 
To implement wave-pipelining paths with latches using the commercial tools, 
however, either the commercial timing tools provide more flexible timing constraints for these paths or
they allow access to the APIs.} %our hope is to access the Application Programming Interfaces (APIs)
%of vendor tools in the future.} 
%For example, we will try to implement wave-pipelining paths with latches into the commercial tools with the access 
%to the APIs of the tools potentially.}
%We will explore the application of VirtualSync+ on large designs 
%with several hundreds of thousands of gates in the critical subcircuit.}
%the circuits with \titlenym\ can achieve a smaller clock  
%period than those with retiming\&sizing under the same area cost and
%the circuits with \titlenym\ can achieve a smaller area cost than those with
%retiming\&sizing under the same clock period.


%Future work includes 
%incorporating design for testing and low power based on the proposed framework. 
%We will also explore more 
%exploring more efficient methods, e.g., Lagrangian Relaxation, to reduce the
%runtime.
%to solve ILP problem
%i
%he proposed new timing model, e.g., Lagrangian relaxation.
%gate delay camouflage by doping modification\cite{BeckerRPB14,VAS17} to decouple gate delay from physical design further.
%In addition, clock skew scheduling in \cite{TZCC05,KNSK09,JT01,ZhangLS16} would also be explored in the same timing dimension to enhance the security of netlists.
%In the future work, we will explore the potential of skew scheduling of flip-flops to further enhance 
%the security of circuits\cite{LYH11,KAE03,JT01,ZhangLS16}.




 




==> cover_letter.tex <==
\setcounter{page}{0} 
\pagenumbering{roman}



\clearpage
\thispagestyle{empty} 
\begin{table*}
\begin{center}
\begin{minipage}[t][21.5cm][t]{15.2cm}
%\fontsize{10}{10}\selectfont
\renewcommand{\baselinestretch}{1.2} 
\normalsize


\vspace{0pt}

Dear Editors, dear Reviewers,\\

\vspace{3pt}

Enclosed please find our manuscript entitled \textit{\papertitle}. We submit this
manuscript as a regular paper for publication in IEEE Transactions on
Computer-Aided Design of Integrated Circuits and Systems. 
%We used the time after the publication of the conference paper to 
%enhance the virtual synchronization concept in several aspects and integrated it with a commercial tool chain. 
%In this manuscript, 
%a timing optimization framework and its integration with Design Compiler from Synopsys are 
%proposed to boost the timing performance of digital circuits. % beyond the limit of traditional timing 
%paradigm.  
%virutal synchronization with sequential and combinational components as delay units 
%are applied  
%to optimize timing peformance of digital circuits 
%We believe it would be of interest to the audience of this journal. 
%for publication in the Special Issue on Deep Physical Design Techniques for
%Next Generation Technologies, IEEE Transactions on Computer-Aided Design of
%Integrated Circuits and Systems.

\vspace{3pt}

%The method in this manuscript builds upon the one described in the appended
%paper,  
%\cite{LICS11}
This manuscript extends the appended paper,  
which was published at the Design Automation Conference (DAC), 2018. 
We used the time after the publication of the conference paper to
enhance the virtual synchronization concept in several aspects and fine-tune it with a commercial tool chain.
The enhancements are listed as follows.
%In this
%manuscript, we enhance the work described in the conference paper in the following
%aspects.

\vspace{3pt}

\begin{enumerate} 

%We analyze the diffculty in identifying the constructed wave-pipelining 
%paths by searching  

\item In the conference paper, 
the prototype of virtual synchronization with sequential and combinational
components as delay units is proposed %. With virtual synchronization, 
to push 
the timing performance of digital circuits beyond the limit of
the traditional timing paradigm. 
%a novel timing model where 
%sequential components and combinational
%logic gates are considered as delay units. With this timing model, 
%a timing optimization framework is proposed to 
%allocate sequential components only at necessary locations in the circuit to 
%boost the timing peformance of digital circuits. 
In this manuscript, 
this optimization is further enhanced by fine-tuning with 
Design Compiler from
Synopsys to 
achieve more accurate result.
%make timing performance improvement accurate. 
%the optimization with this prototype are 
%fine-tuned with Design Compiler from
%Synopsys to make timing performance improvement accurate. 
 
%the circuits optimized with this prototype are seamlessly integrated into Design Compiler from 
%Synopsys to improve timing peformance and reduce area cost.
%To realize this prototype, in this manuscript, we 
%integrate virtual synchronization 
%with Design Compiler from 
%Synopsys and demonstrate the timing performance improvement with this integration. %with respect to 


\item 
In the conference paper, the average pin-to-pin 
delays of logic gates are used in evaluating the arrival times of signals 
during the iterative relaxation of identifying where delay units should be inserted.  
However, this method
might incur inaccuracy in evaluating arrival times and thus path delays. Therefore, critical paths might be considered as non-critical and 
thus cannot be optimized effectively.   %in the iterative relaxation method of 
%identifying the locations of delay units. 
%However, this evaluation might incur inaccuracy in evaluating 
%arrival times of signals, so that the 
To solve this problem, in this manuscript, 
%To achieve the integration with Design Compiler,  
the iterative relaxation method 
is adjusted to 
compensate the inaccuracy in evaluating the arrival times of signals. 
In this adjustment, 
we take advantage of %the accurate timing analysis with 
Design Compiler 
to calibrate 
the arrival times. In addition, we shift gate sizing 
during the iterative relaxation  
to 
Design Compiler for the sake of accuracy and execution efficiency.
This extension is described in Section VI-A.


\item 
After the adjusted iterative relaxation is executed,
the removal of flip-flops 
creates wave-pipelining paths. % where several logic waves propagate
%simultaneously along a combinational path in the resulting circuit.
%To conduct the subsequent optimization to 
To optimize such paths with Design Compiler to satisfy the corresponding wave-pipelining constraints, 
%Design Compiler is used to optimize the circuits with respect to these constraints. 
%To achieve this goal, 
we first 
extract the removal locations of flip-flops with respect to the circuits under optimization 
by combining retiming and removing flip-flops. % on the initial circuits. %, which is described in 
%Section V-B.  
Afterwards, we use 
these removal locations to establish wave-pipelining timing constraints. %, which 
%To maintain the correct functionality of the circuits,
When establishing such constraints, 
wave-pipelining paths with different logic waves propagating along them are required to be separated. % to maintain the correct functionality of the circuits.  
%when establishing wave-pipelining constraints. 
To achieve this goal, we propose to identify the pins that separate such paths. 
The identified pins and the removal locations of flip-flops can thus be used 
to establish the corresponding wave-pipelining timing constraints. 
%is described in Section V-C. 
These constraints are then incorporated into 
Design Compiler to optimize the circuits. If the delays of short paths 
are still not large enough after the optimization, buffers are inserted to pad their delays. 
%and 
%use these removal locations to establish wave-pipelining timing constraints compatible with Design Compiler. 
%Afterwards, Design Compiler is used to optimize the circuits to meet such constraints. 
These three fine-tuning steps are described in Section VI-B, Section VI-C and Section VI-D, respectively. 
%and
%use these removal locations to establish wave-pipelining timing constraints compatible with Design Compiler.
%Afterwards, Design Compiler is used to optimize the circuits to meet such constraints.   

%\item 
%To maintain the correct functionality of the circuits, 
%When establishing wave-pipelining constraints, 
%wave-pipelining paths with different logic waves propagating along them are required to be separated 
%when establishing wave-pipelining constraints. 
%to maintain the correct functionality of the circuits. 
%To achieve this goal,  
%To establish wave-pipelining timing constraints for paths with different logic waves, 
%we propose to figure out the differentiated pins that separate such paths. % in Section V-C. 
%This extension is described in Section V-C. 
%The differentiated pins and the removal locations of flip-flops can thus be used 
%to establish the corresponding wave-pipelining timing constraints. 
%in Design Compiler for 
%the subsequent optimization. 
%them during normal operations of the chips.

\item 
In the experiments, we replaced the old circuits in ISCAS89 with the circuits in TAU13 contest 
to demonstrate 
%The experimental results in Section VII confirm 
the advantages of virtual synchronization in timing performance improvement and area reduction.%can push 
%the timing performance even beyond the limit of the traditional timing paradigm.

%reduction of area overhead and runtime for 
%the wave-pipelining construction in the conference paper. 

%We have also extended the texts of Section I--III to add more details of the proposed
%techniques.

%\item  Experimental results demonstrate that the number of test iterations can be
%reduced effectively while the circuit yield after tuning can be improved
%further due to a better delay estimation and statistical configuration.

\end{enumerate} 

%\vspace{-10pt}
%We confirm that this manuscript has not been published or submitted elsewhere
%and all authors have approved the manuscript and agree with the submission.\\

\vspace{10pt}


We look forward to hearing from you 
%at your earliest convenience.
and thank you very much for your time and consideration.


\vspace{15pt}

Yours sincerely,

\vspace{10pt}

Grace Li Zhang, Bing Li, Xing Huang, Xunzhao Yin, Cheng Zhuo, Masanori Hashimoto, Ulf Schlichtmann\\
%Grace Li Zhang, Bing Li, Meng Li, Bei Yu, David Z. Pan and Ulf Schlichtmann\\


\end{minipage}
\end{center}
\end{table*}

\clearpage
%\thispagestyle{empty} 
%\mbox{}
%\clearpage
\setcounter{page}{0} 
\pagenumbering{arabic}


==> inkscape_fix <==
#!/bin/bash

PAGES=$(pdfinfo $1.pdf | grep Pages | cut -d" " -f11) 
for j in $(egrep "includegraphics.*page=" $1.pdf_tex); do
    CHECKPAGE=$(echo $j | sed 's/^.*page=\([0-9]*\).*/\1/g');
       if [ $CHECKPAGE -gt $PAGES ]; then
           sed -i "s/^.*includegraphics.*page=$CHECKPAGE.*//g" $1.pdf_tex
       fi
done


==> integration.tex <==
\section{Circuit Fine-Tuning with \titlenym\ in Commercial Tools}\label{sec:integration}


%\subsection{Challenges in Integration of \titlenym}\label{sec:chanllege}

%To confirm the timing performance improvement with \titlenym, 
%The proposed timing optimization framework with iterative relaxation in Section~\ref{sec:impl} 
%can be used to quickly evaluate the benefit of VirtualSync+
%in circuit design. If it is beneficial to apply VirtualSync+,
%the integration method with
%Design Compilers from Synopsys\cite{design_compiler} 
%described in this section can be adopted to generate the optimized circuits.

The timing optimization with relaxed \titlenym\ described in Section~\ref{sec:impl} 
can generate the optimized circuits where timing performance is improved and area cost is reduced. 
However, this method might be inconsistent when it is interfaced with commercial tools, e.g., Design Compiler from Synopsys. 
%inaccuracy in optimizing circuits. 
For example, 
the average pin-to-pin delays are used in evaluating the arrival times
of signals for the sake of execution efficiency in the relaxed \titlenym. 
Therefore, %timing performance improvement and area reduction with this method might not be evaluated accurately. 
%To make the optimization accurate,  
we fine-tune the optimized circuits with Design Compiler. 

To fine-tune the optimized circuits with Design Compiler, there are 
several challenges. First, 
the arrival times of signals should be evaluated 
accurately to make the optimization effective. 
Second, after the optimization, 
the removal locations of flip-flops in the optimized circuits should be extracted 
to establish 
the wave-pipelining timing constraints, with which  
Design Compiler can fine-tune the circuits. 
Third, 
buffers should be adjusted along short paths to satisfy the wave-pipelining timing constraints. 


To overcome the challenges described above, %The flow of the fine-tuning with Design Compiler is illustrated in \figname~\ref{fig:integration}, 
we first adjust the iterative relaxation method where iterations of delay unit insertion are executed, as described in Section~\ref{sec:impl},  
to compensate the inaccuracy in timing optimization. Afterwards, 
we extract the removal locations of flip-flops with respect to the circuits under optimization  
%bridge the circuits optimized with the iterative relaxation in Section~\ref{sec:impl} 
%with the initial circuits and 
and establish the corresponding wave-pipelining constraints compatible with Design Compiler. 
These timing constraints are then incorporated into the commercial tools to 
optimize the circuits. 
After this optimization, the delays of short paths might be still too small to meet the wave-pipelining constraints, 
so that 
buffers are inserted to pad their delays until timing constraints are met. These steps 
can be automatically executed without manual intervention. 
%The flow of the fine-tuning with Design Compiler is illustrated in \figname~\ref{fig:integration}. 
%After padding delays for short paths, 
%the optimized circuits are generated.
%During this step, 
% combinational delay units such as buffers are inserted into the optimized circuits to enlarge the delays of 
%short paths. 
%\begin{figure}[t]
%{
%\figurefontsize
%\centering
%\input{Fig/integration.pdf_tex}
%\caption{Fine-Tuning of \titlenym\ with Design Compiler.}
%\label{fig:integration}
%}
%\end{figure}

 


\subsection{Adjusting Iterative Relaxation for Fine-Tuning of \titlenym}\label{sec:first_inte}

%When extracting critical paths 
During the iterative relaxation %of identifying locations of inserting delay units 
described 
in Section~\ref{sec:impl}, 
the average pin-to-pin delays are used in evaluating the arrival times of signals for the sake of execution efficiency. 
However, this simplification might incur inaccuracy in evaluating the arrival times of signals and thus path delays. 
Therefore, 
critical paths 
might be considered as non-critical and thus  
cannot be optimized effectively.
%with the iterative relaxation in Section~\ref{sec:impl}. 
%and thus causes 
%Therefore, I
%the resulting paths containing several logic waves might not meet the required          
%timing constraints. % due to the inconsistentcy between graph-based timing analysis and path-based timing analysis.
To 
solve this problem, we adjust the iterative relaxation in Section~\ref{sec:impl} to compensate this 
evaluation inaccuracy in timing optimization. 
%Since only the latest and earliest arrival times at the input of flip-flops 
%are essential for timing optimization, 
In this adjustment,  
we first run timing slack analysis for all the flip-flops of a circuit with Design Compiler 
%Therefore,Specifically,  
before executing the iterative relaxation framework.
%we first run the timing slack analysis for signals at the inputs of flip-flops in a circuit with Design Compiler. % before 
%Since we use path-based timing analysis in Design Compiler in evaluating the path delays, 
%the timing slack for each flip-flop is accurate. 
Afterwards, the latest and earliest arrival times of signals at the inputs of flip-flops evaluated with Design Compiler 
are used to calibrate those evaluated with the average pin-to-pin delays. 
Specifically, we record the gaps between arrival times evaluated with Design Compiler and with average pin-to-pin delays. 
During the optimization with the iterative relaxation, 
the arrival times at the inputs of flip-flops evaluated with average pin-to-pin delays are calibrated by adding
the corresponding gaps. % are used to calibrate the arrival times.  
%we record the gap between the arrival times at the inputs of flip-flops evaluated with Design Compiler and average
With this  calibration, the critical paths can be identified and optimized effectively. 
%With this calibration, the evaluation inaccuracy in the iterative relaxation 
%can be compensated  
%to optimize the critical paths effectively. 

During the timing optimization with the iterative relaxation framework, 
gate sizing plays an important role of increasing/decreasing delays for short/long paths to meet the timing constraints.
%However, achieving accurate gate sizing is challenging due to discrete cell sizes and complicated cell timing models considering 
%slew and load \cite{Hu2011}.
%considering slope and load incurs computation complexity. 
%However, the evaluation inaccuracy 
%Therefore, 
%However, 
%Although arrival times can be calibrated with Design Compiler 
%before the execution of the iterative relaxation, 
%Since the inaccuracy exists in evaluating arrivial times
Since Design Compiler has the advantages of high accuracy and execution efficiency 
in sizing gates while minimizing the area overhead, 
we shift the task of gate sizing to Design Compiler 
in the adjusted iterative relaxation framework. 
% since it can size gates efficiently while minimize 
%the area overhead. 
%we decouple the gate sizing 
%from the optimization flow in
%the iterative relaxation in Section~\ref{sec:impl}. 
Specifically, 
we first adopt the adjusted iterative relaxation without gate sizing %in Section~\ref{sec:impl} to 
to insert necessary sequential delay units to block fast signals along short paths in a circuit.   
Afterwards, we use Design Compiler to size gates to increase/decrease delays of short/long paths. 
If the delays of short paths are still too small after gate sizing, 
buffers are inserted to pad their delays, as explained later. %, which will be explained in Section~\ref{sec:fourth_inte}. 
%shift the task of gate sizing to Design Compiler. 
%In the adjusted iterative relaxation, 
%Specifically, 
%we evaluate the delay of a gate with the average of its rising and falling delays and restrict  
%such gates to be sized. 
%However, this method leads to timing inaccuracy since the reallocating of sequential components 
%with the iterative relaxation 
%might change the gate delays due to different slope and load with the original circuit. 
%To solve this problem, 
%we use Design Compiler to size gates in a circuit after it is optimized with the iterative relaxation in Section~\ref{sec:impl}.



\subsection{Extracting Removal Locations of Flip-flops }\label{sec:second_inte}
%In an initial circuit, 
%flip-flops are not removed 
After the adjusted iterative relaxation is executed, 
flip-flops along critical paths are removed and 
fast signals are blocked with sequential delay units in the optimized circuit. 
Therefore, 
the sequential components in the optimized circuit 
are reallocated with respect to the circuit under optimization. 
%In this paper, an initial circuit represents the circuit where flip-flops are not removed and 
%a resulting circuit represents the circuit after being optimized with the adjusted iterative relaxation. 
%applying the adjusted iterative relaxation on it.
%For example, 
\figname~\ref{fig:remove_ff} 
illustrates a circuit under optimization  %where the critial path is highlighted in blue. 
 and the optimized circuit where red dots represent anchor points, also the removal locations 
of flip-flops. 
By comparing the circuit under optimization in \figname~\ref{fig:remove_ff}(a) and the optimized  
circuit in \figname~\ref{fig:remove_ff}(b), we can see that  
F6 in the circuit under optimization  
is moved leftwards with retiming to block signals along a loop, 
while  % as shown in \figname~\ref{fig:remove_ff}(b).    
the retimed flip-flops 
between $g_4$ and $g_5$, $g_2$ and $g_5$ and F5 are removed to allow slow signals to propagate through. 
%F5 in the initial circuit is also removed 
 %F4 is moved leftwards to provide more delays for short paths between F4 and F7. 
\begin{figure}[t]
{
\figurefontsize
\centering
\input{Fig/remove_ff1.pdf_tex}
\caption{The circuit under optimization and the optimized circuit after the adjusted iterative relaxation. (a) The circuit under optimization where $g_i$/ZN represent the output pin of $g_i$ and $g_i$/A, $g_i$/A1 and $g_i$/A2 are the input pins of $g_i$. (b) the optimized circuit where flip-flops are removed. }
\label{fig:remove_ff}
}
\end{figure}

The removal of flip-flops %in \figname~\ref{fig:remove_ff} 
creates wave-pipelining paths where several logic waves propagate 
simultaneously in the optimized circuit. 
For example, in \figname~\ref{fig:remove_ff}(b), 
the wave-pipelining path from F2 to F4 has two logic waves propagating along it since this path traverses through one 
removal location along it and 
the wave-pipelining path from F1 to F4 has three logic waves 
propagating along it since it traverses through two removal locations along it. 
To guarantee the correct functionality of the optimized circuit, 
the delays of such paths should satisfy the corresponding wave-pipelining timing constraints. 
%The gates along these wave-pipelining paths should be sized in Design Compiler to satisfy the wave-pipelining timing constraints.  
For example, %the wave-pipelining constraints for the path between F1 and F4 are that
the largest delay of the path between F1 and F4 should be smaller than $3\cdot T-t_{su}$, and
the smallest delay should be larger than $2\cdot T+t_{h}$,
where $T$ is the target clock period, $t_{su}$ and $t_{h}$ are the setup time and hold time of F4, respectively. 
%To conduct subsequent optimization on the resulting circuit in Design Compiler to satisfy the wave-pipelining timing constraints, 
%In Design Compiler, however,  
%combinational paths between a pair of flip-flops are assumed to work within one period. % in Design Compiler.
To optimize such paths to satisfy the wave-pipelining constraints, %conduct the subsequent optimization, e.g., gate sizing and buffer insertion, 
we should 
establish the wave-pipelining constraints compatible with Design Compiler and then 
incorporate such constraints into the optimization flow of Design Compiler. 
%should make Design Compiler aware of the wave-pipelining paths in a circuit. 
To achieve this goal, 
we first extract the removal locations of flip-flops with respect to the circuit under optimization. % with an ILP formulation, as explained later. % and 
%use them to establish wave-pipelining timing constraints compatible with Design Compiler. 
%With these constraints, 
%Design Compiler can optimize the wave-pipelining paths in the resulting circuit correctly. 

According to \figname~\ref{fig:remove_ff}, 
the removal locations of flip-flops in the optimized circuit can be extracted 
by applying retiming together with removing flip-flops on the circuit under optimization. 
%with an ILP formulation, as explained later.
%We used an ILP formulation where retiming and removing flip-flops are used 
%to establish the relation between the initial circuit
%and the resulting circuit, which will described later. 
%To establish the relation between the initial circuit
%and the resulting circuit with 
%To apply retming and removing flip-flops, 
%we used an ILP formulation to establish the relation between the initial circuit
%and the resulting circuit, which will described later. %the relation between the initial circuit 
%and the resulting circuit. 
%the reallocated locations of flip-flops in the resulting circuit 
%can be derived  
%by applying retiming together with removing flip-flops on the initial circuit. 
%Therefore, 
%we extract the removal locations of flip-flops by  
%establishing the relation between the initial circuit and the resulting circuit 
%with retiming and removing flip-flops. 
To apply this technique on the circuit under optimization, %retiming together with removing flip-flops on the initial circuit, 
we use $g \in G$ to represent a combinational gate and $e_{g_i,g_j} \in E$ between gates $g_i$ and $g_j$ 
to represent the net connecting the output of the combinational gate $g_i$ and an
input of another combinational gate $g_j$. 
$e_{g_i,g_j}$ %between gates $g_i$ and $g_j$
has a constant weight $w(e_{g_i,g_j})$ to represent the number of flip-flops along
the connection in the circuit under optimization.
%The number of flip-flops along $e_{g_i,g_j}$ in the resulting circuit
%is denoted as $w^\prime(e_{g_i,g_j})$. $w(e_{g_i,g_j})$ and $w^\prime(e_{g_i,g_j})$ are constants. % from the inital and resulting circuit.
Each combinational gate has a retiming variable $r(g)$, which defines how many flip-flops are moved from the
output of a gate to its inputs. After retiming, the number of flip-flops on a net between gates $g_i$ and $g_j$
is written as $w_r(e_{g_i,g_j})=w(e_{g_i,g_j})+r(g_j)-r(g_i)$. 
The number of flip-flops along $e_{g_i,g_j}$ in the optimized circuit 
is denoted as $w^\prime(e_{g_i,g_j})$, which can be different from $w_r(e_{g_i,g_j})$ due to the removal of flip-flops.  
%which can be derived by applying retiming together with removing flip-flops on the initial circuit. 
To determine how many flip-flops along $e_{g_i,g_j}$ are removed in the optimized circuit, 
a variable $y_{e_{g_i,g_j}}$ is assigned for $e_{g_i,g_j}$. 
%We use a variable $y_{e_{g_i,g_j}}$ to denote %whether 
%how many flip-flops along $e_{g_i,g_j}$ are removed. 
With this setting, two cases for a net between gates $g_i$ and $g_j$ should be examined.

\textbf{Case 1:} If the net from gate $g_i$ to gate $g_j$ has the retimed weight equal to the weight in the optimized circuit, namely 
$w_r(e_{g_i,g_j})=w(e_{g_i,g_j})+r(g_j)-r(g_i)= w^\prime(e_{g_i,g_j})$, 
%In this case, 
there is no removal of flip-flops along this net, so that $y_{e_{g_i,g_j}}=0$. For example, 
$y_{e_{g_5,g_6}}=0$ in case of $r(g5)=1$. 
%since there is no flip-flop along $e_{g_1,g_2}$ and $r(g1)=r(g2)=0$. Although $r(g3)=1$, $y_{e_{g_3,g_4}}=0$ since there is 
%only retiming applied along this net. 

\textbf{Case 2:} If the net from gate $g_i$ to gate $g_j$ has the retimed weight larger than that in the optimized circuit, namely
$w_r(e_{g_i,g_j})=w(e_{g_i,g_j})+r(g_j)-r(g_i)\ge w^\prime(e_{g_i,g_j})+1$, 
%In this case, 
flip-flops are removed along this net, and the number of removed flip-flops is $y_{e_{g_i,g_j}}=w_r(e_{g_i,g_j})-w^\prime(e_{g_i,g_j})$. 
For example, 
$y_{e_{g_4,g_5}}=1$, $y_{e_{g_2,g_5}}=1$ and $y_{e_{g_1,g_2}}=1$ .

When establishing the relation between the circuit under optimization and the optimized circuit, 
each of the cases above can happen. 
We use the constraints in the two cases described above 
to establish an ILP formulation %as follows 
%\begin{align}\label{eq:first_formulation_rrr}
%\equationfontsize
%&\text{Subject to} \nonumber \\ 
%&\text{$y_{e_{g_i,g_j}}=0$, if $w_r(e_{g_i,g_j})= w^\prime(e_{g_i,g_j})$}   \\
%&\text{$y_{e_{g_i,g_j}}=w_r(e_{g_i,g_j})-w^\prime(e_{g_i,g_j})$, if $w_r(e_{g_i,g_j})\ge w^\prime(e_{g_i,g_j})+1$} 
%\end{align}
and let the solver determine which case actually happens during %the optimization of
the adjusted iterative relaxation. After that, 
%where no objective is required since we only need a solution.
%After solving this formulation, 
we can obtain the removal locations of flip-flops 
along net connections where $y_{e_{g_i,g_j}} \ge 1$ in the optimized circuit. 

\subsection{Generating Wave-pipelining Timing Constraints for Integration of \titlenym}\label{sec:third_inte}

After the removal locations of flip-flops are extracted with the method in Section~\ref{sec:second_inte}, 
we can use them to automatically establish the wave-pipelining constraints compatible with Design Compiler. 
%For example, in \figname~\ref{fig:remove_ff},
%the path from F1 to F4 has 3 logic waves since it traverses through 2 removal locations
%along it, namely the connection between $g1$/ZN and $g2$/A
%as well as $g2$/ZN and $g_5$/A1.
%The wave-pipelining constraints for the path between F1 and F4 are that
%the largest delay should be smaller than $3\cdot T-t{su}$, and 
%the smallest delay should be larger than $2\cdot T+t_{h}$ \cite{Burleson1998}.
%where $T$ is the target clock period, $t_{su}$ and $t_{h}$ are the setup time and hold time of F4. 
In Design Compiler, 
wave-pipelining timing constraints can be set with the following commands 
\begin{nospaceflalign}
%&\text{\equationfontsize $set\_max\_delay$ $d$ -$from$ $p_1$ -$through$ $g_2$ -$through$ $g_2$/A -$through$ $g2$/ZN }\label{eq:setup_e} \nonumber\\
&\text{\equationfontsize $set\_max\_delay$ $d$ -$from$ $p_1$ -$through$ $p_2$ ... -$through$ $p_n$ -$to$ $p_{n+1}$} \nonumber\\
%&\text{\equationfontsize -$to$ $p_{n+1}$ }\nonumber\\
&\text{\equationfontsize $set\_min\_delay$ $d^\prime$ -$from$ $p_1$ -$through$ $p_2$ ... -$through$ $p_n$ -$to$ $p_{n+1}$} \nonumber
%&\text{\equationfontsize -$to$ $p_{n+1}$}\nonumber
\end{nospaceflalign}
%``$set\_max\_delay$ $d$ ($-from *p1$) $-through$ $p2$ ($-to p3$)" and ``$set\_min\_delay$ $d$ $-through/-to$ $p$" commands, 
where ``$set\_max\_delay$" and ``$set\_min\_delay$" are used to establish setup and hold time 
constraints 
 for long paths and short paths, respectively, 
``$through$" means propagating through, ``$from$'' and ``$to$'' mean leaving from and arriving at, $d$ and $d^\prime$ are delay values and $p_i$ is a pin name. 
``-$from$ $p_1$'' and ``-$to$ $p_{n+1}$'' can be removed in the constraints as long as the timing constraints are sufficient to identify required paths. 
In these timing constraints, setup time and hold time of flip-flops are subtracted and added automatically.  

In \figname~\ref{fig:remove_ff},
the path from F1 to F4 has three logic waves since it traverses through two removal locations
along it, namely the connection between $g1$/ZN and $g2$/A
as well as $g2$/ZN and $g_5$/A1.
The wave-pipelining constraints from F1 to F4 can be written as follows 
%The wave-pipelining constraints in Design Compiler can be written as 
%\begin{align}
%\text{set}\_\text{max}\_\text{delay} \quad \text{-through}\quad g_1\text{/ZN} \quad \text{-through} \quad g_2\text{/A}  \\
%\text{-through} \quad g_2\text{/ZN}\quad  \text{-through} \quad g_5\text{/A1}
%{\setlength{\abovedisplayskip}{2pt}
\begin{nospaceflalign}
&\text{\equationfontsize $set\_max\_delay$ 3$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_2$/A -$through$ }\label{eq:setup} \nonumber\\
&\text{\equationfontsize $g2$/ZN -through $g_5$/A1}\\
&\text{\equationfontsize $set\_min\_delay$ 2$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_2$/A -$through$ }\label{eq:hold} \nonumber\\ 
&\text{\equationfontsize $g2$/ZN -through $g_5$/A1.}
\end{nospaceflalign}
%{\setlength{\abovedisplayskip}{-15pt}

%{\setlength{\belowdisplayskip}{-12pt}

%\end{align}

The timing constraints of the paths with two logic waves in \figname~\ref{fig:remove_ff}, such as 
the paths from F2 to F4 and from F3 to F4
can be 
written similarly. %For example, 
%the wave-pipelining constraints between F2 and F4 are 
%{\setlength{\abovedisplayskip}{2pt}
%\begin{nospaceflalign}
%&\text{\equationfontsize $set\_max\_delay$ 2$T$ -$through$ $g_4$/ZN -$through$ $g_5$/A2}\label{eq:setup1}\\
%&\text{\equationfontsize $set\_min\_delay$ 1$T$ -$through$ $g_4$/ZN -$through$ $g_5$/A2.}\label{eq:hold1}
%\end{nospaceflalign}
\begin{figure}[t]
{
\figurefontsize
\centering
\input{Fig/separation1.pdf_tex}
\caption{Wave-pipelining paths with different number of logic waves are entangled with each other. Red dots represent anchor points, also the removal locations of flip-flops. $P1$, $P2$ and $P_3$ are the path set. The paths in $P_1$, as shown in blue, have three logic waves propagating along them and the paths in $P_2$ and $P_3$, as shown in green, have two logic waves propagating along them.}
\label{fig:separation}
}
\end{figure}


In \figname~\ref{fig:remove_ff}, 
the wave-pipelining paths with different number of logic waves are clearly separated. 
However, in some optimized circuits, wave-pipelining paths with different number of logic waves 
are entangled with each other. 
\figname~\ref{fig:separation} illustrates such a circuit, where 
the paths in $P_1$, as shown in blue color, % propagating through $g_1$/ZN, $g_4$/A1, $g_4$/ZN and $g_5$/A1 
has three logic waves propagating along it, 
since they traverse through two anchor points. 
The wave-pipelining constraints for such paths 
can be established with the two anchor points directly, similar to (\ref{eq:setup})-(\ref{eq:hold}).  
For example, the setup time constraint of such paths can be written as follows 
\begin{nospaceflalign}
&\text{\equationfontsize $set\_max\_delay$ 3$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_4$/A1 -$through$ }\nonumber\\
&\text{\equationfontsize $g4$/ZN -$through$ $g_5$/A1}\label{eq:setup1} %\nonumber
\end{nospaceflalign}
However, the paths in $P_2$ and $P_3$,  
as shown in green color, propagate through only one of the anchor points and 
entangle with the blue paths with three logic waves. 
Directly using one of the anchor points to  
establish the wave-pipelining constraints for such paths with two logic waves %, similar to (\ref{eq:setup1})-(\ref{eq:hold1}), 
%is not viable, 
leads to a conflict with
the wave-pipelining constraints established with two anchor points. 
For example, if the setup constraint for the paths in $P_2$ is written as follow 
\begin{nospaceflalign}
&\text{\equationfontsize $set\_max\_delay$ 2$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_4$/A1} \label{eq:setup2}
\end{nospaceflalign}
%the paths with 3 logic waves also traverse the same anchor point. 
%When establishing the corresponding timing constraints for the subsequent optimization, 
this constraint and the constraint (\ref{eq:setup1}) confuse Design Compiler, 
since the paths propagating through 
two anchor points also traverse through one of the anchor points. In this case, 
Design Compiler ignores the constraint in (\ref{eq:setup2}), so that the delays of the paths in $P_2$ 
cannot be optimized correctly. 
To solve this problem, 
the paths with two logic waves 
should be 
differentiated from the paths with three logic waves 
when establishing the corresponding timing constraints for the subsequent optimization. 
%otherwise the functionality of the optimized circuit cannot be maintained.

To differentiate the wave-pipelining paths with two logic waves from those with three logic waves,  
%in the resulting circuit such as \figname~\ref{fig:separation}, 
we propose 
to identify the pins that separate such paths. % with different numbers of logic waves. 
We call such pins \textbf{differentiating pins}.  
For example, 
to differentiate the wave-pipelining paths in $P_2$ from those in $P_1$, %propagating only through the first anchor point between 
we first find the sink flip-flops at which the paths in $P_2$ and $P_1$ arrive. %them sink flip-flops. 
As shown in \figname~\ref{fig:separation},
F5 and F6 are such sink flip-flops. 
%If the wave-pipelining paths in $P_2$ and $P_1$ share common sink flip-flops, 
%we need to find the differentiated pins to separate them. 
%If a sink flip-flops is not shared by those paths in $P_1$ and $P_2$, 
%we can use the anchor point together with the sink flip-flop 
%to establish the wave-pipelining constraints. For example, 
Since F6 is the sink flip-flop at which only 
the paths in $P_2$ can arrive, 
the wave-pipelining constraints in such a case can be established with the anchor point between  
$g_1$/ZN and $g_4$/A1 
together with the sink flip-flop as follows 
%{\setlength{\abovedisplayskip}{2pt}
\begin{nospaceflalign} 
%\fontsize{6.2pt}{1}\selectfont
%\equationfontsize
&\text{\equationfontsize $set\_max\_delay$ 2$\cdot T$ -$through$  $g_1$/ZN -$through$ $g_4$/A1 -$to$  F6/D}\nonumber\\
&\text{\equationfontsize $set\_min\_delay$ 1$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_4$/A1 -$to$ F6/D.}\nonumber
\end{nospaceflalign}   

\input{tb_test}

%If the wave-pipelining paths in $P_2$ and $P_1$ share common sink flip-flops, 
Since F5 is the sink flip-flop at which both wave-pipelining paths in $P_1$ and $P_2$ can arrive, 
we need to find the differentiating pins to separate them. 
%As shown in \figname~\ref{fig:remove_ff}, 
%the common sink flip-flop of the wave-pipelining paths in $P_2$ and $P_1$ is F5. 
%To extract the differentiated pin,  
To achieve this goal, 
we enumerate 
the paths starting from F5 and ending at the two anchor points backwards.   
For example, the path propagating through $g6$/A2, $g_3$/A, and $g_4$/A1 terminates at 
the anchor point between $g_1$/ZN and $g_4$/A1 
and 
the path propagating through $g6$/A1 and $g5$/A1 terminates at the anchor point between $g_4$/ZN and $g_5$/A1. 
By comparing these paths, it is clear that 
the pin $g_6$/A2 differentiates the wave-pipelining paths in $P_2$ from those in $P_1$. 
Therefore, the wave-pipelining constraints for the paths in $P_2$ can be established with the 
differentiating pin $g_6$/A2 and the anchor point between $g_1$/ZN and $g_4$/A1 
as follows
%{\setlength{\abovedisplayskip}{2pt}
%\equationfontsize
\begingroup
\allowdisplaybreaks
\begin{nospaceflalign}  
%\small
&\text{\equationfontsize $set\_max\_delay$ 2$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_4$/A1 -$through$ } \nonumber\\
&\text{\equationfontsize  $g_6$/A2}\nonumber\\
&\text{\equationfontsize $set\_min\_delay$ 1$\cdot T$ -$through$ $g_1$/ZN -$through$ $g_4$/A1 -$through$ } \nonumber\\
&\text{\equationfontsize  $g_6$/A2.}\nonumber
\end{nospaceflalign} 
%{\setlength{\belowdisplayskip}{-12pt}
\endgroup
Similarly, to differentiate the wave-pipelining paths in $P_3$ from those in $P_1$, we 
first find the common source flip-flops which the paths in $P_3$ and $P_1$ start from. 
As shown in \figname~\ref{fig:separation}, this common source flip-flop is F2. 
Afterwards, we enumerate the paths starting 
from F2 and ending at the two anchor points in a forward way. 
By comparing these paths, 
we can see that the pin $g_2$/A1 differentiates 
the wave-pipelining paths in $P_3$ from those in $P_1$. 
We then use the differentiating pin $g_2$/A1 and the anchor point between $g_4$/ZN and $g_5$/A1 to establish the wave-pipelining constraints. 
In a general case where $N$ anchor points exist in an optimized circuit after 
the removal locations of flip-flops are extracted, %Fig ??? illustrates such a circuit. 
%To establish the wave-pipelining constraints 
%for the subsequent optimization, we need 
we use the methods described above 
to establish the wave-pipelining constraints for the 
paths where the number of logic waves propagating along them is larger than 1. 
The generation of wave-pipelining constraints is fully automated without manual intervention. 
%Since the paths with $M$ logic waves, where $M \ge 2$, should propagate $M-1$ anchor points, 
%we then extract the wave-pipelining paths with $M$ logic waves by enumerating $M-1$ anchor points in the resulting circuit 
%iteratively. 

\subsection{Circuit Optimizing and Buffer Insertion with Commercial Tools}\label{sec:fourth_inte}

After the wave-pipelining constraints are established for the optimized circuit, 
we 
incorporate such constraints into Design Compiler to optimize this circuit. 
During the optimization,  
Design Compiler sizes gates to increase the delays in short paths to satisfy 
the wave-pipelining constraints. 
After this optimization, the delays of the short paths might still be 
too small to satisfy the wave-pipelining constraints. To pad their delays with Design Compiler, % in the short paths, 
we insert buffers in the optimized circuits to enlarge their delays with 
the command ``insert\_buffer $p$ -no\_of\_cells $d$ $t$", where $p$ is a pin name, $d$ is the number of buffers and $t$ is the type of 
buffers, e.g., BUF\_X1.  
The locations of buffers can be obtained from the adjusted iterative relaxation. Due 
to the heuristic optimization in the adjusted iterative relaxation, 
the number of buffers might not be large or small enough to satisfy the wave-pipelining constraints. 
To solve this problem, 
we iteratively insert/remove buffers along the short/long paths until the 
wave-pipelining constraints are met.  
%the locations of buffers might not be suitable. In this scenario, we 
%\subsection{Buffer Insertion to Pad Delays for Short Paths}\label{sec:fifth_inte}

%Due to the timing complexity of latches, 
%in the integration of VirutalSync+ with Design Compiler, we 
%assume that only flip-flops are used as delay units to block fast signals. 

%\subsection{Discussion}\label{sec:discussion}

%\input{tb_test}
%\nopagebreak


==> introduction.tex <==
\section{Introduction}

\IEEEPARstart{I}{n digital} circuit designs, clock frequency determines the timing performance
of %given 
circuits. In the traditional timing paradigm, sequential components,
e.g., edge-triggered flip-flops, synchronize signal propagations between pairs
of flip-flops.  Consequently, these propagations are blocked at flip-flops
until a clock edge arrives.  At an active clock edge, the data at the inputs 
of flip-flops are transferred to their outputs to drive the logic of the next stage.  
Therefore, combinational logic blocks are isolated by flip-flop stages. This fully synchronous
style can reduce design efforts significantly, since only 
timing constraints local to pairs of flip-flops need to be met.

Within the traditional timing paradigm, 
timing analysis and timing optimization 
have been explored extensively. 
\reviewhl{
%Since timing analysis and optimization are 
%the background of the proposed method, we briefly summarize them as follows. 
% namely 
In timing analysis, researchers focus on 
improving the execution efficiency and accuracy of analysis \cite{huiru2015,Cao2019,tsungwei2017,wire2020,ZhangLS16_iccad,ChenLS12}. 
In timing optimization, several methods have been proposed to improve 
timing performance. 
A widely adopted method is sizing, in which
logic gates are sized to improve objectives such
as clock frequency and area efficiency, while timing constraints between
flip-flops are satisfied.
Typical methods for gate sizing are based on Lagrangian Relaxation and sensitivity \cite{Wong1999,Hu2011,Jin2012,Huiru1999}.
%For example, 
%in \cite{huiru2015}, a novel timing analysis flow 
%considering the flexible properties of flip-flops 
%is proposed to improve the accuracy of  
%timing analysis. 
%To accurately evaluate gate delays and thus path delays 
%considering variations, 
%a novel analytical model is proposed in \cite{Cao2019}. 
%A statistical timing 
%model for CMOS inverter in near-threshold voltage region 
%is proposed in \cite{Cao20191} to make the timing analysis more accurate. 
%To capture accurate timing performance of a circuit, 
%a novel timing analysis framework is proposed in \cite{yuming2015} 
%to remove common path pessimism. 
%In \cite{tsungwei2017}, 
%a fast and accurate macro-modeling algorithm is proposed to accelerate hierarchical 
%timing analysis in large circuits. In addition,  
%a high-performance timing analysis tool is presented in \cite{opentimer2015} to enable 
%efficient and accurate timing analysis. 
%Recently, machine-learning-based methods have been developed to facilitate timing analysis. 
%For example, a novel machine-learning-based wire timing model is proposed 
%in \cite{wire2020} to accelerate  
%timing closure. 
%To deal with the timing uncertainty due to the lack of routing information, 
%a machine learning-based pre-routing timing prediction model is presented in \cite{prediction2019}.
%In addition, inspired by machine learning acceleration with
%graphics processing units (GPUs), % in \cite{gpu2020}, 
%static timing analysis accelerated with GPUs is proposed in \cite{gpu2020}.  
%Another research direction focuses on 
%In timing optimization, 
%Within the traditional timing paradigm, 
%many optimization methods have been proposed to improve
%circuit performance.  
%\reviewhl{%Since 
%In this paper, 
%we %the proposed method in the following sections 
%focus on 
%improving timing performance of digital circuits, 
%so that the existing timing optimization methods are first reviewed as follows.}
%A widely adopted method is sizing, in which
%gates are sized to improve objectives such 
%as clock frequency and area efficiency, while timing constraints between
%flip-flops are satisfied. 
%\reviewhl{Typical methods for gate sizing are based on Lagrangian Relaxation and or sensitivity.}
%For example, \cite{Wong1999} introduces a fast and exact
%algorithm for simultaneous gate and wire sizing to minimize 
%total area and propagation delay inside a circuit.  In \cite{Hu2011}, a Lagrangian
%Relaxation (LR) based formulation together with a graph model is proposed to
%optimize timing slacks and power consumption simultaneously.  In
%\cite{Jin2012}, a metaheuristic approach is developed to size logic gates that have
%the greatest impact on power-performance tradeoffs.  This method guarantees
%slack, capacitance and slew constraints throughout the optimization process.
%In addition, \cite{Huiru1999} presents a simultaneous gate and wire sizing based on 
%Lagrangian Relaxation to optimize timing, area and power of circuits. 
%\cite{Li2012} presents a framework for cell-type selection with
%a further extension of the traditional Lagrangian Relaxation to match discrete
%gate sizes, together with a min-cost network flow method
%to optimize power consumption. 
%To improve the speed of Lagrangian Relaxation-based gate sizing, 
%\cite{Anjur2020}, 
%a fast Lagrangian Relaxation-based multi-threaded gate sizing method is proposed in \cite{Anjur2020}. 
The second method to improve circuit performance in the traditional paradigm
is retiming, which moves sequential components, e.g., 
flip-flops, but still preserves the correct functional behavior of circuits.
The existing retiming methods usually focus on reducing execution time while improving 
the performance of digital circuits \cite{Zhou2006,Aaron2008,Beerel2017,Singh2005,Huimei2021}.
}
Useful clock skew is the third method to enhance timing performance of digital circuits. 
For example, \cite{Grace18_test,Zhang201611,LICS111} 
intentionally exploits clock skews to improve the yield of digital circuits. 
Beyond these techniques, a further method to improve clock frequency is to introduce approximation in computational result \cite{Chuangtao2021}. 
%In \cite{Zhou2006}, an efficient algorithm is proposed to retime sequential
%circuits under both setup and hold constraints.  The work in \cite{Aaron2008}
%demonstrates a maximum-flow-based approach to minimize the number of
%flip-flops. 
%while guaranteeing that timing constraints are satisfied and the
%functionality of circuits is maintained.
%In \cite{Beerel2017}, a new retiming method with a network-simplex algorithm
%is introduced for two-phase latch-based resilient circuits to reduce the
%overhead of normal and error detecting latches.
% in timing resilient designs.
%The work in \cite{Aaron2008} demonstrates a maximum-flow-based approach for
%register minimization while guaranteeing the existence of an equivalent
%initial state. 
%Retiming for FPGA has been investigated in \cite{Singh2005} to meet
%architecture constraints such as avoiding flip-flops through carry chains to
%guarantee a correct circuit function. 
%A retiming algorithm for 3-phase latch designs is proposed in \cite{Huimei2021} to improve the power and area 
%of digital circuits. 
%A retimed circuit can be further improved by introducing intentional clock skews or latches to 
%balance the delays of sequential stages with a finer granularity \cite{Zhang201611,LiS15}.
%\cite{ZhangLS16,Zhang201611,LiS15,ZhangLi2017,ZhangLi2018}.%\cite{Xun1999}.
%Clock skew scheduling, in which intentional skews are introduced to sequential components, 
%can be combined with retiming to 
%improve circuit performance further\cite{Xun1999}. 
%However, the inherent clock-to-q delays and setup time requirements of flip-flops 
%still exist, leading to a degradation of circuit performance. 

Wave-pipelining is the third method to improve circuit performance, where
several logic waves are allowed to propagate through combinational paths without
intermediate sequential components.  
Wave-pipelining paths are different from multi-cycle paths where there is only one logic wave propagating 
along them at a moment. \reviewhl{
In timing constraints,  
multi-cycle paths only restrict their delays to be smaller than a specified upper bound \cite{Gupta_1994,Higuchi_2002} while 
wave-pipelining  paths restrict not only the upper bound but also the lower bound of their delays.}
Wave-pipelining provides a mechanism to make
the clock frequency of a circuit independent of the largest path delay, which
limits circuit performance in traditional circuit designs \cite{Burleson1998}.
% Wave-pipelining per se is a virtual pipelining, in which each gate can be
% considered as a virtual storage element. 
As early as in \cite{wave93}, an algorithm to automatically equalize delays 
in combinational logic circuits is proposed to realize wave-pipelining.  
In \cite{Joy1993}, a linear method to minimize the clock period
using wave-pipelining is proposed. 
%The work in \cite{Burleson1998} introduces the fundamentals of
%wave-pipelining and investigates wave-pipelined VLSI chips and CAD tools for
%designing wave-pipelined circuits. 
%Recently, 
This method %is wave-pipelining 
is also explored for majority-based
beyond-CMOS technologies to improve the throughput of \reviewhl{majority inverter graph
designs} in \cite{Micheli17}. 
Testing methods of wave-pipelined circuits are proposed in \cite{test94}.  
Recently, wave-pipelining 
is applied to accelerate the dot-product operations of neural network accelerators in \cite{Yehuda2021}. 
In addition, wave-pipelining has been applied to enhance netlist security\cite{ZLYPS18,Timingcamouflge+20}.

The first two methods above can be used separately or jointly to improve
circuit performance.  
%They can be combined together to further optimize the circuit performance.
However, sequential components are assumed to synchronize signal propagations
in these methods, where no signal propagation through sequential components is allowed 
except at the clock edges. 
%Although sequential components can be removed by wave-pipelining, circuits
%with structures, such as feedback loops, must have at least a sequential
%component to guarantee the correct function.
This synchronization with sequential components achieves many benefits such
as reducing design efforts.  However, it limits circuit performance in two
regards. Firstly, sequential components have inherent clock-to-q delays and
impose setup time.  The former becomes a part of combinational
paths driven by the corresponding flip-flops and the latter requires a further 
part of the timing budget for the critical paths.  Secondly, delay imbalances
between flip-flop stages cannot be exploited since signal propagations are
blocked at flip-flops instead of being allowed to propagate through
flip-flops. Although clock skew scheduling can relieve this problem to some degree, 
%Although delay compensation between flip-flop stages is utilized in clock skew scheduling, 
it still suffers the inherent clock-to-q delays and setup time constraints of flip-flops. 
%and compensation between several flip-flop stages can not be exploited to
%improve circuit performance.  These delays slow down signal propagation.
%Secondly, the synchronization block signal propagation on critical paths,
%resulting in degradation of circuit performance.     
%Although 
The third method above, wave-pipelining, allows signals to pass through
sequential stages without flip-flops. However, this technique %is usually applicable to a well-balanced 
%circuit and 
is not compatible with
the traditional timing paradigm. 
Although a wave-pipelining utility that \reviewhl{interacts} with commercial tools is proposed in \cite{Yehuda2021} to achieve
delay balance, the proposed method in this work can only deal with generic combinational circuits without feedback loops, which 
restricts its application in sequential digital circuits.


In this paper, we propose a new timing model, \titlenym, which removes 
the confines of the traditional timing paradigm. Our contributions are as follows:
%\vspace{0.08cm}
\begin{itemize} 
\newlength{\mylength} 
\setlength\mylength{\parskip}
\setlength\parskip{1.0mm}
%\setlength\itemsep{0.5em}
\item 
In the proposed new timing model, sequential components and combinational 
logic gates are both considered as delay units. 
%Signal propagations in the
%combinational circuits after removing flip-flops are examined and delayed if a
%fast signal from a latter clock cycle may catch a slow signal from a earlier
%cycle. In this timing model, 
Combinational logic gates add linear delays of the same amount 
to short and long paths, where sequential components provide non-linear
delay effects, which provide different delay effects to fast and slow signal
propagations. %In addition, 
%a flip-flop 
%sequential components can provide a very large virtual delay
%if a signal reaches it far before the active clock edge, enabling an efficient
%replacement of many combinational delay components such as buffers to save
%chip area.  

\setlength\parskip{\mylength}

\item 
With the new timing model, a timing optimization framework is proposed to
allocate sequential components only at necessary locations in the circuit to
synchronize signal propagations, while the functionality of circuits is
maintained. The absence of flip-flops at some sequential stages allows 
a virtual synchronization to provide identical functionality as in the original circuit.
%the function same as the original circuit.  
%Since critical paths %naturally 
%may not need any propagation delay,
%the absence of sequential components on them allows a virtual synchronization
%to provide the function same as the original circuit. 
Consequently, the
original clock-to-q delays and setup requirements along the critical paths can
be removed to achieve a better circuit performance even beyond the limit of traditional
sequential designs.


\item
%To further confirm the timing performance enhancement, 
%To make the timing optimization with \titlenym\ accurate, 
The optimization with \titlenym\ is further enhanced by fine-tuning with
commercial design tools,
e.g., Design Compiler from
Synopsys, to
achieve more accurate result. 
%we fine-tune the optimized circuits    
%To realize the proposed timing optimization framework, 
%we integrate \titlenym\ 
%with commercial tools, e.g., Design Compiler from Synopsys. % to further confirm the 
%improvement of timing performance of digital circuits.  
To achieve this fine-tuning, we first
optimize the circuits %with the proposed timing model 
by reallocating sequential components.  
%with sequential and combinational components as delay units. 
Afterwards,
the removal locations of flip-flops with respect to the circuits under optimization are extracted and
the corresponding wave-pipelining timing constraints compatible with commercial design tools are established.
These timing constraints are then incorporated into the optimization flow of commercial tools
to generate the optimized circuits. % with accurate timing results.


%\item 

%Experimental results demonstrate that timing performance of circuits with the
%proposed framework can be improved by up to 4\% (average 1.5\%) 
%compared with circuits
%after extreme retiming and sizing, with only a negligible increase of area. 
%This timing performance is enhanced beyond        
%the limit of traditional sequential designs. 
%It
%also demonstrates that 
%compared
%with those after retiming and sizing, 
%the circuits with \titlenym\ can achieve
%better timing performance under the same area cost 
%or smaller area cost %compared
%under 
%the same clock period, respectively.

\end{itemize}
%\vspace{0.08cm}
The rest of this paper is organized as follows. In
Section~\ref{sec:motivation}, we explain the motivation and the basic idea of
the proposed method. The timing optimization problem is formulated in Section~\ref{sec:problem_formulation}. 
In Section~\ref{sec:model}, we provide a detailed
description of the proposed timing model \titlenym. 
%With this new timing model, 
The proposed timing optimization %framework implemented with  
with relaxed \titlenym\ timing model 
%iterative relaxation %to implement the proposed timing optimization framework 
%with an iterative relaxation method 
is described in Section~\ref{sec:impl}.  
%This timing framework can be used to quickly evaluate the benefit of VirtualSync+
%in circuit design. 
%To realize this framework, we integrated it with commercial tools, which is 
%The integration with commercial tools to realize \titlenym\ is 
Circuit fine-tuning with \titlenym\ in commercial tools is 
explained in Section~\ref{sec:integration}. 
Experimental results are reported in Section~\ref{sec:results}.  Conclusions
are drawn in Section~\ref{sec:conclusion}.
%\vfil









==> latexmkrc <==
@default_files = ("journal_virtualsyn.tex");

$pdf_mode = 1;

add_cus_dep('svg', 'pdf_tex', 0, 'inkscape' );
sub inkscape {
return system( "inkscape -D -z --file=\"$_[0].svg\" --export-pdf=\"$_[0].pdf\" --export-latex && ./inkscape_fix \"$_[0]\" " ); 
}


==> model.tex <==
\section{\titlenym\  Timing Model}\label{sec:model}
%\section{\reviewhl{\titlenym\  Timing Optimization Framework}}\label{sec:model}
  
\subsection{Delay Units} \label{sec:delay_units}

In the \titlenym\ framework, we first remove all sequential components, 
flip-flops, from the circuit under optimization.  
Consequently, logic synchronization may be lost because  
signals across fast paths may arrive at flip-flops in incorrect clock cycles, e.g., 
earlier than specified, or timing violations may be incurred.
%, such as the
%signal from F1 to F4 in \figname~\ref{fig:concept}(d) without flip-flops. 
In addition, signals along combinational loops should also be blocked to avoid
the loss of logic synchronization. For example, in  
\figname~\ref{fig:concept}(d), the combinational loop across the
XOR gate must have
%pass 
a sequential component; otherwise a signal loses synchronization after traveling
across it many times. 
%after an infinite number of iterations.
%in the end. 
%Therefore, signals traveling along such paths must be delayed.

To slow down a signal, three different components can be used as
delay units, namely, combinational gates such as buffers, 
flip-flops, and latches, which exhibit different delay
characteristics, as shown in \figname~\ref{fig:difference}, 
\reviewhl{where input/output time refers to the input/out arrival time of a signal}.
%where the term 
%\textbf{\textit{input gap}} refers to the difference of arrival times of two signals at a delay unit, 
%and the term \textbf{\textit{output gap}} represents the difference between their arrival times after they pass through the unit.
%After passing through a delay unit, the difference of arrival times represents the output gap of two signals.

In \figname~\ref{fig:difference}(a), a combinational delay unit adds the same amount
of delay to any input signal.
Consequently, the arrival time $s_v$ at the output of the combinational delay 
unit is linear to the arrival time $s_u$ 
%of the signal 
at the input of the
delay unit. Therefore, the absolute gap between \reviewhl{the early and late arrival times of signals} through
short and long paths does not change when a combinational delay unit is passed through.

\begin{figure}[t]
{
\figurefontsize
\centering
\input{Fig/difference.pdf_tex}
\caption{Properties of delay units, assuming the launching and capturing times of an active clock edge are 0 and $T$, respectively. (a) Linear delaying effect of a combinational delay unit. (b) Constant delaying effect of a flip-flop. (c) Piecewise delaying effect of a latch.}
\label{fig:difference}
}
\end{figure}

In delaying input signals, a flip-flop, as a sequential delay unit, behaves completely differently from a
combinational delay unit, as shown in \figname~\ref{fig:difference}(b). If the
arrival time of a signal falls into the time window [$t_h$, $T-t_{su}$], where
$t_h$ is the hold time and $t_{su}$ is the setup time, the output signal
always leaves at the time $T+t_{cq}$, with $t_{cq}$ as the clock-to-q delay of
the flip-flop. Therefore, the gap between \reviewhl{the early and late arrival times of two signals} 
%through short and long paths
reaching the input of a flip-flop is always reduced to zero at the output of the flip-flop.
This is a very useful property because the delays of short paths and long
paths in a circuit may differ significantly after all sequential components
are removed from the circuit under optimization.
 For many short paths, it is not possible to increase their delays
by adding combinational delay units such as buffers to them, because the combinational delay units on
the short paths may also appear on other long paths.
The increased delays along long paths might affect circuit performance negatively.
 Flip-flops are thus of
great use in this scenario, because short paths receive more delay
padding than long paths to align logic waves in the circuit.  

As the second type of sequential delay units, level-sensitive latches have a delay property combining those of combinational
delay units and flip-flops, as shown in \figname~\ref{fig:difference}(c), where
$0<D<1$ is the duty cycle of the clock signal.  Assume that a latch is
non-transparent in the first part of the clock period and transparent in the
second part of the clock period. If two input signals arrive at a latch when
it is non-transparent, the output gap is reduced to zero. If both signals
arrive at a latch when it is transparent, the gap remains unchanged. However,
if the fast signal reaches the latch when it is non-transparent while the slow
signal reaches it when it is transparent, \reviewhl{the gap between the early and late arrival times 
of two signals is} %the output gap of the two signals is
neither zero nor unchanged.  Instead, it takes a value between the two extreme
cases as illustrated in \figname~\ref{fig:difference}(c).  This property gives
us more flexibility to modulate signals with different arrival times, specifically those along 
critical paths where fast signals require more delay padding and
slow signals should not be affected.

%so that they
%still meet all the original setup time and hold time constraints when they
%arrive at the flip-flops at the boundary of the circuit under optimization.

\subsection{Relative Timing References} \label{sec:relative_timing}
In \figname~\ref{fig:concept}(a), if all the logic gates
and flip-flop F3 are considered as the circuit under optimization, 
F1, F2 and F4 are thus the boundary flip-flops. 
No matter how signals inside the circuit propagate, 
the function of the whole circuit is still maintained
if we can guarantee that for any input pattern at flip-flops F1 and
F2 the circuit produces the same result at F4 at the same clock cycle as the original circuit. 

Consider a general case in \figname~\ref{fig:minus_T}, where F1 and F4 are the
boundary flip-flops and F2 and F3 are removed in the initial circuit for
optimization. At F4, the arrival times are required to meet the setup and hold
time constraints, written as
\begin{align}
s_z+t_{su}\le T \label{eq:simple_setup}\\
s^\prime_z\ge t_{h}\label {eq:simple_hold}\
\end{align}
where $s_z$ and $s^\prime_z$ are the latest and earliest arrival times at $z$.
%and $s^\prime_t$ is the earliest
%arrival time. 
These two constraints in fact are defined with respect to the
rising clock edge at F3, since the clock period T in (\ref{eq:simple_setup})
shows that the signal should arrive at F4 within one clock period.  Although
F2 and F3 are removed from the circuit, the constraints at F4 should still be the 
same as (\ref{eq:simple_setup})-(\ref{eq:simple_hold}) to maintain the
compatibility of the timing interface at the boundary flip-flops.

\begin{figure}[t]
{
\figurefontsize
\centering
\input{Fig/minus_T.pdf_tex}
\caption{Concept of relative timing references. Clock period T=10. Clock-to-q delay $t_{cq}$=3. Both setup time $t_{su}$ and hold time $t_h$ are equal to 1. F3 is kept in the optimized circuit and F2 is not included.}
\label{fig:minus_T}
}
\end{figure}
In the general case in \figname~\ref{fig:minus_T},
we can also observe that the timing constraint at F3 in
the original circuit is also defined with respect to the rising clock edge at
F2. This definition can be chained further back until the source flip-flop F1
at the boundary is be reached. We call the locations of these removed
flip-flops such as F2 and F3 
%in the original circuit 
\textbf{\textit{anchor points}}.
%\textit{anchor points}. 
After all sequential components are removed from
the circuit under optimization, these anchor points still allow to relate timing information to boundary 
%these anchor points still provide information of relative relation to boundary
flip-flops. Every time when a signal passes an anchor point, its arrival time
is converted by subtracting $T$ in \titlenym. When a signal finally arrives at a boundary
flip-flop along a combinational path, its arrival time must be converted 
%by subtracting the number of flip-flops multiplied by $T$ on the same path in the original circuit.
so many times as the number of flip-flops on the path,
%it traverses. 
%the
%number of times equal to the the number of flip-flops on the same path in the
%original circuit. 
%This conversion naturally guarantees that the arrival time is
%defined with respect to the time for the boundary flip-flop,
%one clock period earlier than the clock edge
%for the boundary flip-flop, 
so that
(\ref{eq:simple_setup})-(\ref{eq:simple_hold}) is still valid.

In \figname~\ref{fig:minus_T}, assume that F2 is removed but F3 is
inserted back in the optimized circuit. The arrival time $s_u$ is subtracted
by the clock period T=10 to convert it with respect to the time at F1,
%the anchor point at F2,
leading to $s_v$=4. 
%Consequently, 
The arrival time $s_w$ is defined with
respect to the previous flip-flop before F3, so that the timing constraints
can be checked using (\ref{eq:simple_setup})-(\ref{eq:simple_hold}). 
%Because
%F2 does not appear in the optimized circuit, the delay of the first combinational
%logic block can thus exceed 10. 
Since the arrival time before F4 should meet
its timing constraints, F3 thus cannot be removed. Otherwise, the arrival time
$s_t$ would be equal to 7-10=-3. Accordingly, the arrival time $s_z$
%at the input of
%F4 
becomes -3+2=-1, definitely violating the hold time constraint in
(\ref{eq:simple_hold}).

Since F3 is kept in the optimized circuit, it introduces the delay with the
property shown in \figname~\ref{fig:difference}(b). 
The arrival time after this sequential delay unit thus becomes
$T+t_{cq}$=13. This signal at $t$ in \figname~\ref{fig:minus_T} also passes an anchor point. Therefore, the arrival
time $s_t$ is equal to 3, leading to no timing violation at F4. This example
demonstrates that the timing constraints at the boundary flip-flops force the
usage of the internal sequential delay units. \reviewhl{The model to automatically insert these
delay units} will be explained in the next section.

\subsection{Synchronizing Logic Waves by Delay Units} \label{sec:mode_delay_unit}

%In the circuit under optimization, signals start to propagate from boundary
%flip-flops, with arrival times equal to the clock-to-q delays. %of those
%flip-flops. 
With 
%anchor points in the circuit and 
all flip-flops removed
from the circuit under optimization, 
%during the propagation, 
we only need to delay signals that are so fast that
they reach boundary flip-flops too early; signals that propagate 
slowly are already on the critical paths, thus requiring no additional
delay. Since it is not straightforward to determine the locations for inserting
additional delays, we formulate this task as an ILP problem and solve it
later with introduced heuristic steps. The values of variables in the following sections are 
determined by the solver, unless they are declared as constants explicitly.
%described from Section ~\ref{sec:comb} to Section  ~\ref{sec:wave} are selected by the solver during the optimization. 
%Constant values will be pointed out. 

The scenario of delay insertion at a circuit node, i.e., a logic gate, is illustrated in 
\figname~\ref{fig:circuit_graph}, where a combinational delay unit $\xi_{uv}$ may be
inserted, the original delay of the logic gate may be sized, and a sequential
delay unit may be inserted to block fast and slow signals with different
delays. Furthermore, the number of flip-flops \reviewhl{between $t$ and $z$ in the original circuit} is 
represented by an integer constant $\lambda_{tz}$. When $\lambda_{tz}$$\ge$1, an anchor point is found at the location between $t$ and $z$. 
$\lambda_{tz}$ is used to convert arrival times.
%at the anchor point represented by an 
%integer constant $\lambda_{tz}$ in the original circuit need to be checked to convert arrival times..
% Furthermore, the appearance of an anchor point, represented by an
%integer constant $\lambda_{tz}$, the number of flip-flops at the anchor point, 
%in the original circuit need to be checked to 
%convert arrival times.
%checked.

\subsubsection{Combinational delay unit and gate sizing}\label{sec:comb}
\hfill \break
\indent In \figname~\ref{fig:circuit_graph}, the delay at the circuit node can be
changed by sizing the delay of the logic gate, e.g., the XOR gate in \figname~\ref{fig:circuit_graph}. 
For the case that the required
gate delay exceeds the largest permissible value, a combinational delay unit is inserted at 
the corresponding input. For convenience, we assume the combinational delay unit inserted 
at the input is implemented with buffers. 
The relation between the arrival times
$u$ and $w$ is thus expressed as
\begin{align} \label{eq:no_ff_orig}
      s_{w} \ge s_{u}+\xi_{uv}*r^u+d_{vw}*r^u \\
      s^\prime_{w} \le s^\prime_{u}+\xi_{uv}* r^l+d_{vw}*r^l \label{eq:no_ff_orig1}
\end{align}
where $s_{u}$, $s^\prime_{u}$, $s_{w}$ and  $s^\prime_{w}$ 
are the latest and earliest arrival times of node $u$ and $w$ , respectively.
\reviewhl{$\xi_{uv}$ is the extra delay 
introduced by an inserted buffer and $d_{vw}$ is the pin-to-pin delay of the logic gate. }
If $\xi_{uv}$ is reduced to 0 
after optimization,
%in the following
%optimization process, 
no buffer is required in the optimized circuit.
The $\le$ and $\ge$ relaxations of the relation between arrival times guarantee
that only the latest and the earliest arrival times from multiple inputs
are propagated further. 
$r^u$ and $r^l$ are two constants to reserve a guard band for process variations,
%take global process variations
%into account, 
so that $r^u >1 $ and $r^l<1$.

Rising and falling pin-to-pin delays of logic gates, e.g., the XOR gate in \figname~\ref{fig:circuit_graph}, 
\reviewhl{might be different}. % in case of rising and falling input signals. 
Using the rising and falling pin-to-pin delays of logic gates 
to separately establish the constraints of arrival times in 
(\ref{eq:no_ff_orig}) and (\ref{eq:no_ff_orig1}) incurs high computation complexity, and thus long execution time. 
For simplification, we evaluate $d_{vw}$ with  
the average of the rising and falling pin-to-pin delays of the logic gate. 
This simplification may lead to inaccuracy in 
evaluating arrival times of signals and thus affect the subsequent timing optimization negatively. To compensate 
this inaccuracy, we calibrate the arrival times of signals with commercial tools, which 
will be explained in Section~\ref{sec:first_inte}.
%and $\xi_{uv}$ is the extra delay 
%introduced by an inserted buffer. 

%This timing relaxation is 
%based on graph-based timing analysis, where only the latest and earliest arrival times 
%of gates are propagated to derive the latest path delay. 
%Graph-based timing analysis is usullay adopted in evaluating timing of circuits 
%due to the fast computation speed. However, this method suffers
%from inaccuracy compared with path-based timing analysis, which evaluates each path delay individually.
%$r^u$ and $r^l$ are two constants to reserve a guard band for process variations, 
%take global process variations
%into account, 
%so that $r^u >1 $ and $r^l<1$.

\begin{figure}[t]
{%\figurefontsize
\centering
\input{Fig/circuit_graph.pdf_tex}
\caption{Delay insertion model in \titlenym.}
\label{fig:circuit_graph}
}
\end{figure}

\subsubsection{Insertion of sequential delay units}\label{sec:seq}
\hfill \break
\indent Since arrival times through long and short paths reaching $w$ may have a
large difference, we may need to insert sequential delay units to delay 
the fast signal more than the slow signal. This can be implemented with the
sequential units shown in \figname~\ref{fig:difference}, where the gap between
the arrival times is reduced after passing a sequential delay unit, either a
flip-flop or a latch. To insert a sequential delay unit, three cases need to
be examined. \reviewhl{These cases have an ``either-or" relationship, which can be converted into 
equivalent linear forms \cite{gurobi}.}

\textbf{Case 1:} No sequential delay unit is inserted between $w$ and $t$ in
\figname~\ref{fig:circuit_graph}, so that
\begin{align}  \label{eq:ff_insertion_0}
  s_t\ge s_w\\
  s_t^\prime\le s^\prime_w.
\end{align}

\textbf{Case2:}  A flip-flop is inserted between $w$ and $t$. Assume the
flip-flop works at a rising clock edge. 
As shown in \figname~\ref{fig:difference}(b), a flip-flop only works properly 
%in a region [$t_h$, $T-t_{su}$]. 
 in a region $t_h$ after the rising clock edge and $t_{su}$ before the next
rising clock edge. 
Therefore, we need to bound  
the arrival times $s_w$ and $s^\prime_w$ into such a region by
\begin{align} \label{eq:ff_insertion_1}
      s_{w},s^\prime_{w} \ge N_{wt}*T+\phi_{wt}+t_{h}*r^u \\ 
      s_{w},s^\prime_{w} \le (N_{wt}+1)*T+\phi_{wt}-t_{su}*r^u
\label{eq:ff_insertion_2}
\end{align}
\reviewhl{where $N_{wt}$ is an integer variable whose value is determined by the solver. 
This variable 
represents that
the signal arrival time of $w$ 
can be within any clock cycle, 
the starting and ending time of which are $N_{wt}*T$ and $(N_{wt}+1)*T$, respectively. 
%$t$ %the output of the inserted sequential delay unit      
%can start with any number of clock cycles. % in VirutalSync+ framework
}  
$T$ is the given clock period. 
$\phi_{wt}$ is phase shift
of the clock signal. The available values of $\phi_{wt}$ can be set by designers.
If only one clock signal is available, $\phi_{wt}$ can be set to 0 and T/2 to
emulate flip-flops working at rising and falling clock edges. 

When the input arrival times fall into the valid region of a flip-flop as
constrained by (\ref{eq:ff_insertion_1})--(\ref{eq:ff_insertion_2}), 
the signal always starts to propagate from the next active clock edge, 
%the
%arrival time at the output of flip-flop is always equal to $(N_{wt}+1)T$+$\phi_{wt}$+$t_{cq}$,
so that the constraints can be written as
\begin{align}
  s_t \ge (N_{wt}+1)T +\phi_{wt}+t_{cq}*r^u\\ 
  s_t^\prime\le (N_{wt}+1)T +\phi_{wt}+t_{cq}*r^l.
\end{align}

%Note here the arrival time at the output of a newly inserted flip-flop is
%still defined with respect to the previous anchor point. 
%For a combinational
%path with multiple logic waves, $N$ can thus be larger than 1.

\textbf{Case3:} A level-sensitive latch is inserted between $w$ and $t$.
To be consistent with the active region of flip-flops, we assume that the
latches are transparent when the clock signal is equal to 0. We can then
bound the arrival times at $w$ the same as 
(\ref{eq:ff_insertion_1})--(\ref{eq:ff_insertion_2}).

As illustrated in \figname~\ref{fig:difference}(c), the latch is
non-transparent in the first part of the region and transparent in the 
second region. Accordingly, the latest time a signal leaves the latch can be expressed as
\begin{align} \label{eq:arriv_latch_orig_1}
%propagated further in the circuit.
s_t\ge N_{wt}*T+\phi_{wt}+D*T+t_{cq}*r^u\\ 
s_t\ge s_w+t_{dq}*r^u
\label{eq:arriv_latch_orig_2}
\end{align}
where (\ref{eq:arriv_latch_orig_1}) corresponds to the case that the latch is
non-transparent, so that the signal leaves the latch at the moment the clock
switches to 1. 
$D$ is the duty cycle of the clock signal with $0<D<1$.
% $t_{dq}$ is the
%data-to-q delay of the latch.
(\ref{eq:arriv_latch_orig_2}) corresponds to the case that the latch is
transparent, so that only the delay of the latch is added to $s_w$. 
$t_{dq}$ is the
data-to-q delay of the latch.

The earliest time a signal leaves the latch is, however, imposed by a constraint in the
less-than-max form as in \cite{SAMO90},
\begin{equation}\label{eq:latch_min_max}
  s^\prime_t\le \max\{N_{wt}*T+\phi_{wt}+D*T+t_{cq}*r^l,\;\; s^\prime_w+t_{dq}*r^l\}
\end{equation}
which cannot be linearized easily. In the \titlenym\ framework, the purpose of
introducing the sequential delay unit is to delay the short path as much as
possible. This effect happens when a signal arrives at a non-transparent latch. 
%when it is
%non-transparent. 
Therefore, we impose the arrival times of fast signals to be positioned 
in the non-transparent region, expressed as 
\begin{equation}\label{eq:latch_new_region}
N_{wt}*T+\phi_{wt}+t_{h}*r^u  \le s^\prime_{w} \le N_{wt}*T+\phi_{wt}+D*T
\end{equation}
while relaxing (\ref{eq:latch_min_max}) as
\begin{equation}\label{eq:latch_min_max_bound}
  s^\prime_t\le N_{wt}*T+\phi_{wt}+D*T+t_{cq}*r^l.
\end{equation}

When inserting the sequential delay unit, each of the three cases above can happen
in the optimized circuit. We use an integer variable to represent the
selection and let the solver determine which case happens during the optimization.

\subsubsection{Reference shifting with respect to anchor points}\label{sec:reference}
\hfill \break
\indent The arrival times in the model need to be converted each time when an anchor point is
passed. The constant $\lambda_{tz}$ represents the number of flip-flops at such a point in the original
circuit. In \figname~\ref{fig:circuit_graph}, the arrival time at $z$ is
shifted as
\begin{equation}
  s_z=s_t-\lambda_{tz}T.
\end{equation}
%where $\lambda_{tz}$ is a constant to represent the number of flip-flops
%between $t$ and $z$ in the original circuit. 

\subsubsection{Wave non-interference condition} \label{sec:wave}
\hfill \break
\indent \reviewhl{Since we allow multiple waves to propagate along a combinational path, we need to
guarantee that the signal of the next wave starting from a boundary flip-flop  never catches the
signal of the previous wave starting from the same flip-flop %from the previous wave.
\cite{Burleson1998}.} This constraint should be imposed to every node in the circuit.
For example, the constraint for node
$u$ is written as 
\begin{align} \label{eq:stable_orig}
       s_{u}+t_{stable}\le s^\prime_{u}+T
\end{align}  
where
$t_{stable}$ is the minimum gap 
between two consecutive signals.
%for the signal of previous wave safely passing through the node 
%without conflicts with the signal from next wave.

\subsubsection{Overall formulation}
\hfill \break
\indent The introduction of the relative timing references, or the anchor points,
in Section~\ref{sec:relative_timing} guarantees that the number of clock cycles
along any path does not change after optimization. %, because the newly introduced delay units, no
%matter combinational or sequential, only serve to introduce delays
%into the circuit. 
With the timing constraints
(\ref{eq:simple_setup})-(\ref{eq:simple_hold}) at boundary flip-flops,
the correct function of the optimized circuit is always maintained, without
requiring any change in other function blocks.

\reviewhl{The constraints (\ref{eq:simple_setup})--(\ref{eq:stable_orig}) excluding
(\ref{eq:latch_min_max}) need to be established at each node in the circuit
after flip-flops are removed to 
guarantee the correct timing interface to flip-flops at the boundary of the optimized circuit parts. 
If this timing interface %in the
%optimized circuits are correct,
is correct, 
the functionality of the circuit is maintained \cite{Burleson1998,Joy1993, Yehuda2021}}. The appearance of the combinational and
sequential delay units needs to be 
%controlled by integer variables to be
determined by the solver. The delays of logic gates should also be sized.  The
objective of the optimization is to find a solution to make the circuit work
at a given clock period $T$, while reducing the area cost.  
%\reviewhl{The objective can also be modified to minimize the clock period. In this 
%scenario, $T$ in (\ref{eq:simple_setup})--(\ref{eq:stable_orig}) excluding
%(\ref{eq:latch_min_max}) becomes a variable instead of a given value. 
%}
Taking all these
factors into account, the straightforward ILP formulation may become
insolvable. In practice, however, this technique only needs to be applied to
isolated circuit parts containing critical paths. In addition, we introduce
heuristic techniques to overcome this scalability problem, 
%such as iterative
%relaxation, 
as explained in the following section.




==> motivation.tex <==
\section{Background and Motivation}\label{sec:motivation}

\begin{figure}[t]
{
\figurefontsize
\centering
\input{Fig/concept.pdf_tex}
\caption{Timing optimization methods. Delays of logic gates are shown on the gates. The clock-to-q delay ($t_{cq}$), setup time ($t_{su}$) and hold time ($t_{h}$) of a flip-flop are 3, 1 and 1, respectively. (a) Original circuit. (b) Sized circuit. (c) Circuit after retiming.  (d) Circuit after optimization using \titlenym.}
\label{fig:concept}
}
\end{figure}
In traditional digital circuits, sequential components such as flip-flops
synchronize signal propagations between pairs of flip-flops using a global
clock signal, as shown in \figname~\ref{fig:concept}(a). The combinational
path between F2 and F3 is critical with a path delay equal to 17. 
Assume that the clock-to-q delay, the
setup time and the hold time of a flip-flop are 3, 1, and 1, respectively. The
minimum clock period of this circuit is thus equal to 21. 

To reduce the clock period, logic gates with smaller delays can be selected
from the library to accelerate signal propagations on the critical paths of the circuit, at the cost
of additional area overhead, leading to the circuit shown in
\figname~\ref{fig:concept}(b), where the logic gates that are not on the
critical path still have their original delays for the sake of saving area.
After sizing, the minimum clock period of this circuit is reduced to 16 units.
To reduce the clock period further, retiming can be deployed to move F3 to the
left of the XOR gate as shown in \figname~\ref{fig:concept}(c), leading to a
minimum clock period equal to 11. 


The circuit in \figname~\ref{fig:concept}(c) has reached the limit of timing 
performance in the traditional timing model, and no other method except a logic
redesign can reduce the clock period further. 
%\reviewhl{
However, this strict timing constraint can still be relaxed by removing F6
from the circuit, leading to the circuit in \figname~\ref{fig:concept}(d). 
%This circuit is a solution with \titlenym, where F6 is removed and F5 as well as F3 are inserted back to block fast signals.}
If the signal from from F2 can reach the sink flip-flops F3 and F4 after the
next rising clock edge and before the rising edge two periods later, data can
still be latched by F3 and F4 correctly. Since the inverter before F4 can also
be sized further, \reviewhl{the largest path delay including clock-to-q delay is 16. 
The minimum clock period constrained by this path is thus 
(16+1)/2=8.5. In this scenario, 
the minimum clock period of the circuit is limited by the delay of the path from F5 to F4, which is 9,  18.2\% lower than retiming.}
\reviewhl{The circuit in \figname~\ref{fig:concept}(d) is one of the solutions with \titlenym, where F6 is removed and F5 as well as F3 are inserted back to block fast signals.}

%which imposes a 
%lower bound for the clock period as (16+1)/2=8.5. %22.7\% lower than retiming.

Since F6 can be removed from the circuit without affecting its function in fact, it
makes no contribution to the logic function or timing performance in
\figname~\ref{fig:concept}(c).  However, the flip-flop F5 in
\figname~\ref{fig:concept}(c) cannot be removed, because the signal from F1
should also arrive at F4 later than one clock period.
Without F5, the signal from F1 arrives at F4 even before the next rising clock edge, 
 and thus a loss of logic synchronization arises compared with the circuit in \figname~\ref{fig:concept}(a).
%of the next wave from F1 causes a hold time violation. 
Comparing \figname~\ref{fig:concept}(b) and
\figname~\ref{fig:concept}(d), \reviewhl{we can see that F3 in
\figname~\ref{fig:concept}(b) blocks the fast path from F1 to F4 and breaks the feedback loop to avoid loss of 
logic synchronization}, but it degrades the circuit performance by delaying
the signal from F2 to F4 too.   

The concept to allow logic signals to span several sequential stages without a
flip-flop separating them is called \textit{wave-pipelining}
\cite{Burleson1998}. Previously, this technique has only been explored in the
context of circuit design, where the numbers of waves on logic paths should be
defined and their synchronization should be maintained by designers during the
design phase. Since logic design and timing cannot be handled separately as in traditional synchronous designs, 
wave-pipelining becomes incompatible with the traditional fully
synchronous design paradigm, which prevents its adoption in practical designs.
%Although a wave-pipelining utility that interacting with commercial 
%tools is proposed in \cite{Yehuda2021}, 
%the proposed method can only deal with purely combinational circuits without flip-flops, which
%restricts its application in sequential digital circuits.
%Although a utility that interacting with commercial tools is proposed in \cite{Yehuda2021} to achieve 
%wave-pipelining, the proposed utility can only 
In \titlenym, we introduce a new timing model that allows multiple waves on
logic paths as a technique of timing optimization for sequential digital circuits in the
traditional design style. The resulting circuits still provide correct timing
interfaces to sequential components, e.g., flip-flops, at the boundary of the
optimized circuits to maintain timing compatibility.

%\begin{figure}[t]
%{
%\figurefontsize
%\centering
%\input{Fig/wave_delete.pdf_tex}
%\caption{Timing optimization in the \titlenym\ framework. (a) Circuit with wave-pipelining. (b)
%Circuit after optimization using \titlenym.}
%\label{fig:wave_delete}
%}
%\end{figure}




==> problem_formulation.tex <==
\section{Problem Formulation}\label{sec:problem_formulation}

In digital circuits, \reviewhl{we propose that the essential function of sequential components is to
delay signals along fast paths in a circuit.} For example,  in
\figname~\ref{fig:concept}(d), F5 must be kept in the circuit to delay the
signal propagation from F1 to F4. The sequential components that only sit on
the critical path can thus be removed to improve circuit performance, such as F6 in
\figname~\ref{fig:concept}(d). 
%The challenge of this task is to locate the
%flip-flops that can be removed in the original circuits.
%In \figname~\ref{fig:concept}(a), F3 cannot be removed directly. 
%After retiming shown in \figname~\ref{fig:concept}(c), unnecessary flip-flops, 
%such as F6 can be removed.   

%and block signals along fast paths at necessary locations, such as F5 in 
% \figname~\ref{fig:concept}(d).
%and block signals along fast paths at necessary locations.

% because they have different locations compared
%with their original locations in \figname~\ref{fig:concept}(a).

%Through the above analysis, 
In the \titlenym\ framework, we 
%examine this problem differently. Instead of
%trying to remove flip-flops from a given circuit without affecting its
%&unction, we 
remove all flip-flops and then identify the necessary locations
to block fast signals using combinational gates and sequential components, e.g., buffers, flip-flops,
and latches. The advantage of this formulation is that it is possible to
insert the minimum number of delay units into the circuit to achieve the theoretical
minimum clock period.

The problem formulation of \titlenym\ is described as follows:

\noindent \textit{Given}: the netlist of a digital circuit; the delay
information of the circuit; the target clock period T.

\noindent \textit{Output}: a circuit with adjusted number and locations of sequential
components; logic gates with new sizes; inserted delay units, e.g., buffers.

\noindent \textit{Objectives}: the circuit should maintain the same function viewed
from the sequential components at the boundary of the optimized circuit; the
target timing specification should be met; the area of the optimized circuit 
should be reduced. 

\reviewhl{In the following sections, we will introduce the proposed \titlenym\ timing optimization framework. 
Delay units and their insertion with a complete timing model %of delay unit insertion 
are first explained in Section~\ref{sec:model}. 
Since it is time-consuming to optimize circuits with the complete model,
we introduce a heuristic optimization framework with relaxed \titlenym\ timing model %&for timing optimization %to optimize the timing performance of digital circuits
in Section~\ref{sec:impl}. 
This optimization is further applied together with %enhanced by fine-tuning with 
Design Compiler from Synopsys to achieve more accurate results
in Section~\ref{sec:integration}.}




==> replies.tex <==

\newcommand{\reviewb}{\setcounter{page}{0}\pagenumbering{roman}\thispagestyle{empty}} 
\newcommand{\reviewe}{\clearpage\setcounter{page}{0}\pagenumbering{arabic}} 
%\fontsize{11}{12}\selectfont
\newcommand{\spb}{\clearpage\begin{table*}\begin{center}\begin{minipage}[t][24cm][t]{13.5cm}\normalsize} 
\newcommand{\spe}{\end{minipage}\end{center}\end{table*}} 

\reviewb

\spb

Dear Editor-in-Chief, dear Associate Editor, dear Reviewers,\\

Enclosed is the revised version of the paper TCAD-2021-0456. This paper was
reviewed for TCAD and a major revision was required, which we have done in
this version according to the comments and suggestions.\\

We thank the editors and the reviewers sincerely for giving us the constructive
comments and suggestions to improve this manuscript.\\

The textual changes in this manuscript are highlighted using blue color.
A detailed discussion on the changes and the comments in the reviews
is given as follows, where the comments from the reviewers are 
printed in italics.\\

\vspace{35pt}

\textbf{Reviewer: 1} \\

\textit{Comments to the Author}\\
\vskip -5pt
\textit{
This manuscript introduces the timing model VirtualSync+ to 
improve the circuit performance. According to the experiments, 
the performance improvement is 1.5\% on average and the area increase is negligible. This paper is well written.
%The reviewer has a few questions as listed below:
}\\

Thanks a lot for your positive feedback.
%\vskip -5pt

\vskip 10pt
\textit{
(1) This paper compares performance and area. How about the power/energy consumption? It might be more clear to demonstrate the improvement by Energy-Delay-Area product.
}\\

Thanks a lot for the comments. 
In this revised manuscript, we have provided the comparisons of power %comparison and 
and power-delay-area product between VirtualSync+ and extreme retiming and sizing, as illustrated  %comparison 
in Figure 14 on page 12. 
According to this figure, the circuits optimized with VirtualSync+ can 
achieve smaller power/power-delay-area product compared with the 
circuits after extreme retiming and sizing in most cases. 
%\textbf{need more experimental results to demonstrate power consumption.}
\\

\textit{
(2) According to the paper, ``the performance improvement without the fine-tuning is a theoretical upper bound of timing performance improvement". How did you accommodate latches in the commercial tool, what techniques can be further adapted to VirtualSync+ or Design Compiler to close the gap?
}\\

Thanks for these insightful comments. 
With VirtualSync+, 
wave-pipelining paths where latches are inserted to block fast signals  
might be generated to optimize timing performance. 
%Along such a path, a latch %, one of the three delay units, 
%might be inserted %between a pair of flip-flops %as a
%to block fast signals between a pair of flip-flops. 
To guarantee
the correct timing interface, 
the corresponding wave-pipelining timing constraints should be imposed on such paths where 
signals travel from a flip-flop, propagate through a latch and arrive 
at another flip-flop. 
%For example, ``set\_max\_delay -through pin\_name" and ``set\_min\_delay -through pin\_name" can be used to impose 
%such constraints. 
Only with these constraints, 
such paths could be optimized with gate sizing and buffer insertion in Design 
Compiler.  %is analyzed with a 
The timing in the resulting circuit should be verified with a timing analysis tool. 
%timing analysis tool. 
%to guarantee 
%the correct timing interface with respect to the original circuit. 
However, 
Design Compiler and  the timing analysis tool, Primetime from Synopsys, 
do not support %such timing constraints and thus 
timing optimization and timing analysis of such paths % where signals travel from a flip-flop, propagate through a latch and arrive 
%at another flip-flop. %where latches are considered as delay units 
with the commands ``set\_max\_delay" and ``set\_min\_delay", respectively.  
From the perspective of the tools, a latch is the start or the end of a path, so that 
they do not optimize or analyze paths propagating through it. 
%a path traveling 
%from a flip-flop, propagating through a latch and arrive at another flip-flop is not analyzed. 
One possible solution is to 
split such a wave-pipelining path into two paths whose start or end are a latch for timing optimization and
%the subsequent timing 
analysis. 
%If such a wave-pipelining path is split into two paths whose start or end are a latch for timing optimization and 
%the subsequent analysis, 
However, 
such a separate timing optimization %of such separated paths 
with Design Compiler 
deprives of the flexibility of delay compensation between the separated paths, 
which poses challenges in 
%Accordingly, it is challenging to guarantee the delays of the wave-pipelining paths propragating through latches   
satisfying the corresponding wave-pipelining timing constraints. 
%we consider a latch to be the end of a path along the generated wave-pipelining paths,  
%signals might travel along a huge number of combinational 
%paths to arrive at the input of a latch, either at its transparent region or non-transparent region. 
%To make such paths satisfy the wave-pipelining constraints, %realize the optimized circuits in the commerical tool, 
%these paths should be enumerated to make them arrive the latch at the target time, which 
%is very challenging since the number of paths might be huge.  
%an efficient method should be developed to separate 
%fast paths arriving at its non-transparent region %should be separated 
%from slow paths arriving at its transparent region, which is very challenging since the number of paths might be huge. 
%so that the corresponding timing constraints can be imposed on such paths in Design Compiler. 
%This condition restricts the accomodation of latches that are considered as delay units in VirtualSync+ in the commercial tool. 
%In addition, Primetime cannot analyze a large circuit with latch loops, which might exist in the optimized circuits 
%after the application of VirtualSync+.  
%Accordingly, 
These conditions %described above 
restrict the accommodation of latches in the optimized circuits with VirtualSync+ into the commercial tool.  
We have added this analysis in the first paragraph in the right column on page 13. \\
\spe\spb

%To integrate VirtualSync+ timing model %where latches and flip-flops are considered as delay units 
%into the commercial tool, 
%the 
%Application Programming Interfaces (APIs) of tools from Synopsys should be opened to us. %for %researchers in universities. 
%With the access to APIs, 
%we can adjust VirtualSync+ timing model by communicating with tools from Synopsys interactively to 
%fully exploit the advantages of VirtualSync+. 
%We are contacting Synopsys for the access to their APIs and hope to achieve the integration goal in the near future. 
%We have added this point in the conclusion on page 14. \\
To address the limitation above, 
either the commercial timing tools provide more flexible timing constraints for these paths or 
they allow access to the APIs. We hope the research on this topic, including our work, 
will provide more motivation to the EDA vendors to make corresponding changes in 
their timing tools in the future. 
%our hope is to access the Application Programming Interfaces (APIs) 
%of vendor tools in the future. %Currently, we are talking with Synopsys on the possibility of accessing these APIs 
%to integrate VirtualSync+ more efficiently with their tools. 
We have added this point in the conclusion on page 14. \\

%maximum/minimum delay execeptions for the paths whose endpoint is the 
%D pin of a latch or a flip-flop. 
%Accordingly, 
%the wave-pipelining paths where latches are inserted between a pair of flip-flops are not analyzed. 
%This condition restricts the 


%limits the application of latches 

%Thanks for your questions. 
%The timing characteristics of a latch is very complicated 
%when it is accommodated in the commercial tool.
%For example, 
%when a signal arrives at the input of a latch at its transparent region, 
%this signal travels through it directly with a data-to-q delay. 
%When a signal arrives at its non-transparent region, the signal 
%is blocked until an active clock level arrives.  
%With the proposed framework, 
%a latch 
%might be inserted into a circuit to block fast signals 
%while allowing slow signals to travel through it directly. 
%In the resulting optimized circuit, 
%signals might travel along a large number of combinational 
%paths to arrive at the input of a latch, either at its transparent region or non-transparent region. 
%Therefore, to accommodate a latch in a commercial tool after VirtualSync+ is applied, 
%an efficient method should be developed 
%to separate fast paths arriving at its non-transparent region 
%from slow paths arriving at its transparent region, 
%so that the corresponding timing constraints can be imposed on such paths in Design Compiler.\\

%\textbf{We have tried to accommodate latches in Design Compiler for a small circuit. The results is that ....}\\


%combinational paths before a latch might 
%need to be enumerated to evaluate whether their arrivalt times 
%are in transparent or non-transparent region, 
%so that the corresponding timing constraint can be imposed on each combinational path in Design Compiler. 


 %Due to the potential large number of combinational 
%paths, it is not possible to enumerate them.  

\textit{
(3) The reviewer wants to know how did you verify the correctness of VirtualSync+ in circuit design. It is not clear from the paper text whether it is possible to directly verify the designs after the removal of flops with a commercial verification tool. Is it possible? Were the designs from experimental results verified?
}\\ 

Thanks for your comments. In the proposed method, the critical parts of a 
circuit are first extracted for timing optimization. Afterwards, 
we removed all flip-flops in the extracted circuit and inserted delay units 
only at necessary locations to enhance timing performance. % while guaranteeing correct timing interfaces at 
%the boundary of the optimized circuits. %synchronization. 
During this process, 
we did not
%During the optimization, we inserted delay units to block fast signals instead 
remove any logic gates or revise the types of logic gates. Accordingly, 
the logic function of the optimized circuit is still maintained. \\ 

%It is 
After the application of VirtualSync+, % on the extracted critical parts, 
%possible to verify the optimized designs with a commerical verification tool  
instead of verifying the optimized circuits with a verification tool, 
%After the application of VirtualSync+ on the extracted critical parts, 
we have verified and guaranteed
correct timing interfaces to flip-flops at 
the boundary of the optimized circuits with respect to the original circuits. %referring to the timing of the origianl circuits.  
For example, in Fig. 1(d), after the removal of F6, 
we verify and guarantee that the signal from F2 arrives at F4 
after the first rising clock edge and 
before the second rising clock edge, the same with the original circuit. 
%We added this in the first paragraph in Section VII-C on page 13. 
If the timing interfaces in the
optimized circuits are correct, 
the functionality of the circuit is still maintained [19][21]. This
has been further confirmed in [24], where flip-flops are removed in a multiply-and-accumulate
unit to improve the timing performance. In this paper, the timing interface in the optimized
circuit is maintained as in the original circuit. The fabrication result demonstrates the correct
functionality of the optimized circuit. We have revised the second paragraph in the right column on page
6 and the first paragraph in Section VII-C on page 13 accordingly.\\ 

%According to the analysis above, it is not necessary to verify the optimized design with a commercial verification tool. 


\vspace{70pt}


\textbf{Reviewer: 2} \\

\textit{
Major recommendations:}\\
\vskip -5pt
\textit{
(1) The proposed flow of wave pipelining needs to be updated in a more practical aspect. Precisely, this work applied an adjusted iterative relaxation technique to the logic synthesis commercial tool (Design Compiler), where only the gate delay is considered in setting the timing constraints. However, for the logic synthesis tool alone, the delay of interconnect is just an estimation. To be robust and reliable, fully automated wave pipelining constraints in the physical synthesis stage should be retained all the way through the commercial tool of placement and routing since otherwise the wire delay at the post-route may invalidate the time constraint of wave pipelining imposed at the logic optimization step. }\\

%VirtualSync+ can accelerate timing closure by
%removing the few-picosecond timing violations at a late stage
%before which circuits have been optimized. For example,
%VirtualSync+ can improve the timing performance beyond the extreme retiming and sizing by up to 4\%,
%which is equivalenet to
%solve up to 16-picosecond timing violations.

%Thanks for your suggestions. In this manuscript, 
%we proposed an optimization framework and its 
%fine-tuning with Design Compiler to address the challenges in improving timing performance at gate level. 
%At this stage, various timing optimization methods, e.g., gate sizing and retiming, 
%can be adopted to improve the timing performance. 
%However, 
%such methods do not exploit the delay characteristics of sequential components to 
%squeeze out more timing improvement. 
%Therefore, 
%timing violations still appear after physical design,  
%so that it is difficult to achieve timing closure at a specified clock frequency. 
%Our framework provides a chance to accelerate timing closure 
%by pushing the timing performance even beyond the limit of the 
%traditional sequential designs at gate level. 
%\\
Thanks for these suggestions.
The timing performance of digital ICs has been
boosted to the level of GHz in the past decades. % which benefits from
However, such high clock frequency comes with a challenging timing closure.
For example, designers need to spend much effort to remove
picosecond timing violations to achieve timing closure [C1].
To address this challenge, 
we are %seeking a novel method to remove few-picosecond timing violations, so that timing closure can be accelerated. % to 
developing the VirtualSync+ framework in two steps. 
%accelerate timing closure. % by solving
%We plan to achieve this goal with two steps. 
The 
first step is to 
push the timing performance even beyond 
the limit of the traditional sequential designs at the gate level, %where interconnect delay are 
which 
%\spe\spb
is exactly what 
\spe\spb
we did in this work. 
According to the results, 
VirtualSync+ can improve the timing performance beyond extreme retiming and sizing by up to 4\%,
which is equivalent to
solve up to 16-picosecond timing violations at gate level. 
Such timing enhancement at gate level provides a good potential in resolving
timing violations at the physical design stage.  \\ 
%, so that timing closure can be accelerated.  \\


%There are two steps to achieve this goal,
%we first push the timing performance even beyond
%the limit of the traditional sequential designs at the gate level.
%After that


We agree with the reviewer that VirtualSync+ at physical design stage should be explored to make designs robust and reliable. 
This is exactly what we are going to do in the second step. 
At such a design stage, 
wire delays and timing violations can be annotated back to the VirtualSync+ framework to modify path specification and 
to insert delay components. In each optimization iteration, VirtualSync+ framework needs to adapt the delays 
according to the results of placement and routing. In this step, we still expect to obtain further 
improvement in timing performance because VirtualSync+ requires the delays of paths to be increased to meet the requirement of wave-pipelining 
paths. This is easier than reducing path delays in physical design. Since the content of the work on gate-level optimization has already 
obtained some results as in this manuscript, we would consider the work with physical design integration the future work of this paper. 
%timing violations between a pair of flip-flops can be solved by taking advantage 
%of virtual synchronization without flip-flops in this work. 
%To apply VirtualSync+ at physical design stage, a synergic 
%framework is required to adjust the insertion of delay units at gate level %in VirtualSync+ 
%according to the timing results after physical design, which is another work in the future.
%The challenges by applying VirtualSync+ in physcial design 
%include   
%timing violations incurred by larger delays than the specified clock period between pairs of flip-flops %than the specificied clock period 
%hinder the timing closure of sequential designs. %, which means 
%In this scenario, 
%removal of flip-flops in this manuscript can be taken advantage of 
%to relax the timing constraints between pairs of flip-flops and thus 
%solve timing violations after placement and routing. 
We have added this point in the conclusion on page 14.\\

[C1] A. B. Kahng et al., ``Timing Margin Recovery With Flexible Flip-Flop Timing Model", ISQED, 2014.
\\

%At such a design stage, various timing optimization methods can be adopted. However, 
\textit{ 
(2) The 45nm library is used in experiment, which is not the latest technology library. It would be better to show how the proposed method works under the latest technology library (28/32nm or 15nm FreePDK) and how to apply it in an environment with more diverse variations of the latest technology process node. 
}\\

%\spe\spb

Thanks for these suggestions. 
%In this revision,  
%VirtualSync+ was applied to enhance the timing performance of five circuits that have been retimed and sized extremely 
%under 
%the 15nm Nangate library. 
We have tested the VirtualSync+ framework using the 15nm Nangate library. 
Using this library, we found that the path delays in the worst case and the best case 
are about 1.2 times and 0.8 times of those 
in the typical condition. To tolerate such variations, 
the guard bands $r^u$ and $r^l$ in equations (3)-(37) were set to 1.2 and 0.8, respectively. 
Afterwards, VirtualSync+ was applied to enhance the timing performance of five circuits that have been retimed and sized extremely
under
the 15nm Nangate library. 
% to 
We compared the timing performance enhancement and area reduction
using the 15nm with those using the 45nm library. 
%The comparisons in timing performance enhancement and area reduction 
%between using 45nm library and using 15nm library are illustrated 
The comparison results are illustrated in the following figures. According to these figures, 
it is clear that the proposed method can still enhance the timing performance beyond 
that with extreme retiming and sizing using the 15nm library where diverse variations exist. Due to 
the page limit, we did not include the following figures in the revised manuscript.\\
\vskip 5.0pt
%the timing performance can still be enhanced beyond that with extreme retiming and sizing under 15nm library. \\
%\begin{figure*}
\begin{minipage}[t]{0.5\textwidth}%
%\renewcommand{\figurename}{Figure A} 
%\renewcommand{\thefigure}{}
\figurefontsize
\centering
%\vskip 9.0pt
\input{Fig/fre_cmp}
\vskip -5.0pt
\caption*{Comparison in clock period reduction between 45nm and 15nm libraries.} \nonumber%\label{fig:se_cmp}
\end{minipage}
~\hspace{10pt}
\begin{minipage}[t]{0.5\textwidth}%
%\renewcommand{\figurename}{Figure B}
%\renewcommand{\thefigure}{}
\figurefontsize
\centering
%\vskip -11.0pt
\input{Fig/area_cmp}
\vskip -5pt
\caption*{Comparison in area reduction between 45nm and 15nm libraries.}%\label{fig:buffer_replace}
\end{minipage}
%\end{figure*}
%In the experiments, we used 45nm library to demonstrate that VirtualSync+ 
%can push the timing performance even beyond the limit of the traditional sequential designs. 
%To tolerate variations, 
%a timing margin of 10\% was assigned during optimization,  
%indicating that the latest and earliest arrival times become 1.1 and 0.9 of their original values under variations. 
%Such timing margins were guaranteed during the optimization with the command ``set\_timing\_derate -late r1" and 
% ``set\_timing\_derate -early r2"
% in Design Compiler, where r1 and r2 are the derating parameters for the latest and earliest arrival times. \\
%
%We did not apply VirtualSync+ with the latest technology library due to the difficulty in accessing it. 
%However, 
%the application of VirtualSync+ does not depend on the library technologies.
%In case of large variations in the latest technology library, we 
%can increase r1 and decrease r2 for the latest arrival time and the early arrival time, respectively, 
%so that such variations can be tolerated.  
%\textbf{To demonstrate the effectiveness of VirtualSync+ under large variations, we assigned a large timing margin 20\% and applied VirtualSync+ 
%for timing optimization. The experimental 
%results demonstrate that the timing performance can still be improved beyond the traditional sequential designs. In this case, 
%the reduction of clock periods is smaller than that under small variations. } 
%We have added this analysis in the first paragraph of Section VII-A on page 11.
\vskip 15pt
\textit{ 
(3) The clock periods used in experiment should be specified in this paper. 
}\\

Thanks for pointing out this lack of clarity. We have added the clock periods of the original circuits 
in Table I and the corresponding 
description in the first paragraph of Section VII-A on page 11. 

%\vskip -5pt
%\spe\spb

\vskip 70pt

\spe\spb

\textbf{Reviewer: 3} \\

\textit{
Comments to the Author}\\
\vskip -5pt
\textit{
(1) For the circuit shown in Fig. 1(d) authors have calculated “a lower bound for the clock period as (16+1)/2=8.5”. But the path from F5 to F4 seems to have a larger delay of 9 (= 3(t\_cq)+4+1+1(t\_su)).
}\\
%\spe\spb

Thanks a lot for pointing out this. The minimum clock period of the circuit 
in Fig. 1(d) should be 9 as the reviewer mentioned. We have revised this 
in the third paragraph in the left column on page 3. 
\\


\textit{
(2) Reviewer would recommend authors to show a sample solution using VirtualSync+ for the circuit shown in Fig. 1(c) without the internal flip-flops i.e., F3, F5 and F6. It would be interesting to see how VirtualSync+ introduces flip-flops (and how many) to slow down the fast paths.
}\\ 

Thanks for your suggestion. In fact, the circuit in Fig. 1(d) is one of the solutions using VirtualSync+. In Fig. 1(d), 
F6 is removed to accelerate the slow path from F2 to F4. 
However, F5 and F3 are inserted back to slow down the fast path from F1 to F4 and to break the 
feedback loop, respectively. We have emphasized this in the third paragraph in the left column on page 3. \\ 
%\vskip 5pt

\textit{
(3) Can VirtualSync+ replace retiming and sizing? Since the proposed tool does sizing and removes the unnecessary flip-flops from a retimed circuit, why should retiming and sizing precede the invocation of VirtualSync+? It would be interesting to see, starting from an unoptimized netlist, how would a circuit optimized by VirtualSync+ compare with a circuit optimized by sizing and retiming. It would be nice to have some discussion along these lines.
}\\ 

%\vskip 10pt

Thanks for your suggestions. 
%In the past decades, the timing performance of digital ICs has been 
%boosted to the level of GHz. %, which benefits from  
%For example, a CPU can work with 3.2 GHz or even higher. 
%various timing optimization methods and the advanced manufacturing technologies.
%However, such high clock frequency comes with a tedious timing closure. 
%For example, designers need to spend much effort to remove 
%few-picosecond timing violations to achieve timing closure [27]. 
%To address such a challenge, we proposed VirtualSync+ to 
%remove the remaining timing violations in the circuits 
%that have been already optimized with retiming and sizing, so 
%that timing closure can be accelerated. 
%accelerate timing closure 
%To accelerate timing closure, 
%we proposed VirtualSync+ to %has a great potential in 
%VirtualSync+ plays a role in accelerating timing closure by 
%removing the few-picosecond timing violations 
%in the circuits that have been optimized with retiming and sizing. 
%at a late stage 
%before which circuits have been optimized. For example, 
%Therefore, VirtualSync+ can not replace retiming and sizing but further optimize circuits to deal with the remaining violations. 
%According to the results, 
%VirtualSync+ can improve the timing performance beyond the extreme retiming and sizing by up to 4\%, 
%which is equivalent to 
%solve up to 16-picosecond timing violations. 
%Therefore, %VirtualSync+ is used to solve 
%the remaining timing violations in the circuits that have already been optimized, %after circuits 
%are optimized with retiming and sizing. 
%so that it 
%VirtualSync+ cannot replace retiming and sizing but futher optimize circuits to deal with the remaining violations. %accelerate timing closure. 
%We have revised the first paragraph in the right column on page 13.
In fact, retiming and sizing are an integral part of the VirtualSync+ framework. The goal of VirtualSync+ 
is to enhance timing performance so that timing violations can be solved. Therefore, 
we first need to achieve the limit of timing performance of a circuit using retiming and sizing. VirtualSync+ 
then enhances the critical paths in the resulting designs. 
We have revised the second paragraph in the right column on page 11. 
\\


%VirtualSync+ cannot replace retiming and sizing. 
%In the proposed method, the original circuits are first retimed and sized extremely with Design Compiler.
%Afterwards,
%we apply VirtualSync+
%framework onto the optimized circuits. 
%The reason of such a sequence is that
%due to the complexity of the proposed method,
%it is used to resolve timing violations or improve timing performance at a late design stage,
%before which circuits have been optimized.
%In such a late design stage, it is very challenging
%to resolve timing violations and improve the timing performance of digital circuits.
%As demonstrated in [C1],
%achieving 1\% timing improvement at the late design stage is a big step.
%Our method can improve the timing performance by up to 4\% (average 1.5\%).
%We highlighted our method is used at a late stage in the last paragraph in the right column on page 11.\\

%\textbf{
We have also 
tried the direct optimization with VirtualSync+ on the original circuits without using retiming and sizing. 
%Since the original circuit is 
%far from a timing-balanced circuit, 
The timing enhancement with VirtualSync+ on the original circuits  
is smaller than that achieved by extreme retiming and sizing with Design Compiler,  
%since Design Compiler also does 
as illustrated in the following figure. 
The reason of this phenomenon is that 
%during retiming and sizing with 
%Design Compiler, 
Design Compiler also does 
resynthesis to optimize the circuits during retiming and sizing.  % during this process. %retiming and sizing. 
Accordingly, VirtualSync+ is not used to optimize a circuit from scratch but 
to resolve remaining timing violations in the circuits that have already been optimized. 
Due to the page limit, we did not include the following figure in the revised manuscript. 
%This also confirms that our method is used to resolve the remaining timing violations in the circuits 
%that have already been optimized instead of optimizing a circuit from scratch. 
%Since the original circuit is 
%far from a timing-balanced circuit, directly optimizing it with VirtualSync+ cannot push the timing performance beyond 
%the limit of the traditional timing paradigm. 
\\
\vskip 2.0pt
\begin{minipage}[t]{1\textwidth}%
%\renewcommand{\figurename}{Figure C}
%\renewcommand{\thefigure}{}
\figurefontsize
\centering
%\vskip 9.0pt
\input{Fig/new_cmp}
\vskip -5.0pt
\caption*{Comparison in clock period reduction between the extreme retiming and sizing with Design Compiler and 
the direct optimization 
with VirtualSync+ on the original circuits.} \nonumber%\label{fig:se_cmp}
\end{minipage}
\vskip 10.0pt
\spe\spb

\textit{
(4) Since timing model is a major novel contribution of this work and constraints (1)-(17) are integral part of the proposed model, reviewer would highly recommend some discussion around the necessity and sufficiency of these constraints. Specifically, a) which of these constraints are necessary? b) Is (17) a necessary condition for functional correctness? Is the lower bound on 
fast arrival times as established in (2) not sufficient to avoid fast signals from catching up? c) If all constraints (1)-(17) are satisfied, can functional correctness be theoretically proven?
}\\ 
%\vskip 10pt
%\spe\spb
%\spe\spb

Thanks for your comments. The constraints (1)-(17) excluding (13) are necessary to 
guarantee the correct timing interfaces and thus the correct functionality of circuits 
during the optimization with VirtualSync+.\\
%when sequential 
%delay units are inserted into circuits. \\
%determine the locations of sequential delay units 
%while guaranteeing the correctness of the functionality. \\
%(1)-(2) constraints are used to guarantee the setup and hold time of flip-flops at the boundary of the optimized circuit. 
%(3)-(4) constraints to are used to describe the timing relationship betweent the input and output arrival times of a combinational gate. 
%(5)-(15) excluding (13) constraints are used to represent the timing relationship when a sequential delay unit or no sequential delay unit is inserted. 
%(16) is used to describe the relative timing references for signal synchronization. 
%(17) is used to guarantee the next
%earliest wave should not arrive at a gate until the latest wave has propagated. \\

The lower bound on fast arrival times in (2) is not 
sufficient to avoid fast signals from catching up with slow signals, 
since 
this constraint only guarantees no hold violations of flip-flops at the boundary of the optimized circuit. 
Since we allow multiple waves to propagate along a path, 
the constraint (17) is used to guarantee the next
wave should not arrive at a gate until the previous wave has propagated through it with a gap $t_{stable}$. Therefore, 
it is a necessary condition for timing and functional correctness. We have 
emphasized this in the last paragraph in the left column on page 6. \\

In VirtualSync+, we only insert delay units at necessary locations to enhance timing performance. %to slow down fast signals while guaranteeing timing synchronization. 
During this process, 
we do not remove any logic gates or revise the types of logic gates in the optimized circuit. 
If the constraints (1)-(17) excluding (13) are satisfied, 
correct timing interfaces to flip-flops at the boundary of the optimized circuits 
are maintained after the application with VirtualSync+. 
%the timing in the optimized circuits 
%are correct, which 
In other words, signals %at boundary flip-flops 
arrive at 
%other 
boundary flip-flops at the same clock cycle as in the original circuit. 
For example, in Fig. 1(d), after F6 is removed, we still guarantee the signal at F2 arrives at F4 and F3 after 
the first rising clock edge and before the second rising clock edge. 
%In addition, we only inserted buffers and sequential delay units to slow down signals 
%and did not remove/revise any combinational gate in the optimized circuit. 
If the timing interfaces of the optimized circuits are correct, %the same with the original circuits, 
the functionality of the circuit is still maintained [19][21]. 
%In [14], they demonstrated that 
%Since we did not remove/revise any combinational gate, 
%the functionality of 
%the circuit is still maintained if the timing in the optimized circuits is the same with the original circuits. 
In [24], this concept has been confirmed with manufactured 
chips. But the method 
in [24] can only work with circuits with a given structure,  
whereas VirtualSync+ can flexibly deal with any circuit structure. 
%This has been further proven in [24], where 
%flip-flops are removed in a multiply-and-accumulate unit to improve the timing performance. 
%In this paper, the timing interface in the optimized circuit is maintained as in the original circuit.
%The fabrication result 
%demonstrates the correct functionality of the optimized circuit.  
We have revised the second paragraph %in Section IV-C(5) 
%emphasized this 
in the right column on page 6.
\\



\textit{(5) With more logic levels in the critical paths, lesser is the relative gain by removing clock-to-q delay and setup constraint. Can the reduction in clock period reported in Table 1 (column n\_t) be correlated with the logic depth of critical paths from which flip-flops were removed?
}\\
%\vskip 10pt 

Thanks for this insightful observation. 
The correlation between logic levels of the critical paths and relative gain is not obvious. 
For example, the critical paths of systemcaes, ac97\_ctrl and pci\_bridge have average logic levels of 22, 8, 12 after retiming and sizing, respectively. 
However, the percentages of their clock period reduction are 3, 1, and 1, respectively. 
The ratios between these reductions and the logic levels are thus 13.6\%, 12.5\%, 8.3\%, respectively. 
According to these ratios, no strong correlation between timing gain and the levels of critical paths can be observed. 
This is because the levels of critical paths do not represent the path delays, 
since logic gates of the same type can have different sizes and thus different delays. 
In addition, the structures of the circuits may affect the improvement of timing performance. 
For example, self-loops at flip-flops may dominate the clock period and padding short paths may affect the critical paths.  
\\
%Thanks for this insightful analysis. %We agreed with the reviewer that 
%with more logic levels in the critical paths, lesser is the gain by removing clock-to-q delay and setup constraint. 
%The reduction in clock period in Table 1 is correlated with the logic depth of critical paths to some degree. 
%The reduction of clock period in Table 1 
%is correlated with the ratio of clock-to-q delays and setup times of the removed flip-flops 
%to the delay of critical paths extracted for timing optimization. 
%With different logic levels, the delay of critical paths might be different. Accordingly, 
%we agree with the reviewer that 
%the reduction in clock period is correlated with the logic depth, as the reviewer mentioned.  
%In addition, 
%the clock period reduction 
%also depends on the structure of the circuit. For example, systemcaes, ac97\_ctrl and pci\_bridge have 
%logic levels of 22, 8, 12 after retiming and sizing, respectively. 
%Although systemcaes has a larger number of logic levels, the reduction of clock period 
%is larger than those of ac97\_ctrl and pci\_bridge. 
%This indicates that circuit structures also affect the clock period reduction with VirtualSync+.  
%We have added this analysis in the second paragraph of Section VII-B on page 12. 
%For example, 
%\\ 

\textit{
(6) Can the current formulation be modified to minimize the clock period? Even though it is mentioned that user can “quickly evaluate the benefit of VirtualSync+”, in practice, on industrial designs with at least several hundreds of thousands of gates in the critical subcircuit, it may not be practical to run VirtualSync+ several times while successively lowering the clock period until no feasible solution exists.
}\\
%\vskip 10pt
\spe\spb

Thanks for these comments. 
%It is difficult to modify the proposed formulation to minimize both clock period and the number of delay units, 
%since the insertion of delay units depends on the value of the target clock period. 
The formulation in Section IV can be modified to minimize the clock period. 
In this scenario, the clock period $T$ in the constraints in (1)-(17) excluding (13) 
becomes a variable and should be determined by the solver. 
However, 
it becomes time-consuming to solve this formulation to obtain the minimum clock period.  
%To improve execution efficiency, 
Accordingly, 
in this paper,  
we set a target clock period for timing optimization and reduce it iteratively until 
the clock period cannot be reduced anymore. 
%We have revised the second paragraph %added this point in the overall formulation in Section IV-C-(5) 
%in the right column on page 6. \\ 
We agree with the reviewer that industrial designs can contain 
hundreds of thousands of
gates in the critical subcircuit. 
This critical subcircuit is extracted by verifying the largest delays between pairs of flip-flops with respect to  a given clock period. 
Structurally, this critical subcircuit is composed of some critical parts, which can be independent or partially connected through flip-flops. 
These critical parts can be processed with VirtualSync+ by iteratively selecting a small part for timing optimization. % until 
%a target clock period is achieved. 
We have added this point in the first paragraph in the left column on page 12. 
\\



%In industrial designs with hundreds of thousands of 
%gates in the critical subcircuit, the target clock period is usually given. 
%The critical parts in the subcircuit can then be independent or connected. 
%In the former case,  
%we can apply VirtualSync+ on such critical parts in parallel, 
%so that the execution time is acceptable. 
%In the later case,  
%VirtualSync+ can enhance timing performance by iteratively  
%selecting a small part of the subcircuit for timing optimization 
%until the target timing performance is achieved. 
%We will explore the application of VirtualSync+ on large designs with 
%this iterative optimization method in the future. We have added this in the conclusion on page 14. \\
%it is still practical to run VirtualSync+ on such large designs.\\


%\spe\spb


\textit{
(7) It is mentioned that ``In practice, however, it is not easy to identify the exact locations of these units using the exact and complete model in (5)–(15) directly. To solve this problem, we relax the timing constraints (5)–(15) instead of modeling them directly'' How are constraints (18)-(21) derived from relaxing (5)-(15)? Several intermediate steps seem to be missing. Since constraints (18)-(21) are part of the proposed timing optimization problem in the relaxed VirtualSync+ flow, it would help to make the derivation more explicit. 
}\\

Thanks for the suggestions, 
In fact, we relaxed the timing constraints (5)-(15) based on 
the characteristics of delay units illustrated in Fig. 2. As shown in Fig. 2(a), a buffer slows down the propagation of  
a fast and a slow signal at its input with the same value, 
which is the buffer delay. However, sequential delay units slow down fast and slow signals with different values. For example, 
no matter when fast and slow signals arrive at the input of a flip-flop, they leave the output of the flip-flop at the same time. This 
indicates that a flip-flop slows down fast signals with a larger delay than slow signals. 
When a fast signal and a slow signal arrive at the input of a latch when it is non-transparent and transparent, respectively, 
a latch also 
slows down the fast signal with a larger delay than the slow signal. 
According to this analysis, 
for a sequential delay unit, no matter it is a flip-flop or latch, it delays fast and slow signals with different values. 
With this characteristics, in (18)-(21), we use two variables $\delta_{wt}$ and $\delta_{wt}^\prime$ 
to emulate that a sequential delay unit can delay slow and fast signals differently. 
In case $\delta_{wt} = \delta_{wt}^\prime$, a buffer is inserted. If $\delta_{wt} < \delta_{wt}^\prime$, 
a sequential delay unit is inserted. 
%$\delta_{wt} \le \delta_{wt}^\prime$ since the fast signals should be delayed with a larger value than slow signals. 
We have revised the first paragraph in the left column on page 7.
\\


\textit{
(8) Constraint (21) is not clear. If the purpose of (21) is to specify 
``that the arrival time of the fast signal should not exceed the arrival time of the slow signal after padding'', 
then why not formulate it as ``$s_z^\prime \le s_z$''?
}\\

Thanks for pointing out this lack of clarity.
The purpose of (21) is not to specify that 
the arrival time of the fast signal should not exceed the arrival time of the slow signal after padding. 
Instead, the purpose of (21) is to 
%guarantee that a sequential delay unit is required to be inserted to break a feedback loop. 
avoid the case where 
no sequential delay is required to be inserted into a feedback loop. 
%which is not 
%true since sequential delay units are 
%absolutely required to break feedback loops. 
%If we use $s_z^\prime \le s_z$ to replace (21),
%there might be a possibility that
%no sequential delay is required to be inserted into the circuits,
%which is not 
%true since sequential delay units are 
%absolutely required to break feedback loops. 
For example, assume that there is a feedback loop where $s_u$ is larger than $s_u^\prime$.  
%Without the constraint (21), 
If we only use the constraints (18)-(20), we  
might obtain $\delta_{wt}^\prime = \delta_{wt}$, 
since the same values of $\delta_{wt}^\prime$ and $\delta_{wt}$ make (18)-(20) valid. 
$\delta_{wt}^\prime = \delta_{wt}$ indicates that a buffer is inserted along this loop. 
Instead, by including the constraint (21), $\delta_{wt}^\prime > \delta_{wt}$ is obtained due to $s_u> s_u^\prime$, 
which indicates a sequential delay unit is inserted to break this loop.  
%In this case, if $s_z^\prime \le s_z$ and (18)-(21) are used to constrain the paths along this loop,  
%$\delta_{wt}$ might be the same with $\delta_{wt}^\prime$ since their same values make the constraints (18)-(21) valid. 
%Accordingly, %so that 
%no sequential delay units can be inserted into a feedback loop. 
%On the contrary, %in (21), we strictly guaranteed that 
% different $\delta_{wt}^\prime$ and $\delta_{wt}$ are generated with (21), 
%leading to an insertion of a sequential delay unit to break the feedback loop.
%Therefore, (21) is used to avoid that no sequential delay unit is required to break a feedback loop 
%and cannot be replaced with $s_z^\prime \le s_z$. 
We have added this point in the first paragraph in the left column on page 7.\\ 

%Considering a guard band reserved for process variations, the delays of the buffer and the gate 
%are increased by $r^u$ and decreased by $r^l$, 
%set to 1.1 and 0.9 in the experiments. %If 
%Therefore, the reasons leading to ``$s_z^\prime \le s_z$'' includes two aspects. 
%First, the amplfication and minification on the delay with $r^u$ and $r^l$, respectively. 
%Second, the larger and smaller delays are added on fast and slow paths, respectively. 
%According to this analysis, ``$s_z^\prime \le s_z$''does not strictly constrain 
%the relationship between early and late arrival times after insertion of a sequential delay unit. 
%the constraint in (21) has a strong effect than ``$s_z^\prime \le s_z$''. 
%\\
%\vskip 10pt
\spe\spb

\textit{
(9) The optimization problem mentioned in (22)-(24) would definitely benefit from more explanation. 
Firstly, it was mentioned earlier that the optimization objective is to reduce area, and the objective (22) has three terms in it. 
How do the first two terms of (22) relate to area reduction? Why are they in the objective? Secondly, 
why the second term in (22) has delta\_wt’ (delay padding by sequential gate) when the second term is supposed to be related to the delay due to inserted buffers? Thirdly, how are the combinational gate delays, mentioned in the third term in (22), modeled? Fourthly, what are all the variables in (22)-(24)?
}\\
%\vskip 10pt

Thanks for pointing out this lack of clarity.  
It is difficult to represent the area of components in the optimization objective exactly. Therefore, 
we approximate the area of these components as follows. 
In (22), a nonzero value of $\delta_{wt}^\prime-\delta_{wt}$ represents that  
sequential delay units are inserted between w and t. The larger the value of $\delta_{wt}^\prime-\delta_{wt}$ is, 
more sequential delay units are potentially inserted. 
%potentially the larger the number of inserted sequential delay units is. 
$\delta_{wt}^\prime+\xi_{uv}$ represents that buffers are inserted between w and t.  
The larger this value is, more buffers are potentially inserted. %potentially the larger the number of buffers is. 
%$\delta_{wt}^\prime-\delta_{wt}$ roughly represents the number of inserted sequential delay units.  
Therefore, $\delta_{wt}^\prime-\delta_{wt}$ and $\delta_{wt}^\prime+\xi_{uv}$
approximately represent the number of inserted sequential
delay units, e.g., flip-flops,
and the number of inserted buffers, respectively. 
The numbers of inserted sequential
delay units and buffers are correlated with their areas, so that 
 $\delta_{wt}^\prime-\delta_{wt}$ and $\delta_{wt}^\prime+\xi_{uv}$
approximately represent the area of inserted sequential
delay units, e.g., flip-flops,
and the area of the inserted buffers, respectively. 
The combinational gate delay is represented with $d_{vw}$ in (22). A larger delay of a
combinational gate indicates a smaller area. Accordingly, 
$d_{vw}$ inversely represents the area of a logic gate approximately. % we maximize the sum of all combinational gate delays in (22).
% and the logic gates after sizing.
%Since the
%area of a buffer is roughly the average area of logic gates,
%we set the ratio of $\beta$ to $\gamma$ to 1. % respectively.
%We set %the ratio of $\alpha$ to
%$\beta$ and the ratio of $\alpha$ to
%$\gamma$ 
%both $\alpha/\beta$ and $\alpha/\gamma$ 
%to 10 because the area of a flip-flop is
%about 6 times of the area of a buffer and the average area of logic gates,respectively. 
We set both $\alpha/\beta$ and $\alpha/\gamma$
to
10
because the area
of a flip-flop is
about 5.6 times of the area of a buffer and 4.4 times of the average area of combinational gates, respectively.
The motivation of using 10 instead of 5.6 or 4.4 is that
we also intend to improve the execution efficiency of
the formulation (22)-(24) with an integer linear programming solver. 
With this setting, we provide the solver a clear tendency to 
minimize the area of sequential delay units, buffers and logic gates with different 
priorities. We have revised the last paragraph in the left column on page 7. \\

The second term in (22) has $\delta_{wt}^\prime$ because it potentially represents an insertion of a buffer. 
For example, 
in case of $\delta_{wt}^\prime = \delta_{wt}$, a buffer instead of a sequential delay unit is inserted. 
%we have added this explanation in the first paragraph in the right column on page 7. 
%\\
%The combinational gate delays are represented with $d_{vw}$ in (22). Since a larger delay of a 
%combinational gate indicates a smaller area, we maximize the sum of all combinational gate delays in (22). 
%We set the ratio of $\alpha$ to
%$\gamma$ to 10 because the area of a flip-flop is
%about 6 times of the area of a buffer. 
We have added this explanation in the first paragraph in the right column on page 7.
\\

In (22)-(24), $\alpha$, $\beta$ and $\gamma$ are coefficients to balance the area of sequential delay units, 
the area of buffers and the area of logic gates. $G$ is the set of all logic gates. 
$\delta_{wt}^\prime$ and $\delta_{wt}$ are two variables representing the delays padded to fast and slow paths, respectively. 
$\xi_{uv}$ is the extra delay introduced by inserted buffers. $d_{vw}$ is the pin-to-pin delay of the logic gate. 
We have highlighted their explanations in the fourth paragraph 
in the left column on page 5 and in the last paragraph in the left column page 7, respectively. 
\\


\textit{
(10) In the optimization problem mentioned in (27)-(31), 
why is the number of delay units inserted (sum of x\_wt over each gate in S) not part of the objective function (27)? Since the goal is to reduce area, insertion of delay units must be minimized.
}\\

%Thanks for pointing out this lack of clarity. 
The goal of the objective function (27) is to minimize the number of inserted delay units to reduce area. 
This goal can be achieved by minimizing the sum of $x_{wt}$, as the reviewer mentioned.   
Minimizing $\delta_{wt}^\prime-\delta_{wt}$ as written in (27) in the revised manuscript  
can also achieve this goal. 
The reason is that a nonzero value of $\delta_{wt}^\prime-\delta_{wt}$ represents that
sequential delay units are inserted between w and t and the larger the value of $\delta_{wt}^\prime-\delta_{wt}$ is,
the more sequential delay units are potentially inserted. 
$\delta_{wt}^\prime-\delta_{wt}$ instead $x_{wt}$ was used in the objective function (27) 
since it is more efficient for the ILP solver 
to minimize a continuous variable $\delta_{wt}^\prime-\delta_{wt}$ compared with minimizing a binary variable $x_{wt}$. 
%This goal can also be achieved by minimizing 
%minimizing the sum of $x_{wt}$ is equivalent to minimize 
%$\delta_{wt}^\prime-\delta_{wt}$, 
%since 
%$\delta_{wt}^\prime-\delta_{wt}$ approximately represents the number of inserted sequential delay units. 
%%a non-zero value of $\delta_{wt}^\prime-\delta_{wt}$ also represents
%the existence of sequential delays. Accordingly, in the optimization problem (27)-(31), 
%we use $\delta_{wt}^\prime-\delta_{wt}$ to  
\\

%\vskip 10pt


\textit{
Minor recommendations:}\\
\vskip -5pt

\textit{
(1) Unlike wave-pipelining, many of the previous works cited for timing analysis and sizing do not seem relevant here. 
For example, [10], as authors say, presents GPU accelerated static timing analysis. 
Runtime of static timing analysis does not seem to form a discussion in this manuscript, 
then why include such references? Furthermore, one liner generic description}
\spe\spb

\textit{
for works like [6,7] does not add any value to the content. On sizing, a lot of papers have been published in over more than three decades. Why have authors chosen [11-15] to cite? Again, there are only one-line descriptions about each one of them without highlighting their relevance to this work. 
}\\



%Thanks for pointing out this lack of clarity. 
We introduced the existing work
on timing analysis and timing optimization, e.g., sizing and retiming,  
since timing analysis and timing optimization are the background of 
this work. For references on gate sizing, [11-15] were selected because they 
describe the typical methods in gate sizing, Lagrangian Relaxation-based method and sensitivity-based method. \\


We agree with the reviewer that some references, e.g., [10], are not so relevant in this manuscript since 
we do not focus on the runtime of timing analysis. 
Therefore, we removed this reference. We also 
summarized the previous work on timing analysis and timing optimization 
briefly and highlighted their relevance to this work  
in the second paragraph on page 1.\\  

%We include the references on timing analysis such as [10] %for the following reason. 
%because the optimized circuits with VirtualSync+ also require efficient and accurate timing analysis. 
%In the proposed method, 
%the critical parts of a circuit are extracted for optimization. 
%If such critical paths are isolated, 
%we could 
%optimize each part individually and analyze their timing performance in parallel. In such scenario, we could 
%adopt the methods in the references such as GPU-based acceleration in [10].  
%We still agree with the reviewer that runtime of static timing analysis is not so relevant in this manuscript. 
%Therefore, we removed the references and their descriptions on timing analysis in the attached manuscript. \\

%In this manuscript, 
%we would like to optimize the timing performance of digital circuits with virtual synchronization. 
%Since the existing timing optimization methods include gate sizing, retiming and wave-pipelining, 
%we reviewed the relevant work on them. 
%For references on gate sizing, [11-15] were selected because they 
%described the typical methods in gate sizing, Lagrangian Relaxation-based method and sensitivity-based method. 
%We added this explanation and their relevance to this work in the right column on page 1.
%\\

\textit{ 
(2) Even though authors have mentioned that ``wave-pipelining paths are different from multi-cycle path'', multi-cycle path still seems quite relevant here because by removing the sequential gates, authors are essentially generating multi-cycle paths. Reviewer would recommend the authors to include some of the previous works that analyze timing for multi-cycle paths and discuss 1) how timing constraints have been derived for multi-cycle paths, 2) why multi-cycle path timing constraints cannot be extended to allow multiple logic wave propagation along a path, 3) how their proposed timing constraints differ from multi-cycle path constraints, etc. 
}\\

%Thanks for your comments.
%After a flip-flop is removed,
%wave-pipelining paths instead of multi-cycle paths are generated. 
%For example,
%in Fig. 1(d), the path from F2 to F4 is wave-pipelining %since F6 is removed.
%New data is injected into this path by F2 at each rising clock edge,
%so that
%two data waves propagate along this path without a flip-flop separating them after the first rising edge.


%\spe\spb

Thanks for the comments. 
After a flip-flop is removed, 
wave-pipelining paths instead of multi-cycle paths are generated.   
For example, 
in Fig. 1(d), the path from F2 to F4 is wave-pipelining since F6 is removed. 
New data is injected into this path by F2 at each rising clock edge, 
so that 
two data waves propagate along this path without a flip-flop separating them. % after the first rising edge. 
%At each rising clock edge, new 
%data is injected into the combinational path by flip-flop F2, 
%the two data waves along this path 
%are always separated by one clock period initially. 
To guarantee that the second data wave does not flush 
the first data wave when it is waiting for the second 
rising clock edge to be latched by F4, 
the path delay between F2 and F4 should be larger than one clock period. 
In addition, the path delay should be 
smaller than two clock periods to allow the first data wave to arrive at F4 before the second rising clock edge. 
Specifically, the delay of the path from F2 to F4 should be smaller than $2*T-t_{su}$ 
and larger than $T+t_h$,  where 
$T$ is clock period, $t_{su}$ and $t_h$ are the setup time and hold time of F4. \\

For a multi-cycle path, new data is injected into the path every $N*T$ time, where $N$ is the number of clock cycles. 
Accordingly, there is only one data wave propagating on it.
% which 
%means that new data is injected into the path every $N*T$ time, where $N$ is the number of clock cycles. 
The timing constraint is 
that the delay of this path should be smaller than $N*T-t_{su}$ [17, 18].
Therefore, multi-cycle paths are different from wave-pipelining paths and they 
cannot be extended to allow multiple logic waves propagating along them. 
We have added a sentence to explain their differences in timing in the third paragraph in the right column on page 1.\\
%Due to the page limit, we did not add discussion on the differences between wave-pipelining paths 
%and multi-cycle paths in this manuscript. \\

%[C1] A.P. Gupta; D.P. Siewiorek, ``Automated multi-cycle symbolic timing verification of microprocessor-based designs", DAC, 1994.
%[C2] H. Higuchi, ``An implication-based method to detect multi-cycle paths in large sequential circuits", DAC, 2002. 
%\\


\textit{ 
(3) Page 3: ``F3 in Fig. 1(b) simply blocks the fast path from F1 to F4”. This is not entirely true. Even if F1 to F4 happened to be a slow path, F3 would still be needed to break the fast feedback loop.
}\\

Thanks for pointing this out. We agree with the reviewer that F3 is still needed to break the fast feedback loop 
besides blocking the fast path from F1 to F4. 
We have revised the fourth paragraph in the left column on page 3 accordingly.\\


\textit{ 
(4) What does integer variable N\_wt signify? Does it tell the number of sequential delay units between w and t? Can there be multiple consecutive delay units? If yes, what purpose would the second delay unit serve when both fast and slow signals are arriving at its input at the same time? While formulating constraints (7) and (8), its mentioned that solver determines this variable, without any discussion anywhere else.
}\\
\spe\spb
In (7)-(15), $N_{wt}$ is an integer variable whose value is determined by a solver. 
This variable does not represent the number of sequential delay units between w and t. 
%Due to the removal of flip-flops,  
Instead, it represents that in VirtualSync+ model, 
the signal arrival time at the input of an inserted sequential delay unit 
can be within any clock cycle, 
the starting and ending time of which are $N_{wt}*T$ and $(N_{wt}+1)*T$, 
respectively. 
%This flexibility results from the the removal of flip-flops in VirtualSync+. 
%This property is different from the traditional timing paradigm, where the start and time 
%of a signal arrival time should be between $0$ and $T$. 
%In addition, the output of an inserted sequential delay unit 
%can start with any number of clock cycles in VirutalSync+ framework. 
%For example, 
%in Fig. 3, we assume that F2 and F3 are removed and 
%a flip-flop is inserted at $u$. Since the input arrival time of 
%the inserted flip-flop is 14,   
%the arrival time of the signal at the output of the inserted flip-flop becomes 
%$1*T+4+3$, where $T$ is the clock period of 10 and the clock-to-q delay is 3. 
%at $t$ is $s_t=3+11-T+3-T=-2*T+3+11+3$, where $T$ is the clock period. 
%We can see that in this case, $N$ is 1 to match the signal arrival time at the output of the inserted flip-flop. %We have revised the sentence in the left column on page 6. 
%For example, along a path where several flip-flops are removed, 
%if a flip-flop is inserted along the sink of this path, 
%the arrival time at the input of the inserted flip-flop might be negative, which leads
%to a negative $N_{wt}$.
%The only constraint for $N_{wt}$ is that the type of this variable should be integer.
%According to this analysis, 
%there is no
%additional constraints for $N_{wt}$ in the optimization formulation.
This property is different from the traditional timing paradigm, where the starting and ending time     
of a signal arrival time should be between $0$ and $T$.
We have revised the text below the equation (8) on page 5, accordingly.\\


\textit{ 
(5) What is the value of t\_stable, mentioned in constraint (17), used in the experiments?
}\\

Thanks for pointing out this lack of clarity. 
The purpose of (17) is to guarantee that 
%the signal of the next wave starting 
%from a boundary flip-flop never catches the signal of the previous wave starting from the 
%Since 
the next wave should not arrive at a gate until the previous wave has propagated through it.  
$t_{stable}$ in (17) is the minimum time that a signal must be stable 
to correctly propagate through the gate. 
It is set to the delay of a buffer in the experiments since a buffer consists of two inverters 
and such two inverters can isolate the signals of the next wave and the previous wave. 
We have added the value of $t_{stable}$ in the experiments in the first paragraph of Section VII-A on page 11.
\\

\textit{ 
(6) Do all the constraints mentioned in case1 (5-6), case2 (7-10) and case3 (11,12,14,15) 
need be satisfied simultaneously? If a flip-flop gets inserted between w and t,
then only (7-10) 
They look more like ``either-or'' constraints rather than ``and'' constraints. 
If reviewer is correct in their understanding, 
then including (5)-(12) and (14)-(16) in the optimization problem (32)-(36) over-constrains the problem.
}\\

%\spe\spb

%need be satisfied simultaneously? If a flip-flop gets inserted between w and t, 
%then only (7-10) 
%should be satisfied. 
%They look more like `either-or'' constraints rather than `and'' constraints. 
%If reviewer is correct in their understanding, 
%then including (5)-(12) and (14)-(16) in the optimization problem (32)-(36) over-constrains the problem.\\

Thanks a lot for the comments. 
We agree with the reviewer that the constraints (5-6), (7-10) and (11-12,14-15) have 
an ``either-or" instead of ``and" relationship. 
In the optimization problem (33)-(37), we realize this ``either-or" relationship with ``if else" condition. 
For example, if there is a flip-flop inserted, the constraints (7-10) are valid and other constraints are invalid. 
Such ``if else" condition can be converted into equivalent linear forms according to [25], so that the 
overall formulation is still an integer linear programming problem. 
We have added this point in the first paragraph of Section IV-C(2) on page 5.\\

%[C1] Gurobi Optimization, Inc., “Gurobi optimizer reference manual,” 2013.
%[Online]. Available: http://www.gurobi.com


\textit{
Typo/nit-picks:}\\

\textit{ 
(1) Page 2: MIG acronym is defined but never used.
}\\

We have removed this acronym. \\ 

\textit{ 
(2) Page 2: ``that interacting with commercial'' should be ``that interacts with commercial''.
}\\

%Thanks for pointing out this grammar error. 
We have revised this sentence accordingly.\\ %in the first paragraph in the left column on page 2. \\
%\vskip 5pt

\textit{ 
(3) Page 3: ``the essential function of sequential components is to delay signals along fast paths in a circuit''. 
That does not sound right. Traditionally, sequential components are used to break long paths to reduce the clock period. 
Authors may want to re-word this sentence as ``We propose that the essential function..''
}\\

Thanks for the suggestion. We have revised this sentence in the first paragraph of Section III on page 3.\\

\textit{ 
(4) In Fig. 2(b-c), for the sake of completeness, 
authors may want to show the graph for input arrival time after T+t\_h. 
}\\

Thanks for pointing out this lack of clarity. In Fig. 2(b-c), 
we would like to show the input arrival time $s_u$ larger than $0+t_h$ and smaller than $T-t_{su}$, since 
we assume that the launching and capturing times of an active clock edge are 0 and $T$, respectively. 
The graph for input arrival time after $T+t\_h$ repeats that between $0+t_h$ and $T-t_{su}$, as shown in Fig. 2(b-c). 
%The graph for input arrival time after $T+t\_h$ is the same with the Fig. 2(b-c).
We have revise the caption of Fig.2 in the left column on page 4. \\
%\vskip 5pt

\spe\spb

\textit{ 
(5) Page 6: ``The model to insert these delay units automatically will be'' can be reworded as 
``The model to automatically insert these delay units will be''.
}\\

%Thanks for your suggestion. 
We have revised this sentence accordingly. Thanks. \\%in the first paragraph in the left column on page 5. \\

%\vskip 5pt

\textit{ 
(6) Page 6: ``between w and t in the original circuit'' should be ``between t and z in the original circuit''.
}\\

Thanks for pointing out this error. We have revised this sentence. \\ % in the third paragraph in the left column on page 5.\\

%\vskip 5pt
\textit{ 
(7) Page 6: ``might be be different'' should be ``might be different''.
}\\

We have revised this accordingly. Many thanks. \\ %in the last paragraph in the left column on page 5. 
\vskip 100pt

\textbf{Reviewer: 4} \\

\textit{
Comments to the Author}\\
\vskip -5pt

\textit{ 
The main difficulty I faced when reviewing the paper is that there is a lack of an overview of the approach.  If there is an overview of the major components of the methodology, it would be a lot easier to follow the paper.  Similarly, an overview of each major component would greatly assist a reader.  In fact, I would suggest that you present the overall method without a specific commercial tool.  After that, provide a section to show how the method can be modified to work with a commercial too. 
}\\

Thanks for the suggestions. 
Section IV-V of this paper presents the overall method and Section VI demonstrates the fine-tuning of the results using commercial tools. 
We have added an overview of the proposed method in the last paragraph in Section III on page 3. \\

\textit{Step 1:  Section V.A: Are delta\_wt and delta'\_wt non-negative?  Is it important to impose that constraint in the formulation (22)-(24).  How do you determine alpha, beta, and gamma (100, 10, and 10)?
}\\

Thanks for pointing out this lack of clarity. 
$\delta_{wt}$ and $\delta^\prime_{wt}$ are non-negative 
since they are used to emulate non-negative delays. We have 
revised the sentence in the first paragraph in the left column on page 7 and (20). 
This constraint is important and necessary 
in the formulation (22)-(24). Without this constraint, the formulation (22)-(24) 
cannot accurately identify the locations of inserted sequential delay units. \\


In (22), a nonzero value of $\delta_{wt}^\prime-\delta_{wt}$ represents that
sequential delay units are inserted between w and t. The larger the value of $\delta_{wt}^\prime-\delta_{wt}$ is,
more sequential delay units are potentially inserted.
%potentially the larger the number of inserted sequential delay units is. 
$\delta_{wt}^\prime+\xi_{uv}$ represents that buffers are inserted between w and t.
The larger this value is, more buffers are potentially inserted. %potentially the larger the number of buffers is. 
%$\delta_{wt}^\prime-\delta_{wt}$ roughly represents the number of inserted sequential delay units.  
%$d_{vw}$ represents the delays of the combinational gates. The larger this value is, the smaller the area is. 
Therefore, $\delta_{wt}^\prime-\delta_{wt}$ and $\delta_{wt}^\prime+\xi_{uv}$ 
approximately represent the number of inserted sequential
delay units, e.g., flip-flops,
and the number of inserted buffers, respectively.
The numbers of inserted sequential
delay units and buffers are correlated with their areas, so that
 $\delta_{wt}^\prime-\delta_{wt}$ and $\delta_{wt}^\prime+\xi_{uv}$
approximately represent the area of inserted sequential
delay units %, e.g., flip-flops,
and the area of the inserted buffers, respectively.
$d_{vw}$ represents the delay of the combinational gate after sizing. The larger this value is, the smaller the area is. 
Accordingly, $d_{vw}$ inversely represents the area of a combinational gate approximately. 
% and the logic gates after sizing.
%Since the
%area of a buffer is roughly the average area of logic gates,
%we set the ratio of $\beta$ to $\gamma$ to 1. % respectively.
We set both $\alpha/\beta$ 
\spe\spb 
and $\alpha/\gamma$
to 
10 
because the area 
of a flip-flop is
about 5.6 times of the area of a buffer and 4.4 times of the average area of combinational gates, respectively. 
The motivation of using 10 instead of 5.6 or 4.4 is that
we also intend to improve the execution efficiency of
the formulation (22)-(24) with an integer linear programming solver. % since 
A larger ratio provides the solver a clear tendency in reducing the number of inserted sequential delay units. 
%With this setting, we provide the solver a clear tendency to minimize the area of sequential delay units, buffers and combinational gates with different
%priorities. 
We have revised the first paragraph in the right column on page 7. \\

%In (22), $\delta_{wt}^\prime-\delta_{wt}$, $\delta_{wt}^\prime+\xi_{uv}$ 
%and $d_{vw}$ roughly represent the area of inserted sequential 
%delay units, e.g., a flip-flop, 
%the inserted buffers and the logic gates after sizing. 
%Since the 
%area of a buffer is roughly the average area of logic gates, 
%we set the ratio of $\beta$ to $\gamma$ to 1. % respectively.
%Since the area of a flip-flop is 
%about 6 times of the area of a buffer and the 
%area of a buffer is about the average area of logic gates, 
%We set the ratio of $\alpha$ to 
%$\beta$ to 10 because the area of a flip-flop is 
%about 6 times of the area of a buffer. 
%Another reason is %to set the ratio of $\alpha$ to 
%$\beta$ to 10 is 
%With a number larger than 6, 
%The motivation of using 10 instead of 6 is that 
%we also intend to improve the execution efficiency of 
%the formulation (22)-(24) with an inter linear programming solver. % since 
%A larger ratio provides the solver a clear tendency in reducing the number of inserted sequential delay units. %inserting sequential delay units. 
%We have revised the first paragraph in the right column on page 7.\\

%we also %intend to reduce 
%the complexity of timing analysis in fine-tuning circuits with Design Compiler 
%by further reducing 
%the number of inserted sequential delay units. \\
%so that the complexity of timing analysis in fine-tuning circuits with Design Compiler can be reduced. \\
%\spe\spb


\textit{ 
Section V.B:  Do you meet the requirement that delta'\_wt - delta\_wt = 0 before you terminate the second substep?  If you can always meet that requirement, why decrease the bound on the difference?  Should the bounds be part of the formulation (27)-(31)?
}\\


Yes. 
The requirement that $\delta_{wt}^\prime-\delta_{wt}=0$ is met before the second substep is terminated. 
We iteratively decrease the bound on 
the difference between $\delta_{wt}^\prime$ and $\delta_{wt}$ 
to improve the execution efficiency of this formulation. 
Since the formulation (27)-(31) is executed for several iterations until 
no difference between $\delta_{wt}^\prime$  and $\delta_{wt}$ exists,    
a large bound of $\delta_{wt}^\prime-\delta_{wt}$ in the early iterations allows 
the solver to quickly determine the important locations for inserting sequential delay units. 
The bounds should be part of the formulation (27)-(31). 
Thanks for pointing this out. %.that the bounds should be part of the formulation (27)-(31).  
We have added this bound in equation (32) and its description in the right column on page 7 and in the first paragraph of Section VII-A on page 11. \\
  
%For example, in the first iteration, the lower bound of $\delta_{wt}^\prime-\delta_{wt}$ 
%is 

\textit{ 
Does G/S mean G or S or do you actually want to say G minus S, which is G$\backslash S$ (backslash)?  The cost of sequential elements is not accounted for in formulation (27)-(31).  Why?
}\\

Thanks for pointing this out. We actually want to say G minus S. We have revised constraints (28) and (34) on page 7 and page 8, respectively. \\

The area cost of sequential elements has been accounted for in formulation (27)-(32). 
As explained in the second question from the reviewer above, 
in (27), $\delta_{wt}^\prime-\delta_{wt}$, $\delta_{wt}^\prime+\xi_{uv}$
and $d_{vw}$ approximately represents the area of inserted sequential
delay units, 
the inserted buffers, and the logic gate after sizing, respectively.
Since the area of a flip-flop is
about 5.6 times of the area of a buffer and is 4.4 times of the average area of logic gates, 
We set both $\alpha/\beta$ and $\alpha/\gamma$
to 10. 
%we set the ratio of $\alpha$ to
%$\beta$ and the ratio of $\alpha$ to $\gamma$ to 10. 
Accordingly,  
the reduction of the number of sequential delay units has a higher priority when a solver solves this formulation.  
We have revised the first paragraph in the right column on page 7.\\



\textit{ 
Section V.C:  What is the difference between S and S\_d?  
Is S\_d larger than S or smaller than S?  My interpretation is that you have a sequential element only when delta' and delta are different.  
Since you terminate with the difference being 0, S should be the same as S\_d, unless you update S in the second substep (Section V.B).  
However, I did not see that.  Moreover, the paper mentioned that some locations in S\_d may be invalidated.  
Does S\_d reduce in size or you may also add gates into S\_d?
}\\

Thanks for pointing out this lack of clarity. $S$ contains the potential locations of sequential delay
units obtained with the formulation (22)-(24), 
where the existence of sequential delay units is approximately represented with the non-zero value of $\delta_{wt}^\prime-\delta_{wt}$. 
The approximation in (22)-(24) makes $S$ inaccurate 
since it does not model the accurate timing of sequential delay units in (7)-(15) excluding (13). 
 To 
refine the locations of sequential delay units in $S$, 
we consider the clock-to-q delays of 
flip-flops and data-to-q delays of latches in the formulation (27)-(32). 
Therefore, the obtained locations $S_d$ of sequential delay units are more accurate than $S$. 
Since some locations in $S$ might be invalid and removed after the clock-to-q delay and data-to-q delay 
are considered in (27)-(32), the size of $S_d$ might be smaller than $S$. 
%However, 
%besides the refinement of $S$ in the formulation (27)-(32), 
%Due to the removal of some invalid locations when the formulation (27)-(32) is solved, 
However, %&%after solving the formulation (27)-(32), 
new potential locations of sequential delay units might also be identified and are 
added in $S_d$ after solving the formulation (27)-(32) iteratively. \\
%Since $S_d$ also includes locations that are not in $S$, 
%Therefore, 
%it is difficult to compare the sizes of $S$ and $S_d$. \\
%We have revised the second paragraph in the left column on page 8. \\

$S_d$ is identified with the formulation (27)-(32) where only the clock-to-q delays of
flip-flops and data-to-q delays of latches are considered. However, 
the complete timing model of flip-flops and latches in (7)-(15) excluding (13) is not considered. 
Instead, this complete 
timing  
model is approximated by only considering the delays of sequential delay units.  %the clock-to-q delays of flip-flops and the 
%data-to-q delays of latches.  
Therefore, 
\spe\spb
some locations 
in $S_d$ may be invalidated after solving the formulation (33)-(37) and $S_d$ reduces in size. 
We have revised the third paragraph in the left column on page 8. \\
%We have added this point in the left column on page 8.\\


\textit{ 
Step 2: Removal of flip-flops.  In Section VI.B, it is not clear when you applied re-timing.  Do you performing retiming, and then removal, or is the retiming and removal performed together?  If it is the former, what was the formulation:  min area-retiming subject to performance constraint, performance optimization with area constraint, or simply performance optimization?  Does the starting point affect the quality of the final solution?  If it is latter, it would be nice to have a complete formulation presented.
}\\


Thanks for pointing out this lack of clarity. We perform retiming and removal together in Section VI.B. 
We have added a complete formulation in the last paragraph in the right column on page 9.\\


\textit{ 
Experimental results:  If the paper starts with the original circuit, how much improvement in performance can it achieve?  The results reported seem to assume circuits that already meet the performance requirement.  The objective appears to be maintaining performance (or improve performance slightly).  For example, in Fig. 14, I do not see marked improvement in performance.
}\\

%In the proposed method, the original circuits are first retimed and sized extremely with Design Compiler. 
%Afterwards,  
%we apply VirtualSync+ 
%framework onto the optimized circuits. % that are retimed and sized extremely on the original circuits. 
%The reason of such a sequence is that 
%due to the complexity of the proposed method, 
%it is used to resolve timing violations or improve timing performance at a late design stage, 
%before which circuits have been optimized. 
%%As the reviewers mentioned that there is no marked improvement in performance. 
%In such a late design stage, it is very challenging 
%to resolve timing violations and improve the timing performance of digital circuits. 
%As demonstrated in [C1], 
%achieving 1\% timing improvement at the late design stage is a big step. 
%Our method can improve the timing performance by up to 4\% (average 1.5\%). 
%This is also why the reviewer did not see marked improvement in performance in Fig. 14. 
%We highlighted our method is used at a late stage in the right column on page 13.  


Thanks for the comments. 
%In the past decades, the timing performance of digital ICs has been
%boosted to the level of GHz. %, which benefits from  
%For example, a CPU can work with 3.2 GHz or even higher. 
%various timing optimization methods and the advanced manufacturing technologies.
%However, such high clock frequency comes with a tedious timing closure.
%For example, designers need to spend much effort to remove
%few-picosecond timing violations to achieve timing closure [27].
%To address such a challenge, we proposed 
VirtualSync+ enhances a circuit that is already optimized using retiming and sizing to
remove the remaining timing violations. % in the circuits
This is a challenging task in modern IC design where the effort to remove timing violations of a few picosecond is already high [27]. 
%that have been already optimized with retiming and sizing, so
%that timing closure can be accelerated.
%accelerate timing closure 
%To accelerate timing closure, 
%we proposed VirtualSync+ to %has a great potential in 
%VirtualSync+ plays a role in accelerating timing closure by 
%removing the few-picosecond timing violations 
%in the circuits that have been optimized with retiming and sizing. 
%at a late stage 
%before which circuits have been optimized. For example, 
%Therefore, VirtualSync+ is used to futher optimize circuits to deal with the remaining violations.
According to the results,
VirtualSync+ can improve the timing performance beyond the extreme retiming and sizing by up to 4\%,
which is equivalent to
address up to 16-picosecond timing violations. 
This is  why the reviewer did not see marked improvement in performance in Fig. 14 (now Fig. 15).\\

We have also 
tried the direct optimization of the original circuit with VirtualSync+. 
%Since the original circuit is 
%far from a timing-balanced circuit, 
The timing enhancement with VirtualSync+ on the original circuit 
is smaller than that achieved by extreme retiming and sizing with Design Compiler,  
%since Design Compiler also does 
as illustrated in the following figure. 
The reason of this phenomenon is that 
%during retiming and sizing with 
%Design Compiler, 
Design Compiler also does 
resynthesis to optimize the circuits during retiming and sizing. % during this process. %retiming and sizing. 
Accordingly, VirtualSync+ should not be used to optimize a circuit from scratch but 
is proposed to resolve remaining timing violations in the circuits that have already been optimized. 
Due to the page limit, we did not include the following figure in the revised manuscript.
%This also confirms that our method is used to resolve the remaining timing violations in the circuits 
%that have already been optimized instead of optimizing a circuit from scratch. 
%Since the original circuit is 
%far from a timing-balanced circuit, directly optimizing it with VirtualSync+ cannot push the timing performance beyond 
%the limit of the traditional timing paradigm. 
\vskip 5.0pt
\begin{minipage}[t]{1\textwidth}%
%\renewcommand{\figurename}{Figure D}
%\renewcommand{\thefigure}{}
\figurefontsize
\centering
%\vskip 9.0pt
\input{Fig/new_cmp}
\vskip -5.0pt
\caption*{Comparison in clock period reduction between extreme retiming and sizing and 
the direct optimization
with VirtualSync+ on the original circuits.} \nonumber%\label{fig:se_cmp}
\end{minipage}
\vskip 10.0pt

 
%In Fig. 14, the performance improvement is not large under relaxed clock periods since
%we used the intermediate timing performance with VirtualSync+ to compare with the performance 
%with relaxed retiming and sizing. 
%The reason is that such intermediate results are relatively evenly distributed, so that we can clearly see 
%that VirtualSync+ achieves a smaller area under the 
%same clock period and a smaller clock period under the same cost compared with relaxed retiming and sizing. 
%If we use the final timing performance improvement, the results with VirtualSync+ concentrate around one data represented with 
%a symbol in Fig. 4, so that we cannot clearly see the advantages of VirtualSync+ over relaxed timing and sizing in area and timing performance.
%We added this point in the left column on page 14.

 
 

%The performance improvement with VirtualSync+ in relaxed clock periods is not significant since we terminate 
%VirtualSync+ before it pushes 
%the timing performance of circuits in such cases into 

%\spe\spb

\textit{Some other minor issues:}\\

\textit{ 
(1) For Fig. 2, the description talks about the arrival times of two signals.  However, the delay unit, flip-flop, and latch all have only one input.  Do the authors really want to talk about difference in the arrival times of two signals or do the authors want to talk about early and late arrival times at the input?  I also think that the authors should show the mapping of input time to the output time without input gap and output gap.  Rather, use another three plots to show input gap (horizontal axis) and output gap (vertical axis).
}\\
\spe\spb

Thanks for the suggestions. We agree with the reviewer that there 
is only one input for the three types of delay units.
However, signals might 
travel through short/long paths, so that they arrive at the same input at different times. 
A signal traveling through a short path arriving at such an input has an early arrival time; another 
signal traveling through a long path arriving at the same input has a late arrival time. 
In Fig. 2, 
%Accordingly, in Fig. 2, 
we want to demonstrate the difference between the early and late arrival times of two signals at the same input.
We have revised Fig. 2 by replacing input gap and output gap with input time and output time, respectively. %according to the suggestions of the reviewer 
We have also revised the corresponding texts in Section IV-A on page 4. \\



\textit{ 
(2) In Fig. 2(c), why T/2 + t\_cq when you allow uneven duty cycle (see D*T) in the same plot.
}\\

Thanks for pointing out this inconsistency. We have revised this figure 
by replacing $T/2+t_{cq}$ to $D*T+t_{cq}$
in the left column on page 4.\\


\textit{ 
(3) 
There are additional variables such as N\_wt in the constraints (7)-(15).  There should be additional constraints when in the optimization formulation when these variables are involved.
}\\

In (7)-(15), $N_{wt}$ is an integer variable, which is determined by the solver.
%This variable does not represent the number of sequential delay units between w and t.
%Due to the removal of flip-flops,  
This variable represents that
the signal arrival time at the input of an inserted sequential delay unit
can be within any clock cycle,
the starting and ending time of which are $N_{wt}*T$ and $(N_{wt}+1)*T$, respectively.
%In addition, the output of an inserted sequential delay unit 
%can start with any number of clock cycles in VirutalSync+ framework. 
%For example, 
%in Fig. 3, we assume that F2 and F3 are removed and 
%a flip-flop is inserted at $u$. Since the input arrival time of 
%the inserted flip-flop is 14,   
%the arrival time of the signal at the output of the inserted flip-flop becomes 
%$1*T+4+3$, where $T$ is the clock period of 10 and the clock-to-q delay is 3. 
%at $t$ is $s_t=3+11-T+3-T=-2*T+3+11+3$, where $T$ is the clock period. 
%We can see that in this case, $N$ is 1 to match the signal arrival time at the output of the inserted flip-flop. %We have revised the sentence in the left column on page 6. 
%For example, along a path where several flip-flops are removed,
%if a flip-flop is inserted along the sink of this path,
%the arrival time at the input of the inserted flip-flop might be negative, which leads
%to a negative $N_{wt}$.
The only constraint for $N_{wt}$ is that the type of this variable should be integer. 
%According to this analysis, 
%there is no
%additional constraints for $N_{wt}$ in the optimization formulation.
We have revised the text below equation (8) in the right column on page 5.
\\

\spe
\reviewe




==> results.tex <==
%\nopagebreak
\section{Experimental Results}\label{sec:results}


\subsection{Experimental Setup}

The proposed method was implemented in C++ and tested
using a \SI[mode=text]{3.20}{\GHz} CPU. 
%with one thread. 
%To demonstrate the effectiveness of \titlenym, 
In the experiments, 
the circuits from the TAU 2013 variation-aware timing analysis 
contest are first optimized using \SI[mode=text]{45}{\nm} library with Design Compiler to reduce area cost. 
%We demonstrate the results using these optimized circuits as the original circuits 
%as in shown in Table~\ref{tb_test}.
These circuits
are referred to the original circuits. 
\reviewhl{The clock periods of these original circuits are shown as $T$ in the fourth column.}
We optimize these circuits further using the proposed \titlenym\ to 
improve timing performance and reduce area. The optimization results are shown in Table~\ref{tb_test}. 
%\reviewhl{The application of \titlenym\ does not depend on the technology of the used library.} 
%These circuits 
%are referred to original circuits. 
%We demonstrate the results using circuits
%from the TAU 2013 variation-aware timing analysis 
%contest as shown in Table~\ref{tb_test}.
The number of flip-flops and the number of combinational components of the original circuits are shown in the  
columns $\boldsymbol{n_s}$ and $\boldsymbol{n_c}$, respectively.
%The benchmark circuits were retimed and sized using a \SI[mode=text]{45}{\nm} library with Design Compiler from Synopsys.
To tolerate process variations, 10\% of timing margin was assigned, so that $r^u$
and $r^l$ in Section~\ref{sec:impl} were set to 1.1 and 0.9, respectively. 
\reviewhl{In case of large variations in advanced technologies, a large timing margin can be 
assigned by increasing $r^u$ and decreasing $r^l$, respectively.}
The allowed phase shifts $\phi_{wt}$ in Section~\ref{sec:impl} are 0, T/4, T/2 and 3T/4. 
\reviewhl{$t_{stable}$ in equation (17) in Section~\ref{sec:model} is set to the delay of a buffer 
to isolate signals on the next wave and the previous wave. 
The initial delay bound $d_{th}$ in Section~\ref{sec:impl} is 7T/8 and iteratively reduced by T/8.}
%Phase shifts $\phi_{wt}$ of the clock signal were allowed to have values of 0, T/4, T/2 and 3*T/4.
The ILP solver used in the \titlenym\ framework was Gurobi.

%To demonstrate that \titlenym\ can 
%push the timing performance beyond the limit of the traditional sequential designs, 
\reviewhl{%Due to the complexity of \titlenym, 
%it can be used to improve timing performance at a late stage, before which 
%circuits have been optimized. }
%Since \titlenym\ is used to improve timing performance in a late design stage, 
%such improvement is significant\textbf{reference???}. } 
The goal of VirtualSync+ is to enhance timing performance and thus 
solve timing violations in the circuits
which have already been optimized.  
%To demonstrate that \titlenym\ can 
Therefore, 
%push the timing performance beyond the limit of the traditional sequential designs, 
the original circuits 
are first retimed and sized extremely %using a \SI[mode=text]{45}{\nm} library 
with Design Compiler to achieve the limit of timing performance. 
Accordingly, extreme retiming and sizing is an integral part of the VirtualSync+ framework. 
}
%the extreme R&S to push the timing
%performance beyond the limit of traditional sequential designs
This extreme retiming and sizing, abbreviated as extreme R\&S, 
is realized by iteratively reducing the clock period and optimizing the circuits with retiming and sizing in Design Compiler
until the circuits cannot be optimized further anymore. 
%This extreme retiming and sizing method is abbreviated as extreme R\&S.  
In the circuits after extreme R\&S, 
the number of flip-flops and the number of combinational components, shown as $\boldsymbol{n^\prime_{s}}$ and $\boldsymbol{n^\prime_{c}}$ in
Table~\ref{tb_test}, are different from those in the original circuits. 
$\boldsymbol{n^\prime_t}$ and $\boldsymbol{n^\prime_c}$ show the clock period reduction 
and the area increase of the circuits after extreme R\&S with respect to the original circuits. 
Overall, the timing performance 
of a circuit is improved significantly by extreme R\&S while the area is increased. 
%the area a circuit after retiming and sizing is larger than that of the original circuit. 
%For example, the clock period of the circuit tv80 is reduced by 40\% after extreme retiming and sizing, 
%while the area is increased by 50\%. 
%the locations of flip-flops are moved structurally to improve the timing performance. 
%For timing optimization, 
%combinational paths whose delays were within 95\%  
%of the largest path delay in the circuit were selected.  
\begin{figure*}
\figurefontsize

\begin{minipage}[t]{0.32\textwidth}%
\centering
%\vskip 9.0pt
\input{Fig/sequential_cmp}
\vskip -12.0pt
\caption{Comparison of sequential delay units after buffer replacement.}\label{fig:se_cmp}
\end{minipage}
~\hspace{5pt}
\begin{minipage}[t]{0.32\textwidth}%
\centering
%\vskip -11.0pt
\input{Fig/buffer_replace}
\vskip -2pt
\caption{Area comparison before and after buffer replacement.}\label{fig:buffer_replace}
\end{minipage}
~\hspace{5pt}
\begin{minipage}[t]{0.32\textwidth}%
\centering
%\vskip -12.0pt
\input{Fig/samet_area_cmp}
\vskip -10pt
\caption{Area comparisons with extreme R\&S with the same clock period.}\label{fig:samet_area_cmp}
\end{minipage}
\end{figure*}

To increase the timing performance with \titlenym, 
in the circuits after extreme R\&S, 
combinational paths whose delays are larger than a specified clock 
period, which is evaluated by iteratively reducing the clock period obtained from extreme R\&S,  
were selected. 
%This specified clock period can be obtained  
%by reducing the clock period obtained from extreme retiming and sizing. % and optimize the 
%circuits with \titlenym\ under this clock period  
%and verifying whether \titlenym\ can operate with or not 
%until \titlenym\ 
%cannot optimize the circuits.   
The source and sink flip-flops of these selected paths were allowed to be
removed, while the other flip-flops in the circuits were
considered as boundary flip-flops. 
All the combinational components that can
reach the flip-flops at the sources or sinks of these selected paths 
through combinational paths 
are considered as the critical part of a circuit together. 
%This extraction of the critical parts of a circuit in fact allows wave-pipelining within three sequential stages. 
%In real circuits, the extracted critical parts may overlap, thus allowing wave-pipelining with more than three stages.  
%so that wave-pipelining with more than three stages may also be possible.  
The extracted critical part of the circuits 
occupied a large portion of the circuits after extreme R\&S, 
as shown in %Table~\ref{tb_test}, 
$\boldsymbol{n_{cs}}$ and $\boldsymbol{n_{cc}}$, which 
represent the percentage of the number of flip-flops and combinational components 
of the critical part in the circuits after extreme R\&S. 
%As shown in the $\boldsymbol{n_{cs}}$ and $\boldsymbol{n_{cc}}$
%columns in Table~\ref{tb_test},
From $\boldsymbol{n_{cs}}$ and $\boldsymbol{n_{cc}}$, we can see that 
more than 4\% of flip-flops and more than 68\% of combinational components have
been selected for timing optimization.
\reviewhl{
In case of industrial designs which contain
hundreds of thousands of
gates in the extracted critical subcircuit, 
%The critical subcircuit is extracted by verifying the largest delays between pairs of flip-flops with respect to  a given clock period.
%Structrually, this critical subcircuit is composed of some critical parts, whoch can be independent or partially connected through flip-flops.
the critical subcircuit can be processed with VirtualSync+ by iteratively selecting a small part for timing optimization.
}
%The area of extracted critical parts consists of about 30\% of the circuits. 



%\begin{figure*}
%\begin{minipage}{0.31\textwidth}%
%\centering
%\vskip 9.0pt
%\input{Fig/sequential_cmp}
%\caption{Comparison of sequential delay units after buffer replacement.}\label{fig:se_cmp}
%\end{minipage}
%~\hspace{10pt}
%\begin{minipage}{0.31\textwidth}%
%\centering
%\vskip 9.0pt
%{
%\input{Fig/buffer_replace}
%}
%\vskip -5pt
%\caption{Area comparison before and after buffer replacement.}\label{fig:buffer_replace}
%\end{minipage}
%~\hspace{10pt}
%\begin{minipage}{0.31\textwidth}%
%\centering
%\vskip 9.0pt
%{
%\input{Fig/samet_area_cmp}
%}
%\vskip -5pt
%\caption{Area comparisons with retiming and sizing with the same clock period.}\label{fig:samet_area_cmp}
%\end{minipage}
%\end{figure*}
\begin{figure}[h]
{
\figurefontsize
\centering
%\vskip 3.0pt
\input{Fig/timing_com}
\caption{Comparison of the clock period reduction before and after fine-tuning with Design Compiler.}
\label{fig:timing_com}
}
\end{figure}

\begin{figure}[h]
{
\figurefontsize
\centering
%\vskip 3.0pt
\input{Fig/area_com}
\caption{Comparison of the area increase before and after fine-tuning with Design Compiler.}
\label{fig:area_com}
}
\end{figure}



\subsection{Experimental Results with Timing Optimization Using Relaxed \titlenym\ Timing Model}\label{sec:secondstep}

To verify the improvement of circuit performance, we gradually reduced the
clock period by 0.5\% of the clock period obtained from extreme R\&S
and applied the timing optimization with relaxed \titlenym\ in Section~\ref{sec:impl} 
to meet the timing constraints. %The implementation of this step 
%and the corresponding results were also described 
%was implemented 
The results correspond to the results described 
in the conference version \cite{Grace2018_DAC} of this paper. %In this paper, 
% and the corresponding results were reported.  
%The following results are also reported in the conference version \cite{Grace2018_DAC}. 
The column $\boldsymbol{n_f}$ and $\boldsymbol{n_l}$ %in Table~\ref{tb_test}
show the numbers of flip-flops and latches in the critical part after optimization with relaxed \titlenym, respectively.
%Since a flip-flop consists of two latches, the number of flip-flops after optimization 
%can be calculated with $\boldsymbol{n_f}$+$\boldsymbol{n_l}$/2, which is smaller compared with 
%that in the original critical part of the circuits in most cases.
The sums of these numbers are comparable or even smaller than the numbers of
flip-flops before relaxed \titlenym.  %% in the critical parts of the circuits.
%but the area taken
%by these componets is smaller due to the included latches.
%These numbers indicate that sequential components are aligned 
%at only indispensable locations to 
%block signal propagations specially on short paths. 
The numbers of extra inserted buffers to match arrival times 
are shown in the column $\boldsymbol{n_{b}}$. 
Thanks to the buffer replacement with sequential units in the proposed framework,
the numbers of extra inserted are not large. %buffers to match arrival times,
%are shown in the column $\boldsymbol{n_{b}}$ in Tabel I, are not large.
Compared with the number of original combinational components shown in the column $n_{cc}$, 
these numbers show that the cost due to the inserted buffers is still acceptable.
%Compare these numbers with the
%numbers of original logic gates shown in the column $n_{cg}$, the cost due to
%these buffers is still acceptable. 

\begin{figure}[t]
{
\figurefontsize
\centering
%\vskip 11.0pt
\input{Fig/power_com}  
\caption{The reduction of power and power-delay-area product compared with extreme R\&S.}
\label{fig:power_com}
}
\end{figure}


\begin{figure*}
\begin{minipage}{1\textwidth}%
\figurefontsize
\centering
\subfloat[][pci\_bridge]{\makebox{\input{Fig/pci}}
%\label{fig:predict_gap}
}%
%\qquad
%
\subfloat[][ac97\_ctrl]{\makebox{\input{Fig/ac97}}
%\label{fig:test_gap}
}
\subfloat[][usb\_funct]{\makebox{\input{Fig/usb}}
%\label{fig:test_gap}
}
\subfloat[][mem\_ctrl]{\makebox{\input{Fig/mem}}
%\label{fig:test_gap}
}
\\
\subfloat[][systemcaes]{\makebox{\input{Fig/syscas}}
%\label{fig:test_gap}
}
\subfloat[][wb\_dma]{\makebox{\input{Fig/wb}}
%\label{fig:test_gap}
}
\subfloat[][tv80]{\makebox{\input{Fig/tv}}
%\label{fig:test_gap}
}
\subfloat[][systemcdes]{\makebox{\input{Fig/sys}}
%\label{fig:test_gap}
}
\caption{Area comparison between relaxed retiming and sizing and \titlenym\ when the target clock period is relaxed to 1.05T, 1.10T, 1.15T, 1.20T and 1.25T, where T is the clock period achieved by extreme R\&S.}
%\caption{Prediction threshold and its effect on yield in \algname~\ref{alg:select_dmt} and \algname~\ref{alg:path_selection} (a), and test threshold over yield in \algname~\ref{alg:delay_test} (b).}
\label{fig:area_per}%
\end{minipage}

\end{figure*}

%To verify the improvement of circuit performance, we gradually reduced the
%clock period by 0.5\% of the clock period obtained from extreme R\&S 
%and applied \titlenym\ to meet the timing constraints. %, which will be called retiming\&sizing in the following paragraphs. 
%extreme retiming in the critical part of circuits.  
The column $\boldsymbol{n_{t}}$ in Table~\ref{tb_test} shows the final clock period 
reduction compared with the circuits after extreme R\&S. 
 The maximum and average reduction are 8.5\% and 3.2\%, respectively, which 
resulted from the compensation between flip-flop stages and the removal
of clock-to-q delays and setup time requirements on critical paths.  
%\reviewhl{
%The reduction of clock period 
%is correlated with the ratio of clock-to-q delays and setup times of the removed flip-flops
%to the delay of critical paths extracted for timing optimization.
%With different logic levels, the path delay might be different. Accordingly,
%we agree with the reviewer that 
%the reduction in clock period is correlated with the logic depth. % as the reviewer mentioned.
%In addition,
%the clock period reduction
%also depends on the structure of the circuit.}
%The clock period reduction depends not only on the number of logic levels but also on the circuit structure.}
For all the cases, the minimum clock periods have been pushed even further than
those from extreme R\&S. %, the limit
%of the traditional sequential design. This comparison demonstrates that the
%proposed method can improve circuit performance even beyond that with extreme retiming and sizing. 
%specially at a late stage of timing closure further, because no circuit redesign is
%required. 
The timing performance improvement $\boldsymbol{n_{t}}$ is achieved with relaxed \titlenym\ described in Section~\ref{sec:impl}.  
%It is
%an upper bound of timing performance improvement due to the heuristics in 
%the timing optimization with relaxed \titlenym. 
This method can be used to quickly evaluate the benefit of \titlenym\ in circuit design. 


The area increase of the proposed method compared with extreme R\&S 
is shown in column $\boldsymbol{n_{a}}$.  
%To guarantee the circuit
%work a given clock, we do gate sizing in the part outside of the selected part
%of the circuit.  
%Compared with the area of retiming, the area increase is
%negligible.  
In the cases with area increase, the overhead is still negligible; in other
cases, the area is even smaller because unnecessary flip-flops were removed 
in the proposed framework. 
% whereas in
%retiming flip-flops can only be moved instead of being removed. 
The last column $t_r$ in Table~\ref{tb_test} shows the runtime of the proposed method. 
Since the ILP formulation with the complete model in Section~\ref{sec:mode_delay_unit}  
is NP-hard, it is impractical to find a solution with respect to area and clock period. In the experiments, 
the runtime with iterative relaxations 
is acceptable in remedying remaining timing violations for late design stage.  %at a late stage of timing closure. % but still has space for
%further improvement. %Without the iterative relaxation methods in Section~\ref{sec:impl}, the runtime using the complete model 
%in Section~\ref{sec:mode_delay_unit} directly are 
%unacceptable since integer linear programming is NP-hard. 
%because the circuit optimization is a one-time effort. 
%To demonstrate the importance of latches in aligning fast and slow signals, we compare performance improvement deploying only flip-flops in our 
%framework with that after retiming and sizing for all circuits, only s5378 and systemcdes achieve the reduction of the clock period, 11.5\% and
%3.5\%, respectively.

%The proposed framework can also deal with the case where only flip-flops are deployed. 
%In this scenario, 
%In this case, we modify the formulation in Section~\ref{sec:seq} to restrict the selection of sequential delay units 
%to be only flip-flops for the solver. 
%compared with circuits after retiming and sizing, 
%only s5378 and systemcdes achieve the reduction of the clock period, 11.5\% and 
%3.5\%, respectively. 
%For other circuits, no performance improvement is achieved because the paths within feedback loops are critical, so that 
%at least a flip-flop is required.
%For other circuits, the minimum clock period achieved with only insertions of flip-flops is same with 
%that achieved by retiming and sizing. The existence of feedback loops requires at least a sequential component, leading to no 
%performance improvement when paths within feedback loops dominate the critical paths.
  

  
In the proposed framework, sequential delay units are first inserted only at
necessary locations to delay signal propagation. Afterwards,
more of them are used to replace buffers to reduce area, as described in 
Section~\ref{sec:impl}.  
%Thanks to the buffer replacement with sequential units in the proposed framework,
%the numbers of extra inserted buffers to match arrival times,
%are shown in the column $\boldsymbol{n_{b}}$ in Tabel I, are not large. 
%which are 
%enough in terms of block signal propagations on short paths. 
%The buffer replacement with 
%sequential components are used to reduce area. 
To demonstrate the effectiveness of the buffer replacement with sequential units 
in the proposed framework, 
we compare the numbers of sequential delay units without 
and with buffer replacement, as shown in 
Figure~\ref{fig:se_cmp}. %compares the numbers of sequential delay units before 
%and after buffer replacement, which 
This figure shows an increase in the number of
such delay units replacing buffers. %meaning a higher delay efficiency.
%It is clear that the numbers of sequential components used 
%to block signal 
%propagations of short paths are relatively 
%small.  
%
%To verify the effectiveness of buffer replacement with sequential components in Section \ref{sec:four_step}, we 
%compare the area of sequential components and buffers with no buffer replacement with that in our framework. 
Figure~\ref{fig:buffer_replace} shows 
the ratio of the chip area after buffer replacement to that before buffer replacement.
%&the area comparison
%reduction 
%after this replacement.  
In all test cases, 
the area after buffer replacement is smaller than that before buffer replacement, 
%the area taken by the sequential delay units and buffers in the 
%optimized circuits is less than 1\% of those replaced buffers, 
%the area after buffer replacement is less 
%the area has been reduced to less
%than 1\%
%after replacement is
%about only a half 
%of the area without replacing buffers by sequential delay units, 
demonstrating the efficiency of
sequential delay units in delaying fast signals. 
%the area reductions are above 80\%, which results from the non-linear block
%effects of sequential components when blocking signal propagations on short
%and long paths.  results from two characteristics of sequential components.
%Firstly, when relatively large number of buffers are required, to reduce
%area, sequential components can be used instead.  Secondly, when a sequential
%component is replaced with several buffers, it can also absorb the
%unnecessary extra buffers to reduce area.  Sequential components provide
%different block effects on signal propagations of long and short paths, so
%when they are replaced, they can adjust arrival times before themselves to
%reduce further extra buffers.



The comparison of the area overhead, shown as $\boldsymbol{n_{a}}$ in Table~\ref{tb_test}, is between  
%we compare the increase of area overhead of 
the clock period achieved by extreme R\&S and the 
clock period reduced further by the proposed method. To demonstrate the area efficiency of the proposed method, we
also compared the proposed method and the extreme R\&S with the same clock period from the latter.  
%the area overhead of the extracted critical parts of the circuits when the same clock period is used for our framework and the method combines retiming and sizing.
%in the extracted critical parts of the circuits.
%of extracted critical parts with
%the same clock period from retiming together with sizing,
%we use the clock period obtained from extreme retiming 
%as the target clock period 
%in our framework to optimize the circuits.  Since the rest part of the circuit
%except the critical part is same for the two cases, we only compare the area
%of the extracted critical part.  Figure~\ref{fig:samet_area_cmp} shows the
%comparisons of area overhead.  
The results are shown in \figname~\ref{fig:samet_area_cmp}.
In most cases, our
framework can further reduce the area achieved by extreme R\&S.  

\subsection{Experimental Results with Circuit Fine-Tuning in Design Compiler}

%\input{tb_add}

The experimental results described in Section~\ref{sec:secondstep} are generated with the timing 
optimization using relaxed \titlenym\ in Section~\ref{sec:impl}. 
These intermediate results 
might be inconsistent with commercial tools due to the simplified model. 
%might not provide an accurate evaluation in timing performance improvement and area reduction. 
To provide more consistent results,  
%To realize \titlenym, 
we fine-tune the optimized circuits with \titlenym\ in Design Compiler, as described in 
Section~\ref{sec:integration}. 
%\reviewhl{
%We have verified the correctness of the timing interface of the optimized circuit parts after fine-tuning with Design Compiler 
%by comparing the arrival times of flip-flops at the boundary of the optimized circuit parts with those in the original circuit.  
%Accordingly, the correct functionality of the optimized circuits can be maintained.}
After this fine-tuning, we reevaluated the improvement of 
timing performance and area reduction with respect to the circuits after extreme R\&S.
The comparisons between the clock period reduction and the area reduction with and without the fine-tuning 
with Design Compiler are illustrated 
in \figname~\ref{fig:timing_com} and \figname~\ref{fig:area_com}, respectively. 
According to these two figures, 
it is clear that in most cases the timing performance with the fine-tuning %with Design Compiler 
can still be pushed beyond that after extreme R\&S while the area is reduced. 
Specifically, the timing 
performance can be improved by up to 4\% (average 1.5\%) compared with that
after extreme R\&S. 
%\reviewhl{
%To achieve timing closure, designers need to spend much
%effort to remove few-picosecond timing violations \cite{Andrew_2014}. 
%Since designers need to spend much
%effort to remove few-picosecond timing violations to achieve timing closure\cite{Andrew_2014}, 
%\titlenym\ provides a good potential in %plays a role in accelerating timing closure 
%removing timing violations at a late stage
%before which circuits have been optimized. 
%For example, %the proposed VirtualSync+ can
%the performance improvement 4\% with \titlenym\ can solve up to 16-picosecond timing violations.}  
%which is significant since designers need to spend much
%effort to remove few-picosecond timing violations to achieve timing closure\cite{Andrew_2014}.}
%Since \titlenym\ is used to improve timing performance in a late design stage, 
%such improvement is significant\textbf{reference???}. 
However, the timing performance improvement with the fine-tuning is less than that without the fine-tuning in most cases.  
%However, the timing performance improvement with the integration is less than that without the integration in most cases. 
%The reason of the results is that 
%In the integration of \titlenym\ with Design Compiler, 
%This phenomenon results from that 
%Due to the timing complexity of latches, 
%in the integration of VirutalSync+ with Design Compiler, 
\reviewhl{One of the reasons is that 
the commercial 
tools do not support 
the timing optimization and analysis of wave-pipelining paths where latches are inserted to block fast signals.
%From the perspective of the tools, a latch is the start or the end of a path, so that
%they do not optimize or analyze paths propagating through a latch. 
%Splitting a wave-pipelining path into two paths with the latch for timing optimization 
%deprives of the flexibility of delay compensation between the separated paths,
%which poses challenges in
%satisfying the corresponding wave-pipelining timing constraints.
}
%Splitting such a path into two paths with the latch for timing optimization deprives 
%the ability of delay compensation between the separated paths.} %cannot be supported in the commercial 
Accordingly, only flip-flops are used as delay units to block fast signals in the fine-tuning of \titlenym\ with Design Compiler.  
%since the timing properties of latches are too complicated to be incorporated into the commercial tools. 
%In addition, the timing performance improvement without the integration is achieved when gates are sized ideally without 
%considering the changes in input transitions and output loads of gates. 
%Therefore, the timing performance improvement without the integration is a theoretical upper bound of timing performance improvment. 
%Accordingly, 
%Therefore, 
%the timing performance improvement with the integration is less than that without the integration in most cases, 
%as shown in \figname~\ref{fig:timing_com}. 
Another reason of this phenomenon is that  
in the iterative relaxation without the fine-tuning, gates are sized ideally 
without  
considering the input transitions and output loads of gates. 
Therefore, the timing performance improvement without the fine-tuning is 
a theoretical upper bound of timing performance improvement, 
which can be used to quickly evaluate the benefit of \titlenym\ in circuit design. 
If it is beneficial to apply \titlenym, designers can then adopt the proposed fine-tuning method with Design Compiler
to generate the optimized circuits.
% so that the timing performance improvement with Design Compiler 
%is less that this theoretical upper bound. 
%\reviewhl{%We also compared the power 
%consumption and power-delay-area product of the circuits optimized 
%with \titlenym\ and with extreme R\&S. 
%The comparison result in power and power-delay-area product is illustrated in \figname~\ref{fig:power_com}. 
%According to this figure, it is clear that 
With \titlenym, 
the power consumption and power-delay-area product of the optimized circuits
can also be reduced %compared with extreme R\&S 
in most cases. The comparison is illustrated in \figname~\ref{fig:power_com}.
%which results from the removal of flip-flops.}

%The comparison in the timing performance 
%is made between \titlenym\ and the method combining retiming and sizing, 
%where 
%To demonstrate the effectiveness of \titlenym, the method 
%combining retiming and sizing is first 
In the experiments, 
the extreme R\&S to push the timing performance 
beyond the limit of traditional sequential designs 
is realized by iteratively reducing the clock period and optimizing 
the circuits with retiming and sizing in Design Compiler until the circuits cannot be optimized further anymore.  
This method squeezes the timing performance 
at the cost of area overhead. %, as shown 
%in the increase in the number of flip-flops in Table~\ref{tb_test}. 
In cases where timing performance does not need to be pushed so far for the sake of area, 
\titlenym\ can still outperform the method combining retiming and sizing in terms of area and speed. 
To demonstrate the effectiveness of \titlenym\ in such cases, 
the clock period achieved by extreme R\&S, denoted as $T$, is relaxed, denoted as relaxed R\&S. 
For 
example, we used the relaxed clock periods 1.05$T$, 1.10$T$, 1.15$T$, 1.20$T$ and 1.25$T$ 
to compare 
%are used for comparison 
%between 
\titlenym\ and relaxed R\&S
in terms of area and timing performance.  
With these relaxed clock periods, 
\titlenym\ with fine-tuning in commercial tools is applied to 
improve the timing performance of the circuits optimized with relaxed R\&S. 
%\reviewhl{To avoid that the performance with \titlenym\ under relaxed clock periods 
%concentrates on one data point, 
%intermediate timing results are used for comparison.}
%with the relaxed clock periods. 
The comparison in timing performance and area with respect to the relaxed clock periods 
is illustrated in \figname~\ref{fig:area_per}, where each pair of symbols, e.g., triangles, represent a comparison in 
timing and area between \titlenym\ and relaxed R\&S with a specified clock period.  
For example, in \figname~\ref{fig:area_per}(a), the pair of triangles represent the results 
with \titlenym\ and relaxed R\&S when the  
clock period is 1.05$T$. Since the result with \titlenym\ is 
at the lower left of the result with the relaxed R\&S, %we can see that 
%According to \figname~\ref{fig:area_per}(a), 
the timing performance with \titlenym\ is better than that of relaxed R\&S, while the area overhead is reduced. 
%From \figname~\ref{fig:area_per}, %we can see that in most cases, 
%\titlenym\ outpeforms retiming\&sizing in terms of timing peformance and area. 
%In addition, 
By connecting these symbols together,  %the performance under these relaxed clock periods, 
we can see that in most cases \titlenym\ achieves a smaller area 
under the same clock period 
compared with 
relaxed R\&S.
%under the same clock period. 
In addition, 
\titlenym\ achieves a smaller clock period under the same area cost compared with  
relaxed R\&S.
%under the same area cost. 



%With \titlenym, the timing performance can be pushed even beyond the limit in the traditional timing 
%paradigm, which can be achieve by combining retiming and sizing. 
%However, the method combining retiming and sizing might increase the area cost significantly, 
%as shown the increase in the number of flip-flops in Table~\ref{tb_test}. 
%In cases where the timing performance does not need to be squeezed   

%The performance comparison between the method combining retiming\&sizing and \titlenym\ 
%is made 
%To compare the performance improvement 



%In fact, 
%the timing performance without the integration is an 


%is 






%Without the iterative relaxation methods in Section~\ref{sec:impl}, the runtime using the complete model 
%in Section~\ref{sec:mode_delay_unit} directly are 
%unacceptable since integer linear programming is NP-hard. 
%However, iterative relaxation methods deprive the optimality of the original problem, which result in 
%the increase of area overhead compared with the optimal solution.  
%In the future, we will explore more efficient methods %, e.g, Lagrangian Relaxation, 
%to reduce the runtime.
%
%than that of retiming since sequential components are
%only aligned at indispensable locations to block signal propagations on short
%and long paths.  


%The proposed model can also handle the scenarios where only flip-flops are
%deployed to optimize the circuits.  We also do experiments with only
%flip-flops in the proposed model. We find in most cases, the clock period
%with this method is same with that of retiming except that $s5378$ and
%$systemcdes$ can still achieve the performance improvement in
%Table~\ref{tb_test}. The reason is that in other circuits, feedback loops
%dominate the critical paths, 
%causing no removement of flip-flops.  
%\begin{figure}[t]
%{
%\figurefontsize 
%\centering
%\makebox
%{
%\input{Fig/samet_area_cmp}
%}
%\vskip -11pt 
%\caption{Area comparisons with extreme timing with same clock period.}
%\label{fig:samet_area_cmp}
%}
%\end{figure}




 


==> solution.tex <==
%\section{Iterative Relaxation in \titlenym}\label{sec:impl}
\section{Timing Optimization with Relaxed \titlenym\ Timing Model}\label{sec:impl}

In applying the \titlenym\ timing model above, we introduce a framework to identify the
locations of delay unit with iterative relaxation of \titlenym.  %where 
%delay effects of sequential delay units are first emulated instead of being modeled directly  
%to relax the timing constraints. 
The flow of this framework is shown in \figname~\ref{fig:flow}, which will be 
explained in this section.  
The basic strategy is to remove flip-flops along critical paths to 
eliminate the inherent clock-to-q delays and setup time. 
Thereafter, fast signals of short paths will be blocked to guarantee the correct functionality by inserting the 
minimum number of sequential delay units and buffers. 
To reduce area overhead, buffers are replaced with sequential delay units.   

%insert the minimum
%number of sequential elements to block fast signals, presented in Section~\ref{sec:first_step}--Section~\ref{sec:third_step}. 
%Thereafter, 
%buffers are replaced with sequential delay units to reduce area overhead in Section~\ref{sec:four_step}. 
%area recovery. 
%Necessary locations of sequential delay units are refined gradually in the models 
%from Section~\ref{sec:first_step} to Section~\ref{sec:third_step}. 
%The variables in the three sections are selected by the solver during the optimization. Constant
%values will be pointed out.
\begin{figure}[t]
{
\figurefontsize
\centering
\input{Fig/flow.pdf_tex}
\caption{The proposed timing optimization with relaxed \titlenym\ flow.}
\label{fig:flow}
}
\end{figure}


\subsection{Emulation of Sequential Delay Units}\label{sec:first_step}

%As shown in \figname~\ref{fig:difference}(a), combinational delay units 
%introduce the same delays to the fast and slow signals.  
After we remove all
the flip-flops from the original circuit, the short paths may have extremely
small delays. The gap between these delays and those of long paths is very large. 
It cannot be 
reduced with combinational delay units since they introduce the same delays to the fast and slow signals as shown in \figname~\ref{fig:difference}(a). 
Instead, only sequential delay units are
able to reduce this gap so that the fast and slow signals still arrive at
boundary flip-flops within the same clock cycle as those of the original circuit.

In the first step of the framework, we identify the locations at which
sequential delay units are indispensable. Without these units, the fast and
slow signals, such as those within feedback loops, may not be aligned properly into the correct clock cycles, even
though unlimited combinational delay units can be inserted into the circuit. 
In practice, however, it is not easy to identify the exact locations of these units using the exact and complete model in (\ref{eq:ff_insertion_0})--(\ref{eq:latch_min_max_bound}) directly.
To solve this problem, 
%delay effects of sequential delay units are first emulated instead of being modeled directly  
%to relax the timing constraints. 
we relax the timing constraints (\ref{eq:ff_insertion_0})--(\ref{eq:latch_min_max_bound}) 
instead of modeling them directly. 
\reviewhl{From \figname~\ref{fig:difference}, 
we can see that a buffer slows down fast and slow signals with the same delay. On the contrary, 
a sequential delay unit slows down fast and slow signals with different delays. 
For example, no matter when fast and slow signals arrive at the input of a flip-flop, they leave the output of the flip-flop at the same time. 
Accordingly, the flip-flop slows down the fast signal with a larger delay than the slow signal. 
%the delay effects of sequential delay units directly. 
Taking advantage of this characteristic, 
we use two non-negative variables $\delta_{wt}$ and $\delta^\prime_{wt}$ to emulate the delay effects of three delay units 
as described above.  % where different delays can be
%padded to slow and fast signals, respectively. 
In case $\delta_{wt} = \delta^\prime_{wt}$, a buffer is inserted. In case $\delta_{wt} < \delta^\prime_{wt}$, a 
sequential delay unit is inserted. 
}
%Specifically, 
%instead of modeling the delay effects of sequential delay units directly, 
%we %first relax the timing constraints \ref{eq:ff_insertion_0})--(\ref{eq:latch_min_max_bound}) 
%emulate the delay effects of sequential delay units shown in \figname~\ref{fig:difference}(b)--(c). }
%in which sequential delay units provide different delay paddings for short and long paths. 
%Therefore, 
%we use two \reviewhl{non-negative variables $\delta_{wt}$ and $\delta^\prime_{wt}$ to emulate different delays to be 
%padded to slow and fast signals, respectively}. 
%To solve this problem, we first emulate the delay effect of sequential components by
%allowing different delays $\delta_{wt}$ and $\delta^\prime_{wt}$ to be 
%padded to slow and fast signals, respectively. 
When signals travel
from $u$ to $z$ in \figname~\ref{fig:circuit_graph}, the relation of arrival times  
from nodes $u$ to $z$ can be written as
\begin{align} 
  s_{z} \ge s_{u} +\xi_{uv}*r^u +d_{vw}*r^u +\delta_{wt}-\lambda_{tz}T \label{eq:ff_orig1} \\ 
  s^\prime_{z} \le s^\prime_{u} +\xi_{uv}*r^l +d_{vw}*r^l+
  \delta^\prime_{wt}-\lambda_{tz}T \label{eq:ff_orig2}  \\
  %\delta_{wt}\le \delta_{wt}^\prime \label{eq:delta_relation}\\
 \reviewhl{0 \le  \delta_{wt} \le \delta_{wt}^\prime}\label{eq:delta_relation}\\
%\le T-(t_{su}*r^u+t_{h}*r^u) \label{eq:delta_relation}\\
   %\delta_{wt}, \delta_{wt}^\prime,  \xi_{uv} \le T \label{eq:area_restrcition}\\
  % 0 \ge \delta_{wt}^\prime-\delta_{wt} \le T-(t_{su}*r^u+t_{h}*r^u) \label{eq:delta_relation}\\
  %s^\prime_{z}+\delta_{wt}^\prime \le s_{z}+\delta_{wt} \label{eq:delta_arr_relation}
   s^\prime_{u}+\delta_{wt}^\prime \le s_{u}+\delta_{wt} \label{eq:delta_arr_relation}
\end{align}
where the variables $\delta_{wt}$ and $\delta_{wt}^\prime$ emulate delays introduced by sequential delay units. 
%emulate the gap between the arrival times at the input of a sequential delay unit and those at the output 
%in the model 
%emulate the complex sequential delay model
%(\ref{eq:ff_insertion_0})--(\ref{eq:latch_min_max_bound}).  
(\ref{eq:delta_relation}) specifies that
the fast signal should be padded with more delays than the slow signal.  
%%% because the large gap between short and long paths after removing the flip-flops 
%needs to be compensated by sequential delay units. 
% and the gap should be no larger than 
%that of sequential components.
% (\ref{eq:area_restrcition}) specifies that the padding delay is restricted to T to reduce area overhead. 
%Pad gap in (\ref{eq:area_gap}) emulates the block effect of sequential components. 
\reviewhl{ %With (\ref{eq:delta_arr_relation}), the arrival time of the fast
%signal does not exceed the arrival time of the slow signal after padding.  
The purpose of (\ref{eq:delta_arr_relation}) 
is to guarantee that a sequential delay unit is required to break a feedback loop.
}

The optimization problem to find the potential locations of sequential delay
units is thus written as
\begin{align} \label{eq:obj_orig1}
\text{minimize}  \quad& \alpha\sum_{G}(\delta_{wt}^\prime-\delta_{wt})+
\beta\sum_{G}(\delta_{wt}^\prime+\xi_{uv})-\gamma\sum_{G}{d_{vw}}\\
%-\beta\sum_{e}d_{v}     
\text{subject to}  \quad&
\text{(\ref{eq:stable_orig})--(\ref{eq:delta_arr_relation}) for each gate in $G$}\\
\phantom{subject to}  \quad&
\text{constr. (\ref{eq:simple_setup})--(\ref{eq:simple_hold})
for each boundary flip-flop}\label{eq:opt_1_bnd}
\end{align}
\reviewhl{where $G$ is the set of all logic gates in the original circuit. 
This optimization problem also maximizes the overall delays of logic gates in
the circuit with the last term in (\ref{eq:obj_orig1}) since larger delays indicate smaller area. %, so that not only the inserted delays but also the area of the circuit 
%can be reduced.
Since the area of a flip-flop is
about 6 times of the area of a buffer and the average area of combinational gates, 
$\alpha$, $\beta$ and $\gamma$ are set to 100,10,10, to specify the balance
between the area of sequential delay units, inserted buffers and logic gates. 
With this setting, we provide the solver a clear tendency to minimize the area of sequential delay units, buffers and combinational gates with different
priorities. 
% roughly and 
%the execution efficiency. 
In the second term, $\delta_{wt}^\prime$ also represents the existence of buffers in case $\delta_{wt}^\prime = \delta_{wt}$.}
Solving the optimization problem above identifies nodes with unequal padding delays
$\delta_{wt}$ and $\delta_{wt}^\prime$, indicating potential locations of
sequential delay units, as a set $S$. These delays may still violate the exact constraints in (\ref{eq:ff_insertion_0})--(\ref{eq:latch_min_max_bound}), 
so that they need to be refined further.

\subsection{Modeling with Clock/Data-to-Q Delays of Sequential Delay Units} 
\label{sec:second_step}

The optimization problem (\ref{eq:obj_orig1})--(\ref{eq:opt_1_bnd}) does not 
%The potential locations of sequential delay units $S$ obtained after solving the optimization problem (\ref{eq:obj_orig1})--(\ref{eq:opt_1_bnd}) 
%may be not accurate and enough to align fast and slow signals, because the optimization 
consider the inherent clock-to-q delays of flip-flops and data-to-q delays of
latches. Since these delays are introduced only at locations where
sequential delay units are inserted, they need to be modeled for all the locations 
$S$ returned by the previous step. We introduce a binary variable $x_{wt}$ to
represent whether a sequential delay unit appears at a location from $S$, and
revise the constraints (\ref{eq:ff_orig1})--(\ref{eq:ff_orig2}) as
\begin{align} 
  & s_{z} \ge s_{u} +\xi_{uv}*r^u +d_{vw}*r^u +x_{wt}\delta_{wt}+
  x_{wt}t_{cd\to q}*r^u-\lambda_{tz}T \label{eq:ff_delay_orig1} \\ 
  & s^\prime_{z} \le s^\prime_{u} +\xi_{uv}*r^l +d_{vw}*r^l
  +x_{wt}\delta^\prime_{wt}+x_{wt}t_{cd\to q}*r^l-\lambda_{tz}T
  \label{eq:ff_delay_orig2}  
\end{align}
where $t_{cd\to q}$ represents
clock-to-q delay or data-to-q delay, which can be evaluated according to the output 
load of the sequential components, and 
%approximated with the same value for
%simplicity, and 
the delays $\delta_{wt}$, $\delta^\prime_{wt}$ and $t_{cd\to q}$ are only valid 
when $x_{wt}$ is equal to 1. The inclusion of the binary variables $x_{wt}$ is very
computation-intensive, so that they can only be dealt with after the potential
locations of sequential delay units are reduced to $S$ by solving
(\ref{eq:obj_orig1})--(\ref{eq:opt_1_bnd}). 
%The multiplication terms 
Since $x_{wt}$ is a binary variable, the multiplications $x_{wt}\delta_{wt}$ and 
$x_{wt}\delta^\prime_{wt}$ can be converted into equivalent linear forms so
that the overall formulation is still an ILP problem.

Considering the inherent delays of sequential delay units, their locations can
be refined further by solving the optimization problem as
\begin{align} \label{eq:obj_delay_orig1}
\text{minimize}  \quad& \alpha\sum_{G/S}(\delta_{wt}^\prime-\delta_{wt})+
\beta\sum_{G/S}(\delta_{wt}^\prime+\xi_{uv})
-\gamma\sum_{G}{d_{vw}}\\
%-\gamma\sum_{S}x_{wt}*(\delta_{wt}^\prime-\delta_{wt}) \\
%-\beta\sum_{e}d_{v}     
\text{subject to}\quad  &%\quad&
\text{(\ref{eq:stable_orig})--(\ref{eq:delta_arr_relation}) for each gate in \reviewhl{$G\backslash S$}}\\
\phantom{subject to} & %\quad&
\text{(\ref{eq:stable_orig}), (\ref{eq:delta_relation})--(\ref{eq:delta_arr_relation}) 
for each gate in $S$}\\
\phantom{subject to} & %\quad&
\text{(\ref{eq:ff_delay_orig1})--(\ref{eq:ff_delay_orig2})
for each gate in $S$
}\\
\phantom{subject to} & %\quad&
\text{constr. (\ref{eq:simple_setup})--(\ref{eq:simple_hold})
for each boundary flip-flop}\label{eq:opt_2_bnd}\\
\phantom{subject to} &
\reviewhl{\delta_{wt}^\prime-\delta_{wt} \ge d_{th} \text{ if } x_{wt}=1 \label{eq:obj_delay_orig1_bnd}}
\end{align}
%In (\ref{eq:obj_delay_orig1}) we actually maximum the delays introduced by the
%sequential delay units, so that the insertion of such units at other locations
%can be reduced. 
%To find all potenital locations of sequential delay units,
%Since $S$ may not be enough in aligning fast and slow signals, we allow those locations $G/S$ 
%to have different delays $\delta_{wt}^\prime$ and $\delta_{wt}$ padded to slow and fast signals. 
%With this method, $S$ will be expanded into a larger set until $\delta_{wt}^\prime$ and $\delta_{wt}$ are equal, which 
%indicates that no sequential delay units are required to provide different delay effects for fast and slow signals. 
\reviewhl{where $d_{th}$ is a predefined 
delay bound. % used to quickly identify the inserting locations of sequential delays units. 
The condition in (32) can be converted into equivalent linear forms according to \cite{gurobi}. }

%In the implementation, we also
%To make the problem easier to solve, we also 
%constrained the
%lower bound of $\delta_{wt}^\prime-\delta_{wt}$ when $x_{wt}$ is equal to 1 
\reviewhl{To identify the necessary locations of sequential delay units, we execute the 
optimization (\ref{eq:obj_delay_orig1})--(\ref{eq:obj_delay_orig1_bnd}) iteratively until 
no different $\delta_{wt}$ and $\delta_{wt}^\prime$ exist anymore. %indicating no indispensable
%sequential delay units are required to align fast and slow signals.
In each iteration, we 
lower the delay bound $d_{th}$ linearly. %, so
%that the most important locations for inserting sequential delay units are
%identified first, as illustrated in \figname~\ref{fig:flow}. 
A large bound of $\delta_{wt}^\prime-\delta_{wt}$ in the early iterations allows
the solver to quickly determine the important locations for inserting sequential delay units.
%The iterations terminate when 
%no different $\delta_{wt}$ and $\delta_{wt}^\prime$ exist, indicating no indispensable 
%sequential delay units are required to align fast and slow signals.
The refined
locations of sequential delay units from this step are returned as a set
$S_d$, which is more accurate than $S$.}


\subsection{Model Legalization for Timing of Sequential Delay Units} \label{sec:third_step}

In this step, the complete model described in Section~\ref{sec:mode_delay_unit} is
applied to the locations in $S_d$ to generate sequential delay units that are
really required in the circuit. The optimization problem is described as 
\begin{align} \label{eq:obj_model_orig1}
\text{minimize}  \quad& \alpha\sum_{G/S_d}(\delta_{wt}^\prime-\delta_{wt})+
\beta\sum_{G/S_d}(\delta_{wt}^\prime+\xi_{uv})
-\gamma\sum_{G}{d_{vw}}\\
\text{subject to}  \quad&
\text{(\ref{eq:stable_orig})--(\ref{eq:delta_arr_relation}) for each gate in \reviewhl{$G\backslash S_{d}$}}\\
\phantom{subject to}  \quad&
\text{(\ref{eq:ff_insertion_0})--(\ref{eq:arriv_latch_orig_2}) 
for each gate in $S_d$}\\
\phantom{subject to}  \quad&
\text{(\ref{eq:latch_new_region})--(\ref{eq:stable_orig})
for each gate in $S_d$ }\\
\phantom{subject to}  \quad&
\text{constr. (\ref{eq:simple_setup})--(\ref{eq:simple_hold})
for each boundary flip-flop.}\label{eq:opt_3_bnd}
\end{align}

After solving the optimization above, there might still be different
$\delta_{wt}$ and $\delta^\prime_{wt}$ in $G\backslash S_d$, \reviewhl{because the timing legalization
of sequential delay units with the complete model (\ref{eq:simple_setup})--(\ref{eq:stable_orig}) excluding
(\ref{eq:latch_min_max}) in Section~\ref{sec:mode_delay_unit} 
may invalidate some locations in $S_d$ so that $S_d$ reduces in size.} The complete %accurate sequential delay
model is applied to these locations iteratively, 
until no different $\delta_{wt}$ and $\delta^\prime_{wt}$ exists, indicating
the remaining timing synchronization can be achieved with buffers and gate
sizing directly.

\subsection{Buffer Replacement with Sequential Units} \label{sec:four_step}

After solving (\ref{eq:obj_model_orig1})--(\ref{eq:opt_3_bnd}), delays $d_{vw}$ of logic gates are 
set to the nearest discrete delay values defined in the library.
%discretized 
%to the nearest delay values according to the types of logic gates in the library. 
%Solving (\ref{eq:obj_model_orig1})--(\ref{eq:opt_3_bnd}) also determines the
Buffer delays $\xi_{uv}$ are also determined. 
If $\xi_{uv}$ is large, several buffers are needed for its implementation.
 As shown in \figname~\ref{fig:difference},
sequential delay units can introduce a very large delay. For example, a flip-flop
can introduce a delay as large as $T+t_{cq}-t_h$, if the incoming signal
arrives at the flip-flop right after a clock edge.  According to this
observation, we iteratively replace buffers with large delays by sequential delay units
to reduce area. 
%The buffers are processed %in a descreasing order 
%with respect to
%their delays $\xi_{uv}$. 
In each iteration, the accurate sequential model
(\ref{eq:ff_insertion_0})--(\ref{eq:arriv_latch_orig_2}) and
(\ref{eq:latch_new_region})--(\ref{eq:stable_orig}) is applied to guarantee these new sequential delay units are
valid. The iteration stops when no buffer can be replaced by sequential units. 
Buffers that cannot be replaced by sequential delay 
units are implemented directly in the optimized circuit.  


%After buffer replacement, delays $d_{vw}$ of logic gates are discretized and
%timing synchronization in the circuit is legalized again using the accurate
%models for delay units, and buffers that cannot be replaced by sequential
%units are implemented directly in the final circuit.   
 
\nopagebreak


==> tb_test.tex <==
%\renewcommand{\tabcolsep}{4.0pt}
%\begin{table}[t]
%\centering
%\renewcommand{\arraystretch}{1.05}
%\centering
%\renewcommand{\tabcolsep}{4.15pt}
\begin{table*}[t]
%\vspace*{-8pt}
\renewcommand{\tabcolsep}{4.15pt}
\centering
{\small
\renewcommand{\arraystretch}{1}

\vskip 10pt
\caption{Results of \titlenym}
\vskip -2pt
\label{tb_test}
\begin{tabular}{lrrr r rrrr r rr r rrr r rr r r} \hlinewd{0.7pt}

\multicolumn{4}{c}{Circuit} &

\multicolumn{1}{c}{} & 

\multicolumn{4}{c}{Ret.\&Siz.} &

\multicolumn{1}{c}{} &

\multicolumn{2}{c}{Cri. Part} &

\multicolumn{1}{c}{} &

\multicolumn{3}{c}{Opt. Circuit} &

\multicolumn{1}{c}{} &

\multicolumn{2}{c}{Comparison} &

\multicolumn{1}{c}{} &

\multicolumn{1}{c}{Runtime}  \\

\cline {1-4} \cline{6-9}  \cline{11-12}  \cline{14-16} \cline {18-19} \cline {21-21} 


\multicolumn{1}{c}{} &
\multicolumn{1}{c}{$n_s$} &
\multicolumn{1}{c}{$n_c$} &
\multicolumn{1}{c}{$T(ps)$} &

\multicolumn{1}{c}{} &

\multicolumn{1}{c}{$n^\prime_{s}$} &
\multicolumn{1}{c}{$n^\prime_{c}$} &
\multicolumn{1}{c}{$n^\prime_{t}$} &
\multicolumn{1}{c}{$n^\prime_{a}$} &
\multicolumn{1}{c}{} &

\multicolumn{1}{c}{$n_{cs}$} & 
\multicolumn{1}{c}{$n_{cc}$} & 

\multicolumn{1}{c}{} &

\multicolumn{1}{c}{$n_{f}$} & 
\multicolumn{1}{c}{$n_{l}$} &
\multicolumn{1}{c}{$n_{b}$} &

\multicolumn{1}{c}{} &

\multicolumn{1}{c}{$n_{t}$} &
\multicolumn{1}{c}{$n_{a}$} &

\multicolumn{1}{c}{} &

\multicolumn{1}{c}{$t(s)$} \\

\hlinewd{0.8pt}
%\hlinewd{0.2pt} 

systemcdes &574  &1286 &1132 & &523 &2429 &55.5\% &23.1\% & &195  &2290 &  &65 &66  & 31& &2.5\%  &-5.4\%  & &2619.5 \\
tv80     &1014 &2998 &1025 & &1228 &5818 &40.0\% &50.4\% & &296 &5758 &  &158 &141  & 383 & &2\%  &0.6\% & &3081.5 \\
wb\_dma     &720  &1632 &666 & &716 &1974 &31.5\% &11.4\% & &129  &1375 &  &65 &46  & 240 & &8.5\%    &1.5\%  & &2211.3 \\
systemcaes &1181  &3318 &921 & &1635 &5078 &29.5\% &38.0\% & &363  &4531 &  &258 &150  & 141 & &3\%    &-1.5\%  & &2052.1 \\
mem\_ctrl  &879 &1840 &1105 & &1429 &3318 &51.0\% &68.3\% & &290 &2642 &  &156&93  & 296& &4.5\%  &-1.5\%  & &4510.5 \\
usb\_funct &2699 &4952 &1042 & &3005 &8901 &35.5\% &28.6\% & &333 &6293 &  &253&71  & 252 & &3\%    &0.1\%  & &2166.5 \\
ac97\_ctrl &1145 &1467 &802 & &2021 &2363 &48.5\% &70.9\% & &579 &1978 &  &430 &125 & 163& &1\%    &-2.2\% & &1961.2 \\
pci\_bridge&2301 &4993 &1141 & &6243 &6476 &33.5\% &130.1\% & &264 &4410 &  &156&48  & 140& &1\%    &-0.7\%  & &3563.1 \\

\hlinewd{0.7pt}
%\end{tabular}
%\end{table}
\end{tabular}
}
\end{table*}

              

